SkinnerDB: Regret-Bounded Query Evaluation via Reinforcement Learning

SkinnerDB is designed from the ground up for reliable join ordering. It maintains no data statistics and uses no cost or cardinality models. Instead, it uses reinforcement learning to learn optimal join orders on the fly, during the execution of the current query. To that purpose, we divide the execution of a query into many small time slices. Different join orders are tried in different time slices. We merge result tuples generated according to different join orders until a complete result is obtained. By measuring execution progress per time slice, we identify promising join orders as execution proceeds. Along with SkinnerDB, we introduce a new quality criterion for query execution strategies. We compare expected execution cost against execution cost for an optimal join order. SkinnerDB features multiple execution strategies that are optimized for that criterion. Some of them can be executed on top of existing database systems. For maximal performance, we introduce a customized execution engine, facilitating fast join order switching via specialized multi-way join algorithms and tuple representations. We experimentally compare SkinnerDB's performance against various baselines, including MonetDB, Postgres, and adaptive processing methods. We consider various benchmarks, including the join order benchmark and TPC-H variants with user-defined functions. Overall, the overheads of reliable join ordering are negligible compared to the performance impact of the occasional, catastrophic join order choice.

==> sectionsPdf/experimentsAppTikz.tex <==

%, and on a commercial database system ((``ComDB'') with an adaptive optimizer. and the commercial system have . We also re-implemented several research baselines (we were unsuccessful in obtaining the original code), notably Eddies~\cite{Tzoumas2008} and the Re-optimizer~\cite{Wu2016}. Some of our implementations are currently limited to simple queries and can therefore not be used for all benchmarks. Specifically for our micro-benchmarks on small data sets, we execute on a standard laptop with 16~GB of main memory and a 2.5~GHZ Intel i5-7200U CPU running Windows 10. 

We show results for additional benchmarks and baselines. As baseline (and underlying execution engine for SkinnerDB), we add a commercial database system ((``ComDB'') with an adaptive optimizer. We also re-implemented several research baselines (we were unsuccessful in obtaining the original code), notably Eddies~\cite{Tzoumas2008} and the Re-optimizer~\cite{Wu2016}. Some of our implementations are currently limited to simple queries and can therefore not be used for all benchmarks. The following experiments are executed on the hardware described before, except for our micro-benchmarks on small data sets which we execute on a standard laptop with 16~GB of main memory and a 2.5~GHZ Intel i5-7200U CPU.

We use an extended version of the \textit{Optimizer Torture Benchmark} proposed by Wu et al. The idea is to create corner cases where the difference between optimal and sub-optimal query plans is significant. \textit{UDF Torture} designates in the following a benchmark with queries where each join predicate is a user-defined function and therefore a black box from the optimizer perspective. We use one good predicate (i.e., join with that predicate produces an empty result) per query while the remaining predicates are bad (i.e., they are always satisfied for the input data). We experiment with different table sizes and join graph structures. \textit{Correlation Torture} is an extended variant of the original benchmark proposed by Wu et al~\cite{Wu2016}. This benchmark introduces maximal data skew by perfectly correlating values in different table columns. As in the original benchmark, we create chain queries with standard equality join and filter predicates. Correlations between predicates and data skew make it however difficult for standard optimizers to infer the best query plan. We vary the position of the good predicate via parameter $m$ between the beginning of the chain ($m=1$) and the middle ($m=nrTables/2$). %Due to space restrictions, we show a representative extract of our experimental results in the following.


\pgfplotsset{
   /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
        {fill=blue,mark=none},%
        {fill=blue!50,mark=none},%
        {fill=cyan,mark=none},%
        {fill=blue!70!red,mark=none},%
        {fill=green,mark=none},%
        {fill=green!50,mark=none},%
        {fill=green!70!red,mark=none},%
        {fill=yellow,mark=none},%
        {fill=yellow!50,mark=none},%
        {fill=yellow!70!red,mark=none},
        {fill=black,mark=none}
     }
   },
}


\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, width=8.5cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Eddy,Optimizer,Reoptimizer,Postgres,S-G(Postgres),S-H(Postgres),Com-DB,S-G(Com-DB),S-H(Com-DB),MonetDB}, legend columns=3, legend to name=b1millisLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={Chain Queries, 100 tuples/table}]
\addChainPlotTime{plots/mb1s100millisAvg}{30000}

\nextgroupplot[bar width=3pt, title={Star Queries, 100 tuples/table}]
\addStarPlotTime{plots/mb1s100millisAvg}{30000}

\end{groupplot}

\node at (3.25,-4.25) {\ref{b1millisLegend}};
\end{tikzpicture}

\caption{UDF Torture benchmark.\label{udfTortureFig}}
\end{figure}

UDF predicates may hide complex code, invocations of external services, or even calls to human crowd workers. They often have to be treated as black boxes from the optimizer perspective which makes optimization hard. Figure~\ref{udfTortureFig} (this and the following figures show arithmetic averages over ten test cases) compares all baselines according to the UDF Torture benchmark described before (the red line marks the timeout per test case). Skinner-C generally performs best in this scenario and beats existing DBMS by many orders of magnitude. We compare a Java-based implementation against highly optimized DBMS execution engines. However, a high-performance execution engine cannot compensate for the impact of badly chosen join orders. Among the other baselines using the same execution engine as we do, Eddy performs best while Optimizer and Re-optimizer incur huge overheads. Re-optimization is more useful in scenarios where a few selectivity estimates need to be corrected. Here, we essentially start without any information on predicate selectivity. For Postgres, our adaptive processing strategies reduce execution time by up to factor 30 for Postgres and large queries. For the commercial DBMS with adaptive optimizer, we achieve a speedup of up to factor 15 (which is in fact a lower bound due to the timeout). 



\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, width=8.5cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Eddy,Optimizer,Reoptimizer,Postgres,S-G(Postgres),S-H(Postgres),Com-DB,S-G(Com-DB),S-H(Com-DB),MonetDB}, legend columns=3, legend to name=b3largeMillisLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={$m=1$; 1,000,000 tuples/table}]
\addChainPlotTime{plots/mb3m1s1000000clearMillisAvg}{30000}
\nextgroupplot[bar width=3pt, title={$m=nrTables/2$; 1,000,000 tuples/table}]
\addChainPlotTime{plots/mb3m2s1000000clearMillisAvg}{30000}
%\nextgroupplot[bar width=3pt, title={Star Queries}]
%\addStarPlotTime{plots/mb3m1s1000000clearMillisAvg}{30000}
%\nextgroupplot[bar width=3pt, title={Star Queries, $m=nrTables/2$}]
%\addStarPlotTime{plots/mb3m2s1000000clearMillisAvg}{30000}
\end{groupplot}

\node at (3.25,-4.25) {\ref{b3largeMillisLegend}};
\end{tikzpicture}

\caption{Correlation Torture benchmark.\label{correlationLargeFig}}
\end{figure}

Even standard equality predicates can make optimization difficult due to predicate correlations. We evaluate all baselines on the Correlation Torture benchmark~\cite{Wu2016}, Figure~\ref{correlationLargeFig} shows first results. Many of the tendencies are similar to the ones in the UDF Torture benchmark. Skinner-C performs best, traditional query optimizers cope badly with strong predicate correlations. Compared to Figure~\ref{udfTortureFig}, the relative performance gap is slightly smaller. At least in this case, UDF predicates cause more problems than correlations between standard predicates. Again, our adaptive processing strategies improve performance of Postgres and the commercial DBMS significantly and for each configuration (query size and setting for $m$). 

\pgfplotsset{
   /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
        {fill=blue,mark=none},%
        {fill=blue!50,mark=none},%
        {fill=cyan,mark=none},%
        {fill=blue!70!red,mark=none},%
        {fill=green,mark=none},%
        {fill=green!50,mark=none},%
        {fill=green!70!red,mark=none},%
        {fill=yellow,mark=none},%
        {fill=yellow!50,mark=none},%
        {fill=yellow!70!red,mark=none},
        {fill=black,mark=none}
     }
   },
}

\begin{figure}[h!]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=2 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, xlabel={\# Tables}, ybar=0pt, legend entries={Skinner, Eddy, Optimizer, Reoptimizer}, width=4.5cm, height=3cm, ylabel near ticks, xlabel near ticks, legend columns=4, ymajorgrids]
\nextgroupplot[bar width=3pt, ylabel={\# Failures}, legend to name=failuresDisastersLegend, title={By Time}]
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3mctsFailures};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3eddyFailures};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3optFailures};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3reoptFailures};
\nextgroupplot[bar width=3pt, ylabel={\# Disasters}, legend to name=dummy, title={By Time}]
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3mctsDisasters};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3eddyDisasters};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3optDisasters};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3reoptDisasters};


\nextgroupplot[bar width=3pt, ylabel={\# Failures}, legend to name=dummy, title={By \#Evaluations}]
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3mctsFailuresPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3eddyFailuresPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3optFailuresPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3reoptFailuresPreds};
\nextgroupplot[bar width=3pt, ylabel={\# Disasters}, legend to name=dummy, title={By \#Evaluations}]
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3mctsDisastersPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3eddyDisastersPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3optDisastersPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3reoptDisastersPreds};
\end{groupplot}

\node at (3.25,-3.75) {\ref{failuresDisastersLegend}};
\end{tikzpicture}

%\ref{failuresDisastersLegend}
\caption{Number of ``optimizer failures'' and ``optimizer disasters''.\label{disasterFig}}
\end{figure}


A query evaluation method that achieves bounded overhead in each single case is typically preferred over a method that oscillates between great performance and significant overheads (even if the average performance is the same). Figure~\ref{disasterFig} summarizes results for a new run of the Correlation Torture benchmark, varying number of tables, table size, as well as parameter $m$. We study robustness of optimization and focus therefore on baselines that use the same execution engine. Note that we compare baselines not only with regards to time, but also with regards to the number of predicate evaluations (see lower row) which depends only on the optimizer. We classify for each baseline a test case as \textit{optimizer failure} if evaluation time exceeds the optimum among the other baselines for that test case by factor 10. We call a test case an \textit{optimizer disaster} for factor 100. The figure shows a tight race between Eddy and the traditional optimizer. Re-optimization clearly improves robustness. However, using our regret-bounded algorithms avoids any failures or disasters and is therefore the most robust optimization method. All implementations in Figure~\ref{disasterFig} share code to the extend possible. Still, some of the baselines need to add code that could in principle decrease performance (e.g., per-tuple routing policies for Eddy). To exclude such effects, we also count the number of atomic predicate evaluations for each baseline and re-calculate failures and disasters based on that (bottom row in Figure~\ref{disasterFig}). The tendencies remain the same.

\pgfplotsset{
    discard if not/.style 2 args={
        x filter/.code={
            \edef\tempa{\thisrowno{#1}}
            \edef\tempb{#2}
            \ifx\tempa\tempb
            \else
                \def\pgfmathresult{inf}
            \fi
        }
    }
}

% Parameters: File name, timeout
\def\addChainPlotTime#1#2{
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmctsS}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINEddy}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINOpt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINReopt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgres}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgresMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgresMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptive}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptiveMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptiveMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmonet}] {#1};
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},#2) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},#2);
}

% Parameters: File name, timeout
\def\addStarPlotTime#1#2{
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmctsS}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAREddy}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAROpt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARReopt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgres}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgresMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgresMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptive}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptiveMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptiveMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmonet}] {#1};
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},#2) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},#2);
}




\begin{figure}
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 1, x descriptions at=edge bottom}, width=8.5cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Eddy,Reoptimizer,Postgres,S-G(Postgres),S-H(Postgres),Com-DB,S-G(Com-DB),S-H(Com-DB)}, legend columns=3, legend to name=b2millisLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks]
\nextgroupplot[bar width=3pt, title={UDF Equality Predicates, 250 tuples/table}, xtick=data]
\addChainPlotTime{plots/mb2s250millisAvg}{30000}
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},30000) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},30000);
\end{groupplot}

\node at (3.25,-1.75) {\ref{b2millisLegend}};
\end{tikzpicture}

\caption{Trivial Optimization benchmark.\label{easyFig1}}
\end{figure}

Our primary goal is to achieve robust query evaluation for corner cases. Still, we also consider scenarios where sophisticated optimization only adds overheads. Figure~\ref{easyFig1} shows results for the Trivial Optimization benchmark in which all query plans avoiding Cartesian products are equivalent. We are mostly interested in relative execution times obtained for the same execution engine with different optimization strategies. Clearly, optimizers that avoid any exploration perform best in this scenario. For the four baselines sharing the Java-based execution engine (Optimizer, Re-Optimizer, and Eddy), this is the standard optimizer. For the baselines that are based on existing DBMS, the original optimizer works best in each case. While robustness in corner cases clearly costs peak performance in trivial cases, the overheads are bounded.






\pgfplotsset{
   /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
        {fill=blue,mark=none},%
        {fill=green,mark=none},%
        {fill=green!50,mark=none},%
        {fill=green!70!red,mark=none},%
        {fill=black,mark=none}
     }
   },
}


\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, width=8.25cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Postgres,S-G(Postgres),S-H(Postgres),MonetDB}, legend columns=3, legend to name=tpchLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={Query}, xticklabels={Q2,Q3,Q5,Q7,Q8,Q9,Q10,Q11,Q18,Q21}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={Standard TPC-H}]
\addplot table[x=Tick, y=Skinner] {plots/tpch.txt};
\addplot table[x=Tick, y=Postgres] {plots/tpch.txt};
\addplot table[x=Tick, y=SkinnerG] {plots/tpch.txt};
\addplot table[x=Tick, y=SkinnerH] {plots/tpch.txt};
\addplot table[x=Tick, y=Monet] {plots/tpch.txt};


\nextgroupplot[bar width=3pt, title={TPC-H with UDFs}]
\addplot table[x=Tick, y=Skinner] {plots/tpch.txt};
\addplot table[x=Tick, y=Postgres] {plots/tpchUDF.txt};
\addplot table[x=Tick, y=SkinnerG] {plots/tpchUDF.txt};
\addplot table[x=Tick, y=SkinnerH] {plots/tpchUDF.txt};
\addplot table[x=Tick, y=MonetDB] {plots/tpchUDF.txt};

\end{groupplot}

\node at (3.25,-3.75) {\ref{tpchLegend}};
\end{tikzpicture}

\caption{Performance on TPC-H queries.\label{tpchFig}}
\end{figure}


Finally, we benchmark several baselines on the more complex queries of the TPC-H benchmark~\cite{TPC2013}. We restrict evaluated approaches to the ones where our current implementation supports the full set of TPC-H queries. Figure~\ref{tpchFig} reports processing times of ten TPC-H queries that join at least three tables. For each query and each approach, we calculate the relative overhead (i.e., query execution time of approach divided by execution time of best approach for this query). The ``Max.\ Rel.\'' column contains for each approach the maximal value over all queries. We study original TPC-H queries as well as a variant that makes optimization hard. The latter variant replaces all unary query predicates by user-defined functions. Those user-defined functions are semantically equivalent to the original predicate. They typically increase per-tuple evaluation overheads. Most importantly, however, they prevent the optimizer from choosing good query plans. 



\begin{table}[b]
\caption{Result summary for TPC-H variants.\label{tpchTable}}
\begin{tabular}{llll}
\toprule[1pt]
\textbf{Scenario} & \textbf{Approach} & \textbf{Time (s)} & \textbf{Max.\ Rel.\ }\\
\midrule[1pt]
TPC-H & Skinner-C & 9 & 22 \\
\midrule
& Postgres & 15 & 37 \\
\midrule
& S-G(Postgres) & 182 & 594 \\
\midrule
& S-H(Postgres) & 38 & 97 \\
\midrule
& MonetDB & 2 & 3 \\
\midrule[1pt]
TPC-UDF & Skinner-C & 9& 3 \\
\midrule
& Postgres & 3,117 & 3,457 \\
\midrule
& S-G(Postgres) & 305 & 154 \\
\midrule
& S-H(Postgres) & 142 & 88 \\
\midrule
& MonetDB & 53 & 20 \\
\bottomrule[1pt]
\end{tabular}
\end{table}

The upper half of Figure~\ref{tpchFig} shows results on original TPC-H queries while the lower half reports on the UDF variant. Table~\ref{tpchTable} summarizes results, reporting total benchmark time as well as the maximal per-query time overhead (compared to the optimal execution time for that query over all baselines). MonetDB is the clear winner for standard queries (also note that MonetDB and SkinnerDB are column stores while Postgres is a row store). SkinnerDB achieves best performance on the UDF variant. Among the three Postgres-based approaches, the original DBMS performs best on standard cases. The hybrid approach performs reasonably on standard cases but reduces total execution time by an order of magnitude for the UDF scenario. We therefore succeed in trading peak performance in standard cases for robust performance in extreme cases.
\balance

 % On the UDF variant, the hybrid approach reduces total execution time by orders of magnitude.

==> sectionsTikz/algorithm.tex <==
\section{Algorithms}
\label{algorithmSec}

We describe several adaptive processing strategies that are implemented in SkinnerDB. In Section~\ref{uctSub}, we introduce the UCT algorithm that all processing strategies are based upon. In Section~\ref{learningSub}, we describe how the UCT algorithm can generally be used to learn optimal join orders. In Section~\ref{genericSub}, we introduce a join order learning approach that can be implemented on top of existing SQL processing engines, in a completely non-intrusive manner. In Section~\ref{hybridSub}, we show how this strategy can integrate plans proposed by the original optimizer. In Section~\ref{customizedSub}, we propose a new query evaluation method that facilitates join order learning and the associated learning strategy. 

While we describe the following algorithms only for SPJ queries, it is straight-forward to add sorting, grouping, or aggregate calculations in a post-processing step (we do so in our actual implementation). Nested queries can be treated via decomposition~\cite{Neumann}.

\begin{comment}
We describe several adaptive processing strategies based on reinforcement learning. As shown in Section~\ref{analysisSec}, all algorithms offer formal guarantees on expected regret (i.e., delta between actual and optimal execution time). Also, all algorithms have been implemented in the SkinnerDB system. We evaluate those algorithms experimentally in Section~\ref{experimentsSec}.

In Section~\ref{preliminariesSub}, we discuss how reinforcement learning can be used for learning optimal join orders in general. This discussion establishes the fundament for the following subsections. In Section~\ref{genericSub}, we describe a processing strategy that works with any execution engine. We have implemented that strategy in a completely non-intrusive manner on top of several existing DBMS such as Postgres, enabling them to process difficult-to-optimize queries where their original optimizer fails. In Section~\ref{hybridSub}, we show how to combine this learning-based approach with the original optimizer, enabling execution of difficult queries while not causing significant learning overheads for standard queries. The strategies discussed in the latter two subsections can be used on top of all existing DBMSs supporting an SQL interface (without changing a single line of DBMS code). In Section~\ref{customizedSub}, we present a join order learning approach that relies on a customized execution engine for select-project-join (SPJ) queries. While we describe the following algorithms only for SPJ queries, it is straight-forward to add sorting, grouping, or aggregate calculations in a post-processing step. Nested queries can be treated via decomposition~\cite{Selinger1979}.
\end{comment}

\subsection{Background on UCT}
\label{uctSub}

Our method for learning optimal join orders is based on the UCT algorithm~\cite{Kocsis2006}. This is an algorithm from the area of reinforcement learning. It assumes the following scenario. We repeatedly make choices that result in rewards. Each choice is associated with reward probabilities that we can learn over time. Our goal is to maximize the sum of obtained rewards. To achieve that goal, it can be beneficial to make choices that  resulted in large rewards in the past (``exploitation'') or choices about which we have little information (``exploration'') to inform future choices. The UCT algorithm balances between exploration and exploitation in a principled manner that results in probabilistic guarantees. More precisely, assuming that rewards are drawn from the interval $[0,1]$, the UCT algorithm guarantees that the expected regret (i.e., the difference between the sum of obtained rewards to the sum of rewards for optimal choices) is in $O(\log(n))$ where $n$ designates the number of choices made~\cite{Kocsis2006}. %Based on Hoeffding's inequality, those guarantees hold independently from the type of the probability distributions from which rewards are drawn (as long as rewards are drawn from a bounded value domain, typically the interval $[0,1]$). 

We specifically select the UCT algorithm for several reasons. First, UCT has been applied successfully to problems with very large search spaces (e.g., planning Go moves~\cite{Gelly2012}). This is important since the search space for join ordering grows quickly in the query size. Second, UCT provides formal guarantees on cumulative regret (i.e., accumulated regret over all choices made). Other algorithms from the area of reinforcement learning~\cite{Feldman2014} focus for instance on minimizing simple regret (i.e., quality of the final choice). The latter would be more appropriate when separating planning from execution. Our goal is to interleave planning and execution, making the first metric more appropriate. Third, the formal guarantees of UCT do not depend on any instance-specific parameter settings~\cite{Domshlak2013}, distinguishing it from other reinforcement learning algorithms.

We assume that the space of choices can be represented as a search tree. In each round, the UCT algorithm makes a series of decisions that can be represented as a path from the tree root to a leaf. Those decisions result in a reward from the interval $[0,1]$, calculated by an arbitrary, randomized function specific to the leaf node (or as a sum of rewards associated with each path step). Typically, the UCT algorithm is applied in scenarios where materializing the entire tree (in memory) is prohibitively expensive. Instead, the UCT algorithm expands a partial search tree gradually towards promising parts of the search space. The UCT variant used in our system expands the materialized search tree by at most one node per round (adding the first node on the current path that is outside the currently materialized tree). 

Materializing search tree nodes allows to associate statistics with each node. The UCT algorithm maintains two counters per node: the number of times the node was visited and the average reward that was obtained for paths crossing through that node. If counters are available for all relevant nodes, the UCT algorithm selects at each step the child node $c$ maximizing the formula $r_c+w\cdot \sqrt{\log(v_p)/v_c}$ where $r_c$ is the average reward for $c$, $v_c$ and $v_p$ are the number of visits for child and parent node, and $w$ a weight factor. In this formula, the first term represents exploitation while the second term represents exploration. Their sum represents the upper bound of a confidence bound on the reward achievable by passing through the corresponding node (hence the name of the algorithm: UCT for Upper Confidence bounds applied to Trees). Setting $w=\sqrt{2}$ is sufficient to obtain bounds on expected regret. It can however be beneficial to try different values to optimize performance for specific domains~\cite{Domshlak2013}.

\subsection{Learning Optimal Join Orders}
\label{learningSub}

%We explain, in general terms, how to use the UCT algorithm to learn optimal join orders. The following subsections describe concrete instances of the following high-level approach.

Our search space is the space of join orders. We consider all join orders except for join orders that introduce Cartesian product joins without need. Avoiding Cartesian product joins is a very common heuristic that is used by virtually all optimizers~\cite{Gubichev2015}. 
To apply the UCT algorithm for join ordering, we need to represent the search space as a tree. We assume that each tree node represents one decision with regards to the next table in the join order. Tree edges represent the choice of one specific table. The tree root represents the choice of the first table in the join order. All query tables can be chosen since no table has been selected previously. Hence, the root node will have $n$ child nodes where $n$ is the number of tables to join. Nodes in the next layer of the tree (directly below the root) represent the choice of a second table. We cannot select the same table twice in the same join order. Hence, each of the latter node will have at most $n-1$ child nodes associated with remaining choices. The number of choices depends on the structure of the join graph. If at least one of the remaining tables is connected to the first table via join predicates, only such tables will be considered. If none of the remaining tables is connected, all remaining tables become eligible (since a Cartesian product join cannot be avoided given the initial choice). In total, the search tree will have $n$ levels. Each leaf node is associated with a completely specified join order. 

We generally divide the execution of a query into small time slices in which different join order are tried. For each time slice, the UCT algorithm selects a path through the aforementioned tree, thereby selecting the join order to try next. As discussed previously, only part of the tree will be ``materialized'' (i.e., we keep nodes with node-specific counters in main memory). When selecting a path (i.e., a join order), UCT exploits counters in materialized nodes wherever available to select the next path step. Otherwise, the next step is selected randomly. After a join order has been selected, this join order is executed during the current time slice. Results from different time slices are merged (while removing overlapping results). We stop once a complete query result is obtained.

Our goal is to translate the aforementioned formal guarantees of UCT, bounding the distance between expected and optimal reward (i.e., the regret), into guarantees on query evaluation speed. To achieve that goal, we must link the reward function to query evaluation progress. The approaches for combined join order learning and execution, presented in the following subsections, define the reward function in different ways. They all have however the property that higher rewards correlate with better join orders. After executing the selected join order for a bounded amount of time, we measure evaluation progress and calculate a corresponding reward value. The UCT algorithm updates counters (average reward and number of visits) in all materialized tree nodes on the previously selected path. 

The following algorithms use the UCT algorithm as a sub-function.  More precisely, we use two UCT-related commands in the following pseudo-code: \Call{UctChoice}{$T$} and \Call{RewardUpdate}{$T,j,r$}. The first one returns the join order chosen by the UCT algorithm when applied to search tree $T$ (some of the following processing strategies maintain multiple UCT search trees for the same query). The second function updates tree $T$ by registering reward $r$ for join order $j$. Sometimes, we will pass a reward function instead of a constant for $r$ (with the semantics that the reward resulting from an evaluation of that function is registered).

\begin{comment}
Second, the algorithm assumes that the regret to minimize accumulates over the learning phase. It thereby differs from some other, recently proposed, algorithms that measure regret only after learning has finished. The latter would be appropriate if having a separate planning and execution stage. Here, we interleave learning and execution and therefore want to minimize accumulated regret. 

We discuss how reinforcement learning can be used to learn optimal join orders. All processing strategies presented in the following subsections are based on one specific reinforcement learning algorithm: the UCT algorithm. This algorithm learns an optimal sequence of actions. It has been used very successfully for planning problems with large search spaces~\cite{Gelly2012}. To use that algorithm for join ordering, we must first represent the choice of a join order as a sequence of \textit{Actions}. We focus on left-deep query plans where join order is described by a permutation of tables. Hence, we can simply model the selection of the next table in a join order as one action. Executing a sequence of $m$ actions for a query joining $m$ tables leads to a complete join order. 

Applying actions changes \textit{State}. The state generally determines what actions can be applied next. In case of join ordering, we simply use the set of tables joined so far to characterize state. The action sequence selecting a join order starts from the state associated with the empty table set (i.e., no tables are initially joined). Applying action $a$ in state $S$ (where $a$ is a table and $S$ a table set) leads to state $S\cup\{a\}$. The set of applicable actions is determined by the state as follows. First, actions are excluded that refer to tables already joined in the current state. Second, we use a popular heuristic that avoids Cartesian product joins~\cite{Selinger1979}. This means that we consider only actions joining a table that is connected by at least one predicates to tables already joined before (if at least one such action exists). This heuristic is used by virtually all modern optimizers~\cite{Gubichev2015}. 

The UCT algorithm iteratively executes action sequences. Each action sequence results in a \textit{Reward} that accumulates over different iterations. The goal of the UCT algorithm is to maximize the accumulated reward or, equivalently, to minimize expected regret (i.e., the difference between actual and optimal accumulated reward). In case of join ordering, we enable iterative execution for a single query by dividing input data into batches or by limiting execution time after each selection. The processing strategies presented in the following sections use different reward functions. Common to all of those reward functions is that they tend to associate a higher reward with join orders that result in lower execution time. UCT comes with formal bounds on the expected regret~\cite{Kocsis2006}. We prove bounds on expected execution cost regret (i.e., difference between actual and optimal query execution time) for our algorithms in Section~\ref{analysisSec}. They are based on the formal guarantees provided by UCT. 

The knowledge acquired by the UCT algorithm over different iterations is stored in the form of a search tree. This tree only represents parts of the search space that have been explored so far. The UCT algorithm is typically used in situations where representing the entire search space would take prohibitive amounts of space~\cite{Gelly2012}. This applies to the case of join ordering as well. Starting from a single node, we expand the tree by at most one node per iteration. We expand the tree whenever an action leads to a state whose node has not been constructed yet (completing the join order randomly if more than one node is missing). Each node in the UCT search tree is associated with a sequence of actions leading to that point. Tree edges represent actions. Each tree node is associated with a counter, representing the number of iterations in which it was visited. Also, each tree edge is associated with an average reward that was obtained via paths passing through that edge. Together, the number of visits and the average reward allow to calculate a measure of ``interestingness'' for specific actions. More precisely, we can calculate an upper bound on the expected reward associated with specific actions (based on reward average and number of visits). This allows the UCT algorithm to balance the need for exploration (i.e., learning about actions with high uncertainty) versus the need for exploitation (i.e., using actions that have proven to work well in the past).

The following algorithms use the UCT algorithm as a sub-function.  More precisely, we use two UCT-related commands in the following pseudo-code: \Call{UctChoice}{$T$} and \Call{RewardUpdate}{$T,j,r$}. The first one returns the join order chosen by the UCT algorithm when applied to search tree $T$ (some of the following processing strategies maintain multiple UCT search trees for the same query). The second function updates tree $T$ by registering reward $r$ for join order $j$. Sometimes, we will pass a reward function instead of a constant for $r$ (with the semantics that the reward resulting from an evaluation of that function is registered).
\end{comment}

\subsection{Generic Execution Engines}
\label{genericSub}

In this subsection, we show how we can learn optimal join orders when treating the execution engine as a black box with an SQL interface. This approach can be used on top of existing DBMS without changing a single line of their code. 

A naive approach to learn optimal join orders in this context would be the following. Following the discussion in the last subsection, we divide each table joined by the input query into an equal number of batches (if the input query contains unary predicates in the where clause, we can apply them in the same step). We simplify by assuming that all tables are sufficiently large to contain at least one tuple per batch (otherwise, less batches can be used for extremely small tables). We iteratively choose join orders using the UCT algorithm. In each iteration, we use the given join order to process a join between one batch \textit{for the left most table in the join order} and the remaining, complete tables. We remove each processed batch and add the result of each iteration to a result relation. We terminate processing once all batches are processed for at least one table. As we prove in more detail in Section~\ref{analysisSec}, the result relation contains a complete query result at this point. To process the query as quickly as possible, we feed the UCT algorithm with a reward function that is based on processing time for the current iteration. The lower execution time, the higher the corresponding reward. Note that reducing the size of the left-most table in a join order (by using only a single batch) tends to reduce the sizes of all intermediate results. If the dominant execution time component is proportional to those intermediate result sizes (e.g., time for generating intermediate result tuples, index lookups, number of evaluated join predicates), execution time for one batch is proportional to execution time for the entire table (with a scaling factor that corresponds to the number of batches per table). %We formalize this argument in Section~\ref{analysisSec}.

The reason why we call the latter algorithm naive is the following. In many settings, the reward function for the UCT algorithm is relatively inexpensive to evaluate. In our case, it requires executing a join between one batch and all the remaining tables. The problem is that execution cost can vary strongly as a function of join order. The factor separating execution time of best and worst join order may grow exponentially in the number of query tables. Hence, even a single iteration with a bad join order and a single tuple in the left-most table may lead to an overall execution time that is far from the optimum for the entire query. Hence, we must upper-bound execution time in each iteration.

%Our goal is to achieve regret bounds that scale gracefully in the query size. This is not possible if we execute an entire batch with any join order until the end. Clearly, we must upper-bound execution time in each iteration.

This leads however to a new problem: what timeout should we choose per batch in each iteration? Ideally, we would select as timeout the time required by an optimal join order. Of course, we neither know an optimal join order nor its optimal processing time for a new query. Using a timeout that is lower than the optimum prevents us from processing an entire batch before the timeout. This might be less critical if we can backup the state of the processing engine and restore it when trying the same join order again. However, we currently treat the processing engine as a black box and cannot assume access to partial results and internal state. Further, most SQL processing engines execute a series of binary joins and generate potentially large intermediate results. As we may try out many different join orders, already the space required for storing intermediate results for each join order would become prohibitive. So, we must assume that all intermediate results are lost if execution times out before a batch is finished. Using lower timeouts than necessary prevents us from making any progress. On the other side, choosing a timeout that is too high leads to unnecessary overheads when processing sub-optimal join orders. 

\tikzstyle{timeBudget}=[anchor=south west, draw=black, rounded corners=0.15cm, fill=blue!15]

\begin{figure}[t]
\centering
\begin{tikzpicture}
\draw (0,0) -- (7,0);
\draw[->] (0,0) -- (0,2);
\node[timeBudget, minimum width=1cm] at (0,0) {1};
\node[timeBudget, minimum width=1cm] at (1,0) {2};
\node[timeBudget, minimum width=2cm] at (0,0.5) {3};
\node[timeBudget, minimum width=1cm] at (2,0) {4};
\node[timeBudget, minimum width=1cm] at (3,0) {5};
\node[timeBudget, minimum width=2cm] at (2,0.5) {6};
\node[timeBudget, minimum width=4cm] at (0,1) {7};
\node[timeBudget, minimum width=1cm] at (4,0) {8};
\node[timeBudget, minimum width=1cm] at (5,0) {9};
\node[timeBudget, minimum width=2cm] at (4,0.5) {10};
\node[timeBudget, minimum width=1cm] at (6,0) {11};
\node[font=\itshape] at (3.5,-0.5) {Time Units};
\node[font=\itshape, rotate=90, align=center] at (-0.5,1) {Timeout Level};
\foreach \x in {1,2,3,4,5,6,7}{
\draw[draw=black] (\x,0) -- (\x,-0.2);
}
\end{tikzpicture}
\caption{Illustration of time budget allocation scheme: we do not know the optimal time per batch and iterate over different timeouts, allocating higher budgets less frequently.\label{budgetFigure}}
\end{figure}

The choice of a good timeout is therefore crucial while we cannot know the best timeout a-priori. The solution lies in an iterative scheme that tries different timeouts in different iterations. We carefully balance allocated execution time over different timeouts, avoiding to use higher timeouts unless lower ones have been tried sufficiently often. More precisely, we will present a timeout scheme that ensures that the total execution time allocated per timeout does not differ by more than factor two across different timeouts. Figure~\ref{budgetFigure} gives an intuition for the corresponding timeout scheme (numbers indicate the iteration in which the corresponding timeout is chosen). We use timeouts that are powers of two (we also call the exponent the \textit{Level} of the timeout). We always choose the highest timeout for the next iteration such that the accumulated execution time for that timeout does not exceed time allocated to any lower timeout. Having fixed a timeout for each iteration, we assign a reward of one for a fixed join order if the input was processed entirely. We assign a reward of zero otherwise. 

Algorithm~\ref{nonIntrusiveAlg} present pseudo-code matching the verbal description. First, tuples are filtered using unary predicates and the remaining tuples are partitioned into $b$ batches per table (we omit pseudo-code for pre-processing). We use function~\Call{DBMS}{} to invoke the underlying DBMS for processing one batch with a timeout. The function accumulates partial result in a result relation if processing finishes before the timeout and returns \textbf{true} in that case. Vector $o_i$ stores for each table an offset, indicating how many of its batches were completely processed (it is implicitly initialized to one for each table). Variable $n_l$ stores for each timeout level $l$ how much execution time was dedicated to it so far (it is implicitly initialized to zero and updated in each invocation of function~\Call{NextTimeout}{}). Note that we maintain separate UCT trees $T_t$ for each timeout $t$ (implicitly initialized as a single root node representing no joined tables). This prevents for instance processing failures for lower timeouts to influence join ordering decisions for larger timeouts. We prove the postulated properties of the timeout scheme (i.e., balancing time over different timeouts) in Section~\ref{analysisSec}. 

\begin{comment}
\algrenewcommand\alglinenumber[1]{\small #1:}
\begin{algorithm}[t]
\renewcommand{\algorithmiccomment}[1]{// #1}
%\newcommand{\pushcode}[1][1]{\hskip\dimexpr#1\algorithmicindent\relax}
%\algsetup{linenosize=\small}
\begin{small}
\begin{algorithmic}[1]
\State \Comment{Apply unary predicates in query $q$ and}
\State \Comment{partition each table into $b$ batches.}
\Function{PreprocessingG}{$q=R_1\Join\ldots\Join R_m,b$}
\State \Comment{Initialize result set}
\State $R\gets\emptyset$
\State \Comment{Iterate over all tables in query}
\For{$i\in 1\ldots m$}
\State \Comment{Filter each table via unary predicates}
\State $F_i\gets\sigma_{\Call{Unary}{q}}(R_i)$
\State \Comment{Divide table into $b$ batches}
\State $R\gets R\cup\{\Call{Partitions}{F_i,b}\}$
\EndFor
\State \Return{$R$}
\EndFunction
\vspace{0.15cm}
\State \Comment{Returns timeout for processing next batch,}
\State \Comment{based on times $n$ given to each timeout before.}
\Function{NextTimeout}{$n$}
\State \Comment{Choose timeout level}
\State $L\gets\max\{L|\forall l<L:n_l\geq n_L+2^L\}$
\State \Comment{Update total times given to levels}
\State $n_L\gets n_L+2^L$
\State \Comment{Return timeout for chosen level}
\State \Return{$2^L$}
\EndFunction
\end{algorithmic}
\end{small}
\caption{Auxiliary functions for regret-bounded query evaluation with generic engine.\label{nonIntrusiveAuxAlg}}
\end{algorithm}
\end{comment}

\begin{algorithm}[t!]
\renewcommand{\algorithmiccomment}[1]{// #1}
%\newcommand{\pushcode}[1][1]{\hskip\dimexpr#1\algorithmicindent\relax}
%\algsetup{linenosize=\small}
\begin{small}
\begin{algorithmic}[1]
\State \Comment{Returns timeout for processing next batch,}
\State \Comment{based on times $n$ given to each timeout before.}
\Function{NextTimeout}{$n$}
\State \Comment{Choose timeout level}
\State $L\gets\max\{L|\forall l<L:n_l\geq n_L+2^L\}$
\State \Comment{Update total time given to level}
\State $n_L\gets n_L+2^L$
\State \Comment{Return timeout for chosen level}
\State \Return{$2^L$}
\EndFunction
\vspace{0.15cm}
\State \Comment{Process SPJ query $q$ using existing DBMS and}
\State \Comment{by dividing each table into $b$ batches.}
\Procedure{SkinnerG}{$q=R_1\Join\ldots\Join R_m,b$}
\State \Comment{Apply unary predicates and partitioning}
\State $\{R_1^1,\ldots,R_m^b\}\gets$\Call{PreprocessingG}{$q,b$}
\State \Comment{Until we processed all batches of one table}
\While{$\nexists i:o_i>b$}
\State \Comment{Select timeout using pyramid scheme}
\State $t\gets$\Call{NextTimeout}{n}
\State \Comment{Select join order via UCT algorithm}
\State $j\gets$\Call{UctChoice}{$T_t$}
\State \Comment{Process one batch until timeout}
\State $suc\gets$\Call{DBMS}{$R_{j1}^{o_{j1}}\Join R_{j2}^{o_{j2}..b}\ldots\Join R_{jm}^{o_{jm}..b},t$}
\State \Comment{Was entire batch processed successfully?}
\If{$suc$}
\State \Comment{Mark current batch as processed}
\State $o_{j1}\gets o_{j1}+1$
\State \Comment{Store maximal reward in search tree}
\State \Call{RewardUpdate}{$T_t,j,1$}
\Else
\State \Comment{Store minimal reward in search tree}
\State \Call{RewardUpdate}{$T_t,j,0$}
\EndIf
\EndWhile
\EndProcedure
\end{algorithmic}
\end{small}
\caption{Regret-bounded query evaluation using a generic execution engine.\label{nonIntrusiveAlg}}
\end{algorithm}

\subsection{Hybrid Algorithm}
\label{hybridSub}

%The algorithm presented in the last subsection uses an existing execution engine, for instance a relational DBMS. Typically, a relational DBMS comes with a traditional query optimizer that uses data statistics to calculate optimal join orders. 

The algorithm presented in the last subsection uses reinforcement learning alone to order joins. It bypasses any join ordering capabilities offered by an existing optimizer completely. This approach is efficient for queries where erroneous statistics or difficult-to-analyze predicates mislead the traditional optimizer. However, it adds unnecessary learning overheads for standard queries where a traditional optimizer would produce reasonable query plans. 


\begin{figure}[t]
\begin{tikzpicture}
\draw[->] (0,0) -- (7,0);
\node[timeBudget, fill=red!15, minimum width=1cm] at (0,0) {1};
\node[timeBudget, minimum width=1cm] at (1,0) {2};
\node[timeBudget, fill=red!15, minimum width=2cm] at (2,0) {3};
\node[timeBudget, minimum width=2cm] at (4,0) {4};
\node at (6.5,0.25) {\ldots};
\node[font=\itshape] at (3.5,-0.5) {Time};
\foreach \x in {1,2,3,4,5,6}{
\draw[draw=black] (\x,0) -- (\x,-0.2);
}
\end{tikzpicture}
\caption{The hybrid approach alternates with increasing timeouts between executing plans proposed by the traditional optimizer (red) and learned plans (blue).\label{hybridFig}}
\end{figure}


We present a hybrid algorithm that combines reinforcement learning with a traditional query optimizer. Instead of using an existing DBMS only as an execution engine, we additionally try benefiting from its query optimizer whenever possible. We do not provide pseudo-code for the hybrid algorithm as it is quick to explain. We iteratively execute the query using the plan chosen by the traditional query optimizer, using a timeout of $2^i$ where $i$ is the number of invocations (for the same input query) and time is measured according to some atomic units (e.g., several tens of milliseconds). In between two traditional optimizer invocations, we execute the learning based algorithm described in the last subsection. We execute it for the same amount of time as the traditional optimizer. We save the state of the UCT search trees between different invocations of the learning approach. Optionally, if a table batch was processed by the latter, we can remove the corresponding tuples before invoking the traditional optimizer. Figure~\ref{hybridFig} illustrates the hybrid approach. As shown in Section~\ref{analysisSec}, the hybrid approach bounds expected regret (compared to the optimal plan) and guarantees a constant factor overhead compared to the original optimizer.

%We analyze the guarantees offered by the hybrid algorithm in Section~\ref{analysisSec}.


%Calling the traditional optimizer with a timeout is an insurance against cases where the traditional optimizer produces catastrophic plans. In those cases, we learn good join orders via the UCT approach. Due to the geometric progression of timeouts, the accumulated time spent in all prior invocations is always bounded by the timeout for the next iteration. This means that our insurance against catastrophic query plans increases execution time only by a bounded amount (i.e., bounded by a constant factor) for cases where the traditional optimizer works well. Compared to using the traditional optimizer alone, the hybrid algorithm essentially provides a way to sacrifice a bounded amount of performance for standard cases to achieve robustness for difficult-to-optimize queries. We analyze the guarantees offered by the hybrid algorithm in more detail in Section~\ref{analysisSec}. We share progress between the traditional optimizer and the learning approach (by removing tuples in processed batches). 


\subsection{Customized Execution Engines}
\label{customizedSub}

The algorithms presented in the previous sections can work with any execution engine for SPJ queries. In this section, we present an execution engine that is tailored towards the needs of a learning based join ordering strategy.  In addition, we present a variant of the join order learning algorithm that optimally exploits that execution engine. 

\begin{comment}
\begin{algorithm}[t]
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \Comment{Advance tuple pointer $p$ for position $i$ in join order $j$}
\State \Comment{for query $q$, considering tuple offsets $o$.}
\Function{Advance}{$q=R_1\Join\ldots\Join R_m,j,o,p,i$}
\State \Comment{Advance tuple pointer for join order position}
\State $p_{j_i}\gets p_{j_i}+1$
\State \Comment{While index exceeds relation cardinality}
%\While{$p_{j_i}>|q.R_{j_i}|$}
\While{$p_{j_i}>|q.R_{j_i}|$ \textbf{and} $i>0$}
\State $p_{j_i}\gets o_{j_i}$
\State $i\gets i-1$
\State $p_{j_i}\gets p_{j_i}+1$
%\State \Comment{Check if all data processed}
%\If{$i<1$}
%\State \Return{$\langle\mathbf{null},0\rangle$}
%\EndIf
\EndWhile
\State \Return{$\langle p,i\rangle$}
\EndFunction
\vspace{0.15cm}
\State \Comment{Execute join order $j$ for query $q$ starting from}
\State \Comment{tuple pointer $p$ with tuple offsets $o$. Add results}
\State \Comment{to $R$ until time budget $b$ is depleted.}
\Function{Execute}{$q=R_1\Join\ldots\Join R_m,j,o,b,p,R$}
\State $i\gets1$ \Comment{Initialize join order index}
%\State \Comment{Iterate until time budget depleted}
\While{processing time $<b$ \textbf{and} $i>0$}
\State $t\gets\Call{Materialize}{q.R[p_{j_1}]\times\ldots\times q.R[p_{j_i}]}$
\If{$t$ satisfies all newly applicable predicates}
\If{$i=q.n$} \Comment{Is result tuple completed?}
\State $R\gets R\cup\{p\}$ \Comment{Add pointers to result set}
\State $\langle p,i\rangle\gets\Call{Advance}{q,j,o,p,i}$ %\Comment{Advance}
\Else \Comment{Tuple is incomplete}
\State $i\gets i+1$
\EndIf
\Else \Comment{Tuple violates predicates}
\State $\langle p,i\rangle\gets\Call{Advance}{q,j,o,p,i}$ %\Comment{Advance}
\EndIf
\EndWhile
\State \Comment{Join order position 0 indicates termination}
%\State \Return{$(p=\mathbf{null})$}
\State \Return{$(i<1)$}
\EndFunction
\end{algorithmic}
\end{small}
\caption{Auxiliary functions for regret-bounded query evaluation with customized engine.\label{customizedAuxAlg}}
\end{algorithm}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[t]
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
\State \Comment{Advance tuple index in state $s$ for table at position $i$}
\State \Comment{in join order $j$ for query $q$, considering tuple offsets $o$.}
\Function{NextTuple}{$q=R_1\Join\ldots\Join R_m,j,o,s,i$}
\State \Comment{Advance tuple index for join order position}
\State $s_{j_i}\gets s_{j_i}+1$
\State \Comment{While index exceeds relation cardinality}
\While{$s_{j_i}>|R_{j_i}|$ \textbf{and} $i>0$}
\State $s_{j_i}\gets o_{j_i}$
\State $i\gets i-1$
\State $s_{j_i}\gets s_{j_i}+1$
%\State \Comment{Check if all data processed}
%\If{$i<1$}
%\State \Return{$\langle\mathbf{null},0\rangle$}
%\EndIf
\EndWhile
\State \Return{$\langle s,i\rangle$}
\EndFunction
\vspace{0.15cm}
\State \Comment{Execute join order $j$ for query $q$ starting from}
\State \Comment{tuple indices $s$ with tuple offsets $o$. Add results}
\State \Comment{to $R$ until time budget $b$ is depleted.}
\Function{ContinueJoin}{$q=R_1\Join\ldots\Join R_m,j,o,b,s,R$}
\State $i\gets1$ \Comment{Initialize join order index}
\While{processing time $<b$ \textbf{and} $i>0$}
\State $t\gets\Call{Materialize}{R_{j_1}[s_{j_1}]\times\ldots\times R_{j_i}[s_{j_i}]}$
\If{$t$ satisfies all newly applicable predicates}
\If{$i=m$} \Comment{Is result tuple completed?}
\State $R\gets R\cup\{s\}$ \Comment{Add indices to result set}
\State $\langle s,i\rangle\gets\Call{NextTuple}{q,j,o,s,i}$ %\Comment{Advance}
\Else \Comment{Tuple is incomplete}
\State $i\gets i+1$
\EndIf
\Else \Comment{Tuple violates predicates}
\State $\langle s,i\rangle\gets\Call{NextTuple}{q,j,o,s,i}$ %\Comment{Advance}
\EndIf
\EndWhile
\State \Comment{Join order position 0 indicates termination}
%\State \Return{$(p=\mathbf{null})$}
\State \Return{$(i<1)$}
\EndFunction
\end{algorithmic}
\end{small}
\caption{Multi-way join algorithm supporting fast join order switching.\label{customizedAuxAlg}}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{comment}
\begin{algorithm}[t]
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
%\vspace{0.15cm}
\State \Comment{Regret-bounded evaluation of SPJ query $q$,}
\State \Comment{sampling join orders with time budget $b$}
\State \Comment{and using reward function $F_R$.}
\Function{SkinnerC}{$q,b,F_R$}
\State $o\gets \langle 0,\ldots,0\rangle$ \Comment{Initialize tuple offsets}
\State $R\gets\emptyset$ \Comment{Initialize result pointers}
\State $finished\gets\mathbf{false}$ \Comment{Initialize termination flag}
\While{$\neg finished$}
\State \Comment{Choose join order via UCT algorithm}
\State $j\gets\Call{UctChoice}{T}$
\State \Comment{Restore tuple pointers for this join order}
\State $p\gets\Call{RestorePointers}{j}$
\State \Comment{Execute join order for time budget}
\State $finished\gets\Call{ContinueJoin}{q,j,o,b,p,R}$
\State \Comment{Update UCT tree via progress-based rewards}
\State \Call{RewardUpdate}{$T,j,F_R$}
\State \Comment{Backup pointers and update tuple offsets}
\State $o\gets\Call{BackupProgress}{j,p,o}$
\EndWhile
\State \Return{$[\Call{Materialize}{R_1[p_1]\times R_2[p_2]\ldots}|p\in R]$}
\EndFunction
\end{algorithmic}
\end{small}
\caption{Regret-bounded query evaluation using a customized execution engine.\label{customizedAlg}}
\end{algorithm}
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{algorithm}[t]
\renewcommand{\algorithmiccomment}[1]{// #1}
\begin{small}
\begin{algorithmic}[1]
%\vspace{0.15cm}
\State \Comment{Regret-bounded evaluation of SPJ query $q$,}
%\State \Comment{sampling join orders with time budget $b$.}
\State \Comment{length of time slices is restricted by $b$.}
%\State \Comment{and using reward function $F_R$.}
\Function{SkinnerC}{$q=R_1\Join\ldots\Join R_m,b$}
\State \Comment{Apply unary predicates and hashing}
\State $q\gets$\Call{PreprocessingC}{$q$}
%\State $o\gets \langle 0,\ldots,0\rangle$ \Comment{Initialize tuple offsets}
\State $R\gets\emptyset$ \Comment{Initialize result indices}
\State $finished\gets\mathbf{false}$ \Comment{Initialize termination flag}
\While{$\neg finished$}
\State \Comment{Choose join order via UCT algorithm}
\State $j\gets\Call{UctChoice}{T}$
\State \Comment{Restore execution state for this join order}
\State $s\gets\Call{RestoreState}{j,o,S}; s_{prior}\gets s$
\State \Comment{Execute join order during time budget}
\State $finished\gets\Call{ContinueJoin}{q,j,o,b,s,R}$
\State \Comment{Update UCT tree via progress-based rewards}
\State \Call{RewardUpdate}{$T,j,\textproc{Reward}(s-s_{prior},j)$}
\State \Comment{Backup execution state for join order}
\State $\langle o,S\rangle\gets\Call{BackupState}{j,s,o,S}$
\EndWhile
\State \Return{$[\Call{Materialize}{R_1[s_1]\times R_2[s_2]\ldots}|s\in R]$}
\EndFunction
\end{algorithmic}
\end{small}
\caption{Regret-bounded query evaluation using a customized execution engine.\label{customizedAlg}}
\end{algorithm}

Most execution engines are designed for a traditional approach to query evaluation. They assume that a single join order is executed for a given query (after being generated by the optimizer). Learning optimal join orders while executing a query leads to unique requirements on the execution engine. First, we execute many different join orders for the same query, each one only for a short amount of time. Second, we may even execute the same join order multiple times with many interruptions (during which we try different join orders). This specific scenario leads to (at least) three desirable performance properties for the execution engine. First, the execution engine should minimize overheads when switching join orders. Second, the engine should preserve progress achieved for a given join order even if execution is interrupted. Finally, the engine should allow to share achieved progress, to the maximal extent possible, between different join orders as well. The generic approach realizes the latter point only to a limited extend (by discarding batches processed completely by any join order from consideration by other join orders). 

The key towards achieving the first two desiderata (i.e., minimal overhead when switching join orders or interrupting execution) is a mechanism that backs up execution state as completely as possible. Also, restoring prior state when switching join order must be very efficient. By ``state'', we mean the sum of all intermediate results and changes to auxiliary data structures that were achieved during a partial query evaluation for one specific join order. We must keep execution state as small as possible in order to back it up and to restore it efficiently. 

%Note that we use the term ``state'' now in a different sense than before: we do not refer to the state of a Markov Decision Process but to 

Two key ideas enable us to keep execution state small. First, we represent tuples in intermediate results concisely as vectors of tuple indices (each index pointing to one tuple in a base table). Second, we use a multi-way join strategy limiting the number of intermediate result tuples to at most one at any point in time. Next, we discuss both ideas in detail. 

%Note that our design is based on the assumption that large parts of the input data set (all data remaining in the input tables after applying unary predicates) fit into main memory. As discussed before, we believe that current hardware trends, enabling memory-resident databases, facilitate reinforcement learning based query evaluation strategies such as the ones we propose here. 

Traditional execution engines for SPJ queries produce intermediate results that consist of actual tuples (potentially containing many columns with elevated byte sizes). To reduce the size of the execution state, we materialize tuples only on demand. Each tuple, be it a result tuple or a tuple in an intermediate result, is the result of a join between single tuples in a subset of base tables. Hence, whenever possible, we describe tuples simply by an array of tuple indices (whose length is bounded by the number of tables in the input query). We materialize partial tuples (i.e., only the required columns) temporarily to check whether they satisfy applicable predicates or immediately before returning results to the user. To do that efficiently, we assume a column store architecture (allowing quick access to selected columns) and a main-memory resident data set (reducing the penalty of random data access). 

Most traditional execution engines for SPJ queries process join orders by a sequence of binary join operations. This can generate large intermediate results that would become part of the execution state. We avoid that by a multi-way join strategy whose intermediate result size is restricted to at most one tuple. We describe this strategy first for queries with generic predicates. Later, we discuss an extension for queries with equality join predicates based on hashing.

Intuitively, our multi-way join strategy can be understood as a depth-first search for result tuples. Considering input tables in one specific join order, we fix one tuple in a predecessor table before considering tuples in the successor table. We start with the first tuple in the first table (in join order). Next, we select the first tuple in the second table and verify whether all applicable predicates are satisfied. If that is the case, we proceed to considering tuples in the third table. If not, we consider the next tuple in the second table. Once all tuples in the second table have been considered for a fixed tuple in the first table, we ``backtrack'' and advance the tuple indices for the first table by one. Execution ends once all tuples in the first table have been considered. 


\tikzstyle{row}=[anchor=south west, draw=black, fill=blue!50, minimum width=1cm, minimum height=0.5cm]
\tikzstyle{joinFlow}=[thick, -stealth, red, dashed]
\tikzstyle{joinOrder}=[red, font=\small]

\begin{figure}[t]
\begin{tikzpicture}
\foreach \y in {1,2,3,4,5}{
\node[row] (R\y) at (0,0.5*\y) {...};
}
\foreach \y in {1,2,3,4,5}{
\node[row] (S\y) at (2.5,0.5*\y) {...};
}
\foreach \y in {1,2,3,4,5}{
\node[row] (T\y) at (5,0.5*\y) {...};
}

\draw[joinFlow] (S5.west) to[out=180, in=180] (S4.west);
\node[joinOrder] at (2,2.5) {2};
\draw[joinFlow] (S4.west) to[out=180, in=180] (S3.west);
\node[joinOrder] at (2,2) {3};

\draw[joinFlow] (R5.east) to (S5.west);

\node[joinOrder] at (1.75,2.9) {1};
%\draw[joinFlow] (S4.west) to[out=180, in=180] (S2.west);
\node[joinOrder] at (4,2.5) {4};
\draw[joinFlow] (S3.east) to (T5.west);
\draw[joinFlow] (T5.west) to[out=180, in=180] (T4.west);
\node[joinOrder] at (4.7,2.4) {5};
\draw[joinFlow] (T4.west) to[out=180, in=180] (T3.west);
\node[joinOrder] at (4.7,2) {6};
\draw[joinFlow] (T3.west) to[out=180, in=180] (T2.west);
\node[joinOrder] at (4.7,1.5) {7};
\draw[joinFlow] (T2.west) to[out=180, in=180] (T1.west);
\node[joinOrder] at (4.7,1.1) {8};
\draw[joinFlow] (T1.west) to (S3.east);
\node[joinOrder] at (4,1.75) {9};
\draw[joinFlow] (S3.west) to[out=180, in=180] (S2.west);
\node[joinFlow] at (3.75,1.25) {...};
\node[joinOrder] at (2,1.5) {10};
\end{tikzpicture}
\caption{Depth-first multi-way join strategy: we increase the join order index once the first tuple satisfying all applicable predicates is found, we decrease it once all tuples in the current table were considered.\label{joinFigure}}
\end{figure}

\begin{example}
Figure~\ref{joinFigure} illustrates the process for a three-table join. Having fixed a tuple in the left-most table (at the left, we start with the first tuple), the join order index is increased. Next, we find the first tuple in the second table satisfying the join condition with the current tuple in the first table. Having found such a tuple, we increase the join order index again. Now, we iterate over tuples in the third table, adding each tuple combination satisfying all applicable conditions to the result. After all tuples in the last table have been considered, we decrease the join order index and consider the next tuple in the second table.
\end{example}

Algorithm~\ref{customizedAuxAlg} implements that approach. Function~\Call{ContinueJoin}{} realizes the execution strategy described before. For a fixed amount of processing time (we use the number of outer while loop iterations as a proxy in our implementation) or until all input data is processed, it either increases ``depth'' (i.e., join order index $i$) to complete a partial tuple, satisfying all applicable predicates, further, or it advances tuples indices using Function~\Call{NextTuple}{}. The latter function increases the tuple indices for the current join order index or backtracks if the table cardinality is exceeded. Note that the same result tuple might be added multiple times in invocations of the execution engine for different join orders. However, we add tuple index vectors into a result \textit{set}, avoiding duplicate entries (of course, two different tuple index vectors can represent two result tuples with the same values in each column). %As execution time is difficult to measure at extremely fine granularity, we define timeouts in terms of the number of loop iterations in our actual implementation. 

%show pseudo-code for 

We discuss the main function (\Call{SkinnerC}{}) learning optimal join orders using a customized execution engine (see Algorithm~\ref{customizedAlg}). The most apparent difference to the version from Section~\ref{genericSub} is the lack of a dynamic timeout scheme. Instead, we use the same timeout for each invocation of the execution engine. This becomes possible since progress made when executing a specific join order is never lost. By minimizing the size of the execution state, we have enabled an efficient backup and restore mechanism (encapsulated by functions \Call{BackupState}{} and \Call{RestoreState}{} whose pseudo-code we omit) that operates only on a small vector of indices. The number of stored vectors is furthermore proportional to the size of the UCT tree. The fact that we do not lose partial results due to inappropriate timeouts anymore has huge impact from the theoretical perspective (see Section~\ref{analysisSec}) as well as for performance in practice (see Section~\ref{experimentsSec}). Learning overheads are lower than before since we only maintain a single UCT search tree accumulating knowledge from all executions. 

% (represented by parameter $F_R$ in the pseudo-code)

%Multiple choices are valid as long as execution speed correlates with reward. Currently, 

In Section~\ref{genericSub}, we used a binary reward function based on whether the current batch was processed. We do not process data batch-wise anymore and must therefore change the reward function (represented as function~\textproc{Reward} in the pseudo-code which depends on execution state delta and join order). For instance, we can we use as reward the percentage of tuples processed in the left-most table during the last invocation. This function correlates with execution speed and returns values in the range between 0 and 1 (the standard formulas used for selecting actions by the UCT algorithm are optimized for that case~\cite{Kocsis2006}). SkinnerDB uses a slight refinement: we sum over all tuple index deltas, scaling each one down by the product of cardinality values of its associated table and the preceding tables in the current join order. Note that the UCT algorithm averages rewards over multiple invocations of the same join order and keeps exploring (i.e., obtaining a reward of zero for one good join order during a single invocation of the execution engine will not exclude that order from further consideration). 

We have not yet discussed how our approach satisfies the third desiderata (sharing as much progress as possible among different join orders) mentioned at the beginning. We use in fact several techniques to share progress between different join orders (those techniques are encapsulated in Function~\Call{RestoreState}{}). First, we use again offset counters to exclude for each table tuples that have been joined with all other tuples already (vector $o$ in the pseudo-code which is implicitly initialized to one). In contrast to the version from Section~\ref{genericSub}, offsets are not defined at the granularity of data batches but at the granularity of single tuples. This allows for a more fine-grained sharing of progress between different join orders than before. 

Second, we share progress between all join orders with the same prefix. Whenever we restore state for a given join order, we compare execution progress between the current join order and all other orders with the same prefix (iterating over all possible prefix lengths). Comparing execution states $s$ and $s'$ for two join orders $j$ and $j'$ with the same prefix of length $k$ (i.e., the first $k$ tables are identical), the first order is ``ahead'' of the second if there is a join order position $p\leq k$ such that $s_{j_i}\geq s'_{j_i}$ for $i<p$ and $s_{j_p}>s'_{j_p}+1$. In that case, we can ``fast-forward'' execution of the second join order, skipping result tuples that were already generated via the first join order. We do so by executing $j'$ from a merged state $s''$ where $s''_{j'_i}=s_{j'_i}$ for $i<p$, $s''_{j'_p}=s_{j'_p}-1$, and $s''_{j'_i}=o_{j'_i}$ for $i>p$ (since we can only share progress for the common prefix). Progress for different join orders is stored in the data structure represented as $S$ in Algorithm~\ref{customizedAlg}, Function~\textproc{RestoreState} takes care of fast-forwarding (selecting the most advanced execution state among all alternatives).

%Execution progress is measured as the percentage of tuples in the Cartesian product between all input query tables that have been considered either explicitly or implicitly (i.e., by adding tuples satisfying all predicates to the result set and establishing for the others that they are not in the result). Most tuples in the Cartesian product will never be explicitly considered since a predicate is not satisfied before the tuple is completed. Execution progress can be calculated based on the tuple pointers. Denote by $p_i$ the current tuple pointer value for the $i$-th table in a specific join order, by $c_i$ the cardinality of the $i$-th table (and $1\leq p_i\leq c_i$). Execution progress is then calculated by the expression $\sum_i (\prod_{j<i}1/c_j)\cdot (p_i-1)/c_i$. When comparing progress for two join orders with the same prefix until table $t$, we calculate only a partial sum for $i\leq t$. Among all join orders with the same prefix as the current join order, we select the one with maximal progress for the common prefix. We use, for all tables of the common prefix, the pointer values from the maximum-progress order and set the remaining pointers to their minimal values (i.e., the first unprocessed tuple in the corresponding table). 

So far, we described the algorithm for queries with generic predicates. Our actual implementation uses an extended version supporting equality join predicates via hashing. If equality join predicates are present, we create hash tables on all columns subject to equality predicates during pre-processing. Of course, creating hash tables to support all possible join orders creates overheads. However, those overheads are typically small as only tuples satisfying all unary predicates are hashed. We extend Algorithm~\ref{customizedAuxAlg} to benefit from hash tables: instead of incrementing tuple indices always by one (line~5), we ``jump'' directly to the next highest tuple index that satisfies at least all applicable equality predicates with preceding tables in the current join order (this index can be determined efficiently via probing).


%The given algorithm works for generic predicates. It can easily be extended to probe indexes on base tables (or hash tables created during pre-processing) to process equality predicates. Our actual implementation, evaluated in Section~\ref{experimentsSec}, supports hash joins and nested loop joins. It uses hash joins for answering equality predicates. To enable hash joins for all possible join orders, we generate corresponding hash tables in a pre-processing step. However, we only hash tuples which satisfy all unary predicates placed on tables. For typical benchmarks, the number of qualifying tuples is relatively small.

%Note that, in contrast to other main-memory focused execution engines, we do not compile query plans nor do we optimize data access for cache efficiency. This is in line with our overarching goal of favoring robust performance in all cases over peak performance in standard scenarios. 


%no intermediate results are generated and the current state is represented as a small vector.

% TODO: Special treatment of equality predicates, extensions to more complex queries
% Introduce symbols from pseudo-code


==> sectionsTikz/analysis.tex <==
\section{Formal Analysis}
\label{analysisSec}

We prove correctness (see Section~\ref{correctnessSub}), and the regret bounds (see Section~\ref{regretSub}) for all Skinner variants. 

\begin{comment}
We refer to an extended technical report~\cite{Skinners} for termination proofs.

Next, we introduce terminology and assumptions used throughout this section. \textit{Execution Time}, without further qualification, is total time required by SkinnerDB to execute a query. \textit{Regret} refers to the difference between actual and optimal execution time (i.e., using an optimal join order) for a given query. We express regret as a function of $n$, designating execution time of SkinnerDB. Intuitively, we calculate upper bounds on the expected ratio of execution time that was ``wasted''. Note that $n$ is proportional to the number of iterations of the UCT algorithm for a fixed timeout. We assume a query whose properties, such as the number of tables $m$ and the best average reward $r^*$ achievable by an optimal join order (for Skinner-C), are fixed.

Skinner-C and Skinner-H use a variable \textit{Timeout} that restricts execution time spent on a specific data batch using a specific join order. This timeout is determined by the \textit{Timeout Level} via the pyramid timeout scheme described in Section~\ref{genericSub}. Intuitively, the \textit{Number of Timeout Levels} refers to the ``height'' of the colored area in Figure~\ref{budgetFigure}. The execution time \textit{Allocated} to a specific timeout level is the accumulated time spent executing batches with the associated timeout. Intuitively, it corresponds to the ``width'' of a row (associated with a specific timeout level) in Figure~\ref{budgetFigure}. For Skinner-C, the timeout is static and restricts time spent on achieving progress for a fixed join order during a time slice. 

%, the \textit{Timeout Level} specified the \textit{Timeout} per data batch ($2^l$ is the timeout for level $l$). The number of timeout levels refers intuitively to the ``height'' of the colored area in Figure~\ref{budgetFigure}. The execution time allocated to one specific timeout level is the accumulated time spent executing batches with the associated timeout. Intuitively, it corresponds to the ``width'' of a row (associated with a specific timeout level) in Figure~\ref{budgetFigure}.

%, i.e.\ execution time for all data batches is drawn from the same probability distribution . 

We make several simplifying assumptions to facilitate the regret analysis. First, we assume that data batches are homogeneous. This means that, for a fixed join order, execution time per data batch (for Skinner-G and Skinner-H) and evaluation progress (i.e., delta of left-most tuple index per time unit for Skinner-C), is fixed. Second, we study slightly simplified versions of the algorithms from Section~\ref{algorithmSec}. In particular, we assume that offsets are only applied to exclude tuples for the left-most table in the current join order. This means that no progress is shared between join orders that do not share the left-most table. Third, we pessimistically assume that timeouts are completely exploited by SkinnerDB when using sub-optimal join orders (i.e., execution does not finish before the timeout).
\end{comment}

%Without that simplification, even the size of non-batched tables keeps shifting, thereby preventing a stable execution time distribution per batch. 
%we pessimistically assume that no work can be shared between different join orders. Fourth,

%All three Skinner variants are guaranteed to terminate. They terminate once at least one offset reaches its threshold. Offsets increase monotonically and we can show that at least one offset must increase after finite amounts of time. We refer the reader to an extended technical report for detailed termination proofs~\cite{Skinners}.

\begin{comment}
We analyze the three algorithms presented in Section~\ref{algorithmSec}. Skinner-G designates the algorithm that works with any execution engine (see Section~\ref{genericSub}), Skinner-H the hybrid version that mixes learning with traditional query optimization (see Section~\ref{hybridSub}), and Skinner-C the algorithm that is tailored to exploit a customized execution engine (see Section~\ref{customizedSub}). Each of the three algorithms is iterative. We prove termination first. 

%(i.e., that each algorithm is guaranteed to terminate after a finite number of iterations) 

\begin{theorem}
Skinner-G terminates for each input.
\end{theorem}
\begin{proof}
The algorithm terminates once one of the offsets exceeds the number of batches per table (i.e., it terminates once all batches of one table have been processed). An offset is advanced once a batch is processed successfully within the timeout. The processing time per batch is finite and the algorithm tries higher and higher timeouts. Hence, each batch must eventually be processed successfully once the timeout is high enough. The algorithm terminates since the total number of batches is fixed for a given input.
\end{proof}

\begin{theorem}
Skinner-H terminates for each input.
\end{theorem}
\begin{proof}
This follows directly from the previous theorem as the hybrid algorithm uses Skinner-G as a sub-function. Skinner-H terminates once Skinner-G terminates (or before if the traditional optimizer finishes execution first).
\end{proof}

\begin{theorem}
Skinner-C terminates for each input.
\end{theorem}
\begin{proof}
Assume no termination. The number of join orders is finite. Hence, there must be at least one join order for which the execution engine is invoked infinitely often. We consider one such join order in the following. Before each invocation for that join order, we restore tuple pointers to their state after the last invocation for the same join order. Hence, progress is never lost while a join order is suspended. In each iteration, we either increase $i$ or advance the tuple pointers. As $i$ is upper-bounded by the number of tables $m$, tuples pointers must be advanced at least every $m$ iterations. We make the (reasonable) assumption that the execution time budget is sufficient to allow advancing tuple pointers at least once per executor invocation. When advancing tuple pointers, the pointer of a given table is either increased or the pointer of one of its predecessor tables in the join order. As each pointer is upper-bounded by the corresponding table cardinality, the pointer of the left-most table must eventually reach the cardinality bound after which $i$ reaches value zero. But then, the algorithm terminates.
\end{proof}
\end{comment}


\subsection{Correctness}
\label{correctnessSub}

Next, we prove correctness (i.e., that each algorithm produces a correct query result). We distinguish result tuples (tuples from the result relation joining all query tables) from component tuples (tuples taken from a single table). 

\begin{theorem}
Skinner-G produces the correct query result.
\end{theorem}
\begin{proof}
Offsets exclude component tuples from consideration when executing the following joins. We show the following invariant: all result tuples containing excluded component tuples have been generated. This is certainly true at the start where offsets do not exclude any tuples. Offsets are only advanced if batches have been successfully processed. In that case, all newly excluded component tuples have been joined with tuples from all other tables that are not excluded. But excluded tuples can be neglected according to our invariant. The algorithm terminates only after all tuples from one table have been excluded. In that case, all result tuples have been generated. Still, we need to show that no result tuple has been generated more often than with a traditional execution. This is the case since we exclude all component tuples in one table after each successfully processed batch.
\end{proof}

\begin{theorem}
Skinner-H produces the correct query result.
\end{theorem}
\begin{proof}
We assume that executing a query plan produced by the traditional optimizer generates a correct result. The result produced by Skinner-G is correct according to the preceding theorem. This implies that Skinner-H produces a correct result as it returns the result generated by one of the latter two algorithms.
\end{proof}

\begin{theorem}
Skinner-C produces the correct query result.
\end{theorem}
\begin{proof}
Skinner-C does not produce any duplicate result tuples as justified next. Result tuples are materialized only at the very end of the main function. The result set contains tuple index vectors until then. Vectors are unique over all result tuples (as they indicate the component tuples from which they have been formed) and, due to set semantics, no vector will be contained twice in the result. Also, Skinner-C produces each result tuple at least once. This is due to the fact that \textit{i)}~complete tuples are always inserted into the result set, \textit{ii)}~partial tuples (i.e., $i<m$) are completed unless they violate predicates (then they cannot be completed into result tuples), and \textit{iii)}~tuple indices are advanced in a way that covers all combinations of component tuples.
\end{proof}

%Next, we analyze expected regret for all Skinner variants. 

 %An analysis of regret for prior approaches, for traditional query optimizers and for Eddies, can be found in Appendix~\ref{regretApp}.

\begin{comment}
Regret refers to the difference between actual and optimal execution time for a given query. Before we analyze SkinnerDB, we analyze regret bounds of traditional approaches in a worst case. 

Assume a query joining $m$ tables ($m$ is a constant) of cardinality $s$ ($s$ is variable). Tables are connected in a chain via join predicates and one unary predicate is placed on each table. All predicates evaluate to true on each tuple with the exception of the unary predicate on table $t^*$, located on one end of the chain. The latter predicate evaluates to false on each tuple. We consider left-deep join orders that avoid Cartesaian products and measure execution cost by the number of tuples read. Clearly, an optimal plan reads tuples from $t^*$ first and terminates in $O(s)$. If we choose to start from the table at the opposite end of the chain, $t^{-}$, compared to $t^*$, execution cost are in $O(s^{m-1})$. 

If a traditional optimizer~\cite{Selinger1979} cannot reliably estimate the selectivity of predicates (e.g., because they are user-defined functions or because of data skew), we can consider the choice of the first join order table as random. Assuming for instance a uniform distribution, the expected regret is in $O(s^{m-2})$ (based on a $1/m$ chance of selecting $t^-$). Eddies~\cite{Tzoumas2008} fare slightly better in this extreme case. They operate on small data batches (e.g., tuples) and adapt their join order based on feedback. However, Eddies never discard partial results and join them with all remaining tables. If at least one tuple is selected from table $t^-$, there is no other way of completing it into result tuples than consecutive joins with all remaining tables. However, as the associated join predicates are non-selective, execution time will be in $O(s^{m-2})$. Assuming optimistically that Eddies will learn an optimal order after the very first tuple is selected, and assuming a uniform distribution over tables for the initial tuple choice, we have expected regret in $O(s^{m-3})$ for Eddies. 

In the following, we denote by $m$ the number of tables joined by a query ($m$ is fixed) and by $s$ the size of the largest table. Imagine a query connecting all joined tables in a chain via equality join predicates. Further, assume that a unary user-defined function predicate is placed on each table. Assume that all those predicates evaluate to true on each tuple, except for the predicate on table $t^*$. The latter table is located at one end of the chain and its associated unary predicate evaluates always to false. Clearly, an optimal query plan starts joins with table $t^*$, discovering that the query result is empty and terminating in $O(s)$. A left-deep query plan that starts joins at the other end of the chain incurs cost in $O(s^{m-1})$ according to the $C_{out}$ metric. If we start at the other end of the chain, evaluation cost according to the
\end{comment}

%Next, we analyze expected regret for all algorithms (i.e., the expected difference between actual execution time and execution time of an optimal join order). We denote by $n\in\mathbb{N}$ execution time for a specific query (measured according to some atomic time unit such as seconds) and by $m$ the number of joined query tables. The logarithm uses basis two unless noted otherwise.

%Data shuffling in combination with a sufficiently large batch size increase homogeneity in practice. 

%TODO: logarithm of basis 2

\subsection{Regret Bounds}
\label{regretSub}

Regret is the difference between actual and optimal execution time. We denote execution time by $n$ and optimal time by $n^*$. Skinner-G and Skinner-H choose timeout levels (represented by the $y$ axis in Figure~\ref{budgetFigure}) that we denote by $l$. We use the subscript notation (e.g., $n_l$) to denote accumulated execution time spent with a specific timeout level. We study regret for fixed query properties (e.g., the number of joined tables, $m$, or the optimal reward per time slice, $r^*$) for growing amounts of input data (i.e., table size) and execution time. In particular, we assume that execution time, in relation to query size, is large enough to make the impact of transitory regret negligible~\cite{Coquelin2007b}. We focus on regret of the join phase as pre-processing overheads are linear in data and query size (while post-processing overheads are polynomial in query and join result size). We assume that time slices are chosen large enough to make overheads related to learning and join order switching negligible. Specifically for Skinner-G and Skinner-H, we assume that the optimal timeout per time slice applies to all batches. To simplify the analysis, we study slightly simplified versions of the algorithms from Section~\ref{algorithmSec}. In particular, we assume that offsets are only applied to exclude tuples for the left-most table in the current join order. This means that no progress is shared between join orders that do not share the left-most table. For Skinner-C, we assume that the simpler reward function (progress in left-most table only) is used. We base our analysis on the properties of the UCT variant proposed by Kocsis and Szepesvari~\cite{Kocsis2006}.

For a given join order, processing time in SkinnerDB is equivalent to processing time in traditional engines if scaling down the size of the left-most table scales down execution time proportionally (i.e., execution time behaves similarly to the $C_{out}$ cost metric~\cite{Krishnamurthy1986}). If so, the regret bounds apply compared to an optimal traditional query plan execution.

%The processing time of an optimal join order in SkinnerDB is equivalent 

%assume that query properties such as the number of joined tables, $m$, and the optimal reward per time slice, $r^*$, are fixed while the amount of input data is variable. 

%Skinner-C and Skinner-H use a variable \textit{Timeout} that restricts execution time spent on a specific data batch using a specific join order. This timeout is determined by the \textit{Timeout Level} via the pyramid timeout scheme described in Section~\ref{genericSub}. Intuitively, the \textit{Number of Timeout Levels} refers to the ``height'' of the colored area in Figure~\ref{budgetFigure}. The execution time \textit{Allocated} to a specific timeout level is the accumulated time spent executing batches with the associated timeout. Intuitively, it corresponds to the ``width'' of a row (associated with a specific timeout level) in Figure~\ref{budgetFigure}. For Skinner-C, the timeout is static and restricts time spent on achieving progress for a fixed join order during a time slice. 

%SkinnerDB partitions execution time over different join orders and (for Skinner-G and Skinner-H) over different timeout. We use the subscript notation (e.g., $n_l$) to designate execution time over

Before analyzing Skinner-G, we first prove several properties of the pyramid timeout scheme introduced in Section~\ref{genericSub}. 

\begin{lemma}
The number of timeout levels used by Skinner-G is upper-bounded by $\log(n)$.\label{nrLevelsLemma}
\end{lemma}
\begin{proof}
We add a new timeout level $L$, whenever the equation $n_l\geq n_L+2^L$ is satisfied for all $0\leq l<L$ for the first time. As $n_l$ is generally a sum over powers of two ($2^l$), and as $n_L=0$ before $L$ is used for the first time, the latter condition can be tightened to $2^L=n_l$ for all $0\leq l<L$. Hence, we add a new timeout whenever the total execution time so far can be represented as $L\cdot 2^L$ for $L\in\mathbb{N}$. Assuming that $n$ is large, specifically $n>1$, the number of levels grows faster if adding levels whenever execution time can be represented as $2^L$ for $L\in\mathbb{N}$. In that case, the number of levels can be bounded by $\log(n)$ (using the binary logarithm). 
\end{proof}



\begin{lemma}\label{balancedLevelsLemma}
The total amount of execution time allocated to different (already used) timeout levels cannot differ by more than factor two.
\end{lemma}
\begin{proof}
Assume the allocated time differs by more than factor two between two timeout levels, i.e.\ $\exists l_1,l_2:n_{l_1}>2\cdot n_{l_2}$ (and $n_{l_1},n_{l_2}\neq 0$). Consider the situation in which this happens for the first time. Since $\forall i:n_i\geq n_{i+1}$, we must have $n_0>2\cdot n_L$ where $L$ is the largest timeout level used so far. This was not the case previously so we either selected timeout level 0 or a new timeout level $L$ in the last step. If we selected a new timeout level $L$ then it was $n_l\geq n_L+2^L$ for all $0\leq l<L$ which can be tightened to $\forall 0\leq l<L:n_l=2^L$ (exploiting that $n_L=0$ previously and that timeouts are powers of two). Hence, selecting a new timeout cannot increase the maximal ratio of time per level. Assume now that timeout level 0 was selected. Denote by $\delta_{i}=n_i-n_{i+1}$ for $i<L$ the difference in allocated execution time between consecutive levels, before the last selection. It is $\delta_{i}\leq 2^{i}$ since $n_{i}$ is increased in steps of size $2^{i}$ and strictly smaller than $2^{i+1}$ (otherwise, level $i+1$ or a higher one would have been selected). It was $n_0-n_L=\sum_{0\leq i<L}\delta_i\leq \sum_{0\leq i<L}2^i< 2^L$. On the other side, it was $n_L\geq 2^L$ (as $n_L\neq0$ and since $n_L$ is increased in steps of $2^L$). After $n_0$ is increased by one, it is still $n_0\leq 2\cdot n_L$. The initial assumption leads always to a contradiction.
\end{proof}

\begin{comment}
\begin{proof}
We use induction. The statement holds trivially after executing a first batch with a timeout of one time unit (as only a single timeout level was used so far). Assume that the statement holds after executing up to $i$ batches. This implies that it holds after executing $i+1$ batches as shown next. Designate by $l$ the level used for the next batch and by $L$ the maximal level used before. The total amount of allocated execution time (i.e., $w_l$) can only decrease for increasing levels. Hence, the maximal relative difference in total execution time per level is encountered between the largest and smallest level used so far. Therefore, if the new level is neither of them (i.e, $0<l<L$), the maximal relative difference cannot change. If $l=L$ (i.e., $l$ is the maximal level used so far), the relative distance can only decrease. If $l=L+1$ (i.e., we start using a new level), then $w_L=2^{L+1}$ (since we add new levels as soon as possible) and therefore $w_{L+1}=w_L$. The relative distance between $w_{L+1}$ and $w_0$ is bounded by two since the relative distance between $w_L$ and $w_0$ was bounded by two. If the next level is minimal (i.e., $l=0$) then for all higher levels $h>0$ we must have $w_{h}+2^{h}>w_{h-1}$. The latter implies $w_{h-1}-w_{h}\leq 2^{h-1}$ since $w_{h}$ is increased in steps of $2^h$ while $w_{h-1}$ is increased in steps of $2^{h-1}$. Before increasing $w_0$ due to the newly executed batch, the absolute difference between $w_0$ and $w_L$ is bounded by $\sum_{h=1..L}2^{h-1}=2^L-1$. After increasing $w_0$ by one, the absolute difference is bounded by $2^L$. The induction holds since $w_L$ is increased in steps of size $2^L$ and therefore $w_L\geq 2^L$ if it was used. This implies $w_0/w_L\leq 2$.
\end{proof}
\end{comment}

We are now ready to provide worst-case bounds on the expected regret when evaluating queries via Skinner-G.

\begin{theorem}\label{skinnerGtheorem}
Expected execution time regret of Skinner-G is upper-bounded by $(1-1/(\log(n)\cdot m\cdot 4))\cdot n+O(\log(n))$.
\end{theorem}
\begin{proof}
Total execution time $n$ is the sum over execution time components $n_l$ that we spent using timeout level $l$, i.e.\ we have $n=\sum_{0\leq l\leq L}n_l$ where $L+1$ is the number of timeout levels used. It is $L+1\leq \log(n)$ due to Lemma~\ref{nrLevelsLemma} and $\forall l_1,l_2\in L:n_{l_1}\geq n_{l_2}/2$ due to Lemma~\ref{balancedLevelsLemma}. Hence, for any specific timeout level $l$, we have $n_l\geq n/(2\cdot\log(n))$. Denote by $l^*$ the smallest timeout, tried by the pyramid timeout scheme, which allows to process an entire batch using the optimal join order. It is $n_{l^*}\geq n/(2\cdot\log(n))$. We also have $n_{l^*}=n_{l^*,1}+n_{l^*,0}$ where $n_{l^*,1}$ designates time spent executing join orders with timeout level $l^*$ that resulted in reward $1$, $n_{l^*,0}$ designates time for executions with reward $0$. UCT guarantees that expected regret grows as the logarithm in the number of rounds (which, for a fixed timeout level, is proportional to execution time). Hence, $n_{l^*,0}\in O(\log(n_{l^*}))$ and $n_{l^*,1}\geq n_{l^*}-O(\log(n_{l^*}))$. Denote by $b$ the number of batches per table. The optimal algorithm executes $b$ batches with timeout $l^*$ and the optimal join order. Skinner can execute at most $m\cdot b-m+1\in O(m\cdot b)$ batches for timeout $l^*$ before no batches are left for at least one table, terminating execution. Since $l^*$ is the smallest timeout greater than the optimal time per batch, the time per batch consumed by Skinner-G exceeds the optimal time per batch at most by factor 2. Hence, denoting by $n^*$ time for an optimal execution, it is $n^*\geq n_{l^*,1}/(2\cdot m)$, therefore $n^*\geq (n_{l^*}-O(\log(n)))/(2\cdot m)\geq n_{l^*}/(2\cdot m)-O(\log(n))$ (since $m$ is fixed), which implies $n^*\geq n/(4\cdot m\cdot\log(n))-O(\log(n))$. Hence, the regret $n-n^*$ is upper-bounded by $(1-1/(4\cdot m\cdot\log(n)))\cdot n+O(\log(n))$. 
\end{proof}

\begin{comment}
\begin{proof}
We first calculate regret due to inappropriate timeouts. We pessimistically assume that there is one optimal timeout level $l^*$ per batch and that no other timeout leads to significant progress. The number of timeout levels used after $n$ units of execution time is upper-bounded by $\log(n)$ according to Lemma~\ref{nrLevelsLemma}. Also, the time allocated to different levels than $l^*$ exceeds the time dedicated to level $l^*$ at most by factor two (according to Lemma~\ref{balancedLevelsLemma}). Hence, the regret due to inappropriate timeouts is upper-bounded by $(1-1/(\log(n)\cdot 2))\cdot n$. According to the guarantees of the UCT algorithm~\cite{Kocsis2006}, the expected regret due to suboptimal choices (join orders in our case) is upper-bounded by $O(\log(n))$. Variable $n$ designates in general the number of UCT iterations. In our case the number of iterations (specifically for the right timeout) is indeed upper-bounded by the number $n$ of time units spent in execution. Skinner-G stops once all batches of one table are processed. We pessimistically assume that there is one optimal choice for the left-most table. Hence, we count regret for processing batches successfully with the right timeout unless they come from the right table. As the number of batches is the same in all tables, this type of regret is upper-bounded by factor $((m-1)/(\log(n)\cdot m\cdot 2))\cdot n$ for $m$ tables. Finally, even when processing batches from the right table with the right timeout, we may still incur regret by fully exploiting the timeout. This is suboptimal if it is possible to process batches within slightly more than half of the time budget (if the distance is higher, a different timeout level would be optimal). This regret is upper-bounded by $((m-1)/(\log(n)\cdot m\cdot 4))\cdot n$. Adding all regret terms yields the postulated bound.
\end{proof}
\end{comment}

Next, we analyze regret of Skinner-H.

%This bound is derived under extremely pessimistic assumptions. Still, as discussed in the introduction, this regret scales more gracefully in the query size compared to traditional query evaluation methods. The relative upper bound on expected regret grows in the execution time (this can be understood as a growing uncertainty about what timeouts are appropriate as execution time progresses, leading to overheads due to a more diverse set of timeouts). Skinner-C, analyzed latter, improves upon this bound. First, we analyze Skinner-H.

\begin{theorem}
Expected execution time regret of Skinner-H is upper-bounded by $(1-1/(\log(n)\cdot m\cdot 12))\cdot n+O(\log(n))$.
\end{theorem}
\begin{proof}
Denote by $n_O$ and $n_L$ time dedicated to executing the traditional optimizer plan or learned plans respectively. Assuming pessimistically that optimizer plan executions consume all dedicated time without terminating, it is $n_O=\sum_{0\leq l\leq L}2^l$ for a suitable $L\in\mathbb{N}$ at any point. Also, we have $n_L\geq\sum_{0\leq l<L}2^l$ as time is divided between the two approaches. It is $n_L/n\geq (2^L-1)/(2^{L+1}+2^L-2)$ which converges to $1/3$ as $n$ grows. We obtain the postulated bound from Theorem~\ref{skinnerGtheorem} by dividing the ``useful'' (non-regret) part of execution time by factor three.
\end{proof}

%from the fact that Skinner-H balances time between learning and traditional query execution.

%The potential advantage of Skinner-H over Skinner-G is rather shown in the following theorem. 

The following theorem is relevant if traditional query optimization works well (and learning creates overheads).

\begin{theorem}\label{skinnerHtraditionalTheorem}
The maximal execution time regret of Skinner-H compared to traditional query execution is $n\cdot 4/5$.
\end{theorem}
\begin{proof}
Denote by $n^*$ execution time of the plan produced by the traditional optimizer. Hence, Skinner-H terminates at the latest once the timeout for the traditional approach reaches at most $2\cdot n^*$ (since the timeout doubles after each iteration). The accumulated execution time of all prior invocations of the traditional optimizer is upper-bounded by $2\cdot n^*$ as well. At the same time, the time dedicated to learning is upper-bounded by $2\cdot n^*$. Hence, the total regret (i.e., added time compared to $n^*$) is upper-bounded by $n\cdot 4/5$.
\end{proof}

Finally, we analyze expected regret of Skinner-C.

\begin{comment}
\begin{theorem}
Expected execution time regret of Skinner-C is upper-bounded by $(1-1/(m\cdot 2))\cdot n+O(\log(n))$.
\end{theorem}
\begin{proof}[Sketch]
The proof follows closely the one of Theorem~\ref{skinnerGtheorem} with the difference that no regret for inappropriate timeouts is incurred.
\end{proof}
\end{comment}

\begin{theorem}
Expected execution time regret of Skinner-C is upper-bounded by $(1-1/m)\cdot n+O(\log(n))$.\label{skinnerCadditiveTheorem}
\end{theorem}

\begin{comment}
\begin{proof}
Denote by $R$ the cumulative reward realized by Skinner-C during the execution of a specific query. It is $R=\sum_{t\in T}R_t$ where $R_t$ denotes rewards accumulated over time slices in which join orders starting with table $t\in T$ were selected. Reward is calculated as the relative tuple index delta in the left-most table (i.e., tuple index delta in left-most table divided by table cardinality). Hence, execution terminates whenever there is a table $t$ such that $R_t=1$. Skinner-C may accumulate more reward than necessary, when partitioning efforts over join orders with different start tables. The reward that can be collected before termination is however bounded by $R\leq m$. Skinner-C may lose time due to sub-optimal choices. However, it achieves near-optimal average rewards (and therefore near-optimal evaluation progress) based on the UCT guarantees~\cite{Kocsis2006}. More precisely, it is $r^*-r\in O(\log(n)/n)$ where $r$ is the expected average reward achieved by Skinner-C, $r^*$ the optimal average reward, and $n$ denotes execution time of Skinner-C (which is proportional to the number of UCT rounds as we use a fixed timeout). We calculate bounds on the optimal execution time $n^*$, required for collecting a reward of at least $R/m$ with optimal average reward per round $r^*$. It is $n^*\leq n\cdot r/(m\cdot r^*)=n\cdot (r^*-O(\log(n)/n))/(m\cdot r^*)$. From that, we obtain bounds on expected regret $n-n^*\leq n\cdot(1-1/m\cdot (r^*-O(\log(n)/n))/r^*)=n\cdot (1-1/m)+O(\log(n))$ (since $r^*$ is considered a constant). 
\end{proof}
\end{comment}

\begin{proof}
Regret is the difference between optimal execution time, $n^*$, and actual time, $n$. It is $n-n^*=n\cdot(1-n^*/n)$. Denote by $R$ the total reward achieved by Skinner-C during query execution and by $r$ the average reward per time slice. It is $n=R/r$. Denote by $r^*$ the optimal reward per time slice. Reward is calculated as the relative tuple index delta in the left-most table (i.e., tuple index delta in left-most table divided by table cardinality). An optimal execution always uses the same join order and therefore terminates once the accumulated reward reaches one. Hence, we obtain $n^*=1/r^*$. We can rewrite regret as $n-n^*=n\cdot(1-(1/r^*)/(R/r))=n\cdot (1-r/(R\cdot r^*))$. The difference between expected reward and optimal reward is bounded as $r^*-r\in O(\log(n)/n)$~\cite{Kocsis2006}. Substituting $r$ by $r^*-(r^*-r)$, we can upper-bound regret by $n\cdot(1-1/R)+O(\log(n))$. Denote by $R_t\leq R$ rewards accumulated over time slices in which join orders starting with table $t\in T$ were selected. Skinner-C terminates whenever $R_t=1$ for any $t\in T$. Hence, we obtain $R\leq m$ and $n\cdot(1-1/m)+O(\log(n))$ as upper bound on expected regret.
\end{proof}

\begin{comment}
\begin{proof}
 Denote by $n_R$ the time required by an optimal policy to reach the same reward $R$ as Skinner-C (assuming optimistically that maximal rewards can be obtained over the whole execution period). It is $n_R=R/r^*=n\cdot r/r^*$ and therefore $n-n_r=n\cdot r^*/r^*-n\cdot (r^*-O(\log(n)/n)/r^*=O(\log(n))/r^*\in O(\log(n))$ (since we consider $r^*$ as constant). %n\cdot(r^*-r^*+O(\log(n)/n))/r^*=

Denote by $n_R$ an optimistic estimate of the time required by an optimal policy to reach reward $R$: it is $n_R\cdot r^*=R$ and therefore $n_R=R/r^*$, hence $n-n_R=R/r-R/r^*=R\cdot(1/r+1/(r+O(\log(n))$

 $n_R\cdot(r+O(\log(n)/n))=R$. Since $n\cdot r=R$, it is $n_R\cdot (r+O(\log(n)/n))=n\cdot r$, hence 

Denote by $n$ execution time of Skinner-C for one specific query. 
Skinner-C uses the relative delta in the left-most tuple index as reward function (i.e., tuple index delta divided by table cardinality). This links reward to evaluation progress. Execution terminates, at the latest, once the reward accumulated for join orders starting with one specific table reaches 1. Denote execution time of Skinner-C by $n$ (which is proportional to the number of UCT rounds since we used a fixed timeout) for a given query. , the expected difference between average reward $r$ of Skinner-C and optimal average reward $r^*$ is upper-bounded by $O(\log(n)/n)$. Furthermore, Skinner-C might partition its efforts over join orders starting with different tables. The optimal approach 
\end{proof}
\end{comment}

Instead of the (additive) difference between expected and optimal execution time, we can also consider the ratio.

\begin{theorem}
The ratio of expected to optimal execution time for Skinner-C is upper-bounded and that bound converges to $m$ as $n$ grows. 
\end{theorem}
\begin{proof}
Let $a=n-n^*$ be additive regret, i.e.\ the difference between actual and optimal execution time. It is $n^*=n-a$ and, as $a\leq (1-1/m)\cdot n+O(\log(n))$ due to Theorem~\ref{skinnerCadditiveTheorem}, it is $n^*\geq n-(1-1/m)\cdot n-O(\log(n))=n/m-O(\log n)=n\cdot(1/m-O(\log(n))/n)$. Optimal execution time is therefore lower-bounded by a term that converges to $n/m$ as $n$ grows. Then, the ratio $n/n^*$ is upper-bounded by $m$.
\end{proof}

% $n/n^*=n/(n-a)$ $n-a\geq n-(1-1/m)\cdot n-O(\log(n))=n/m-O(\log n)$ $n/n^*\leq n/(n/m-O(\log(n)))=n/(n\cdot (1/m-O(\log(n)/n))$ which converges towards $m$.


%We have so far calculated regret with regards to the best ``batched'' execution (i.e., not with regards to cost incurred by a traditional execution engine performing binary joins without batching). We finally discuss the relationship between the best batched and the best traditional execution. In particular, we are interested in conditions under which total batched execution cost is comparable to non-batched execution cost. Intuitively, this is the case if execution cost for a given join order scales down gracefully in the size of the left-most table (e.g., using for the left-most table a sample that is ten times smaller than the original table reduces execution time by factor 10). Similar assumptions with regards to cost scaling are common in prior work~\cite{Dutt2017, Trummer2016paoq}. We assume that the sizes of all intermediate results scale down proportionally to the size of the left-most table for a fixed join order. Then, the number of intermediate result tuples generated during execution scales down proportionally. Also, the number of predicate evaluations (except for unary predicates which can be evaluated in a pre-processing step) scales down proportionally. Similarly, the number of lookup operations in indexes on base tables (or in hash tables created during pre-processing) scales down proportionally. On the other side, the total amount of data read does not scale down proportionally (since non-indexed base tables must be read for each batch). In summary, if pure data access is relatively cheap compared to lookups, predicate evaluations, and tuple generations (e.g., because data is read from main memory or predicates are expensive to evaluate), batched execution cost is comparable to non-batched execution cost. Then, the regret bounds outlined before apply to execution cost of a traditional execution engine as well.

\begin{comment}

%The total amount of allocated execution time (i.e., $w_l$) can only decrease for increasing levels. Hence, if the $0<l<L$ (i.e., the newly chosen level is neither minimal nor used for the first time) then 

%Consider an arbitrary but fixed level $l\in\mathbb{N}$. Due to the definition of the timeout scheme, we always have $w_l\geq w_{l+1}$. In addition, we have $w_l-w_{l+1}\leq 2^{l+1}$. The latter can be seen as follows: $w_l$ is incremented in steps of size $2^l$ while $w_{l+1}$ is incremented in steps of $w^{l+1}$. Hence, if $w_l-w_{l+1}> 2^{l+1}$ there would have to be a prior point at which $w_l-w_{l+1}=2^{l+1}$. From that point on, $w_{l+1}$ would be incremented before $w_l$ is incremented for the next time (since the timeout scheme always chooses the largest level for which a balanced allocation is possible), hence the distance shrinks again. This means that the difference $w_L-w_l$ is bounded by the term $\sum_{i=l+1..L}2^i<$

%Assume there are two levels $l$ and $L$ with $l<L$, $w_l>0$ and $w_L>0$, and $w_l>2\cdot w_L$. We must have $l<L$ due to the definition of the timeout scheme. Note that $w_l$ is increased in steps of size $2^l$ while $w_L$ is increased in steps of size $2^L$ and $2^L>2^l$. Hence, If $w_l>2\cdot w_L$, there must have been a situation previously in which $w_l=2\cdot w_L$. In that situation, a higher level than $l$ would have been chosen 


%We have $w_l\geq w_L$ for all $l<L$ due to the definition of the timeout scheme. Hence, whenever $w_L\geq w_{L+1}+2^{L+1}$, we also have $w_l\geq w_{L+1}+2^{L+1}$ for each $l<L$. In that case, the next timeout 

%Consider an arbitrary but fixed level $L\in\mathbb{N}$. Variable $w_L$ designates the total execution time allocated to level $L$. Assume there was another level $l\neq L$ with $w_l>0$ and $w_l/w_L>2$ or $w_L/w_l>2$. If $l<L$ then we must have $w_l\geq w_L$. Assume $w_l>2\cdot w_L$ which also implies $w_{\widetilde{l}}>2\cdot w_L$ for all $\widetilde{l}<l$. 

$n$ is total execution time according to some atomic time unit

Assume that completely balanced over different timeouts to simplify the following proofs (relaxation is relatively straight-forward)

Assume that processing time per batch is homogeneous plus random noise (current proof sufficient for the latter?), can be achieved by shuffling and choosing batches large enough

Simplified version of the algorithm to simplify proofs

TODO: coupon collector, pyramid

Proof via induction concerning balancing of pyramid scheme?

\begin{equation}
R=R_T+R_P+R_F+R_J
\end{equation}

\begin{lemma}
Regret due to inappropriate timeouts is upper-bounded by $n\cdot(\log(n)-1)/\log(n)$.\label{timeoutRegretLemma}
\end{lemma}
\begin{proof}
We use different timeouts to process data batches. The number of different timeouts grows logarithmically in the total execution time. Further, our pyramid scheme ensures that execution time allocations are balanced over different timeouts (i.e, the total time spent in executing batches with larger timeouts does not exceed the total time spent in executing batches with smaller timeouts). Hence, the execution time allocated to one specific timeout is bounded by $n/\log(n)$ time units. We assume that there is one optimal timeout per batch that is minimal among all timeouts allowing to process batches reliably. We (very pessimistically) assume that invocations with smaller timeouts generally do not allow to make progress. We also assume that invocations with larger timeouts waste a disproportional amount of processing time to make negligible progress. Still, regret is bounded by the ratio of invocations for sub-optimal timeouts which is $n\cdot(\log(n)-1)/\log(n)$.
\end{proof}

\begin{lemma}
Expected regret due to processing failures is upper-bounded by $O(\log(n/\log(n)))$.
\end{lemma}
\begin{proof}
Following the proof of the previous lemma, the execution time fraction allocated to the optimal timeout per batch is $n/\log(n)$. As we use a minimal timeout of one time unit, the number of batches processed with that optimal timeout is upper-bounded by the same number. We use the UCT algorithm to find join orders that process batches reliably with that timeout. Each processed batch corresponds to one sample of the UCT algorithm. Following the proof by Kocsis and Szepesv\`ari~\cite{Kocsis2006}, expected regret is bounded by $O(\log(n/\log(n)))$. It is $\log((n)/\log(n))=\log(n)-\log(\log(n))\in O(\log(n))$.
\end{proof}

\begin{lemma}
Regret due to sub-optimal choice of the first join table is upper-bounded by $((m-1)/m)\cdot n/\log(n)$.
\end{lemma}
\begin{proof}
Following again the proof of Lemma~\ref{timeoutRegretLemma}, the execution time fraction allocated to the optimal timeout per batch is $n/\log(n)$. The number of successfully processed batches using that timeout is trivially upper-bounded by the same number. Not all successfully processed batches share the same left-most table with the optimal join order. As the number of batches is the same over all tables, the number of batches processed from sub-optimal tables is for each single table strictly upper-bounded by the number of batches processed in the optimal table (after processing finishes). Hence, the total number of batches processed for join orders starting with the wrong table is upper bounded by factor $(m-1)/m$.
\end{proof}

% In a worst-case scenario, progress achieved by such join orders is of negligible benefit for join orders starting with the optimal table (e.g., if processing cost is concentrated on the first join such that the size of the following intermediate results matters less). 

\begin{lemma}
Regret due to a sub-optimal join order after the first table is upper-bounded by $1/(2\cdot m)\cdot n/\log(n)$
\end{lemma}
\begin{proof}
We choose timeouts per batch from a geometric progression. The optimal timeout in that progression may exceed the optimal timeout by up to factor two. As the reward function depends only on whether or not a batch was processed successfully, the algorithm does not distinguish between join orders whose processing cost differs by up to factor two. In the worst case, we loose half of the processing time allocated to the optimal timeout per batch and to the optimal left-most table due to such sub-optimal choices.
\end{proof}

\begin{theorem}
Expected regret of Skinner-NI is bounded by $n\cdot(1-1/(2\cdot m\cdot\log(n)))+O(\log(n))$.
\end{theorem}

\begin{corollary}
The actual
$O(n-2\cdot m\cdot\log(n)\cdot\log(n)/(2\cdot m\cdot\log(n))$
\end{corollary}

Link to optimal processing time of original plan under specific assumptions

Proof sketch for Skinner-C
\end{comment}

==> sectionsTikz/conclusion.tex <==

We introduce a new quality criterion for query evaluation strategies: we consider the distance (either difference or ratio) between expected execution time and processing time for an optimal join order. We designed several query evaluation strategies, based on reinforcement learning, that are optimized for that criterion. We implemented them in SkinnerDB, leading to the following insights. First, regret-bounded query evaluation leads to robust performance even for difficult queries, given enough data to process. Second, performance gains by robust join ordering can outweigh learning overheads for benchmarks on real data. Third, actual performance is significantly better than our theoretical worst-case guarantees. Fourth, to realize the full potential of our approach, an (in-query) learning-based optimizer must be paired with a specialized execution engine. 

%We summarize our experimental results. 

%Third, realizing the full potential of regret-bounded query evaluation requires an execution engine that is specialized for the translates into robust performance in face of correlated data we are able to find execution strategies that 

%We use reinforcement learning to learn optimal join orders during the execution of a query. We have shown experimentally that reliable optimization is sometimes more important than maximally efficient implementation of single operators. In our future work, we plan to parallelize join order execution, to extend our approach to bushy pans (requiring changes to execution engine and optimizer at the same time), and to integrate data compression methods. The appendix contains many more experimental results.

%Under simplifying assumptions, we are able to translate regret bounds in reinforcement learning to bounds on execution overheads. 

%Our approach can work in a completely non-intrusive manner on top of existing DBMS. This leads to speedups of orders of magnitude for difficult-to-optimize queries (containing for instance UDFs or correlated predicates) while we bound overheads compared to the original optimizer. An integrated approach, combining learning with a specialized execution engine, works best on difficult-to-optimize queries. 

==> sectionsTikz/experiments.tex <==
\pgfplotsset{
    discard if not/.style 2 args={
        x filter/.code={
            \edef\tempa{\thisrowno{#1}}
            \edef\tempb{#2}
            \ifx\tempa\tempb
            \else
                \def\pgfmathresult{inf}
            \fi
        }
    }
}

% Parameters: File name, timeout
\def\addChainPlotTime#1#2{
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmctsS}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINEddy}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINOpt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINReopt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgres}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgresMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgresMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptive}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptiveMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptiveMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmonet}] {#1};
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},#2) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},#2);
}

% Parameters: File name, timeout
\def\addStarPlotTime#1#2{
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmctsS}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAREddy}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAROpt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARReopt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgres}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgresMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgresMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptive}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptiveMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptiveMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmonet}] {#1};
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},#2) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},#2);
}

% and compare to several baselines

We evaluate the performance of SkinnerDB experimentally. Additional results can be found in the appendix. %We implemented the adaptive processing strategies described in Section~\ref{algorithmSec} in a novel DBMS called SkinnerDB. 

\subsection{Experimental Setup}

%The first two SkinnerDB variants run on top of existing database systems. 

Skinner-G(X) is the generic Skinner version (see Section~\ref{genericSub}) on top of database system X in the following. Skinner-H(X) is the hybrid version on system X. We execute Skinner on top of MonetDB (Database Server Toolkit v1.1 (Mar2018-SP1))~\cite{Boncz2008} and Postgres (version 9.5.14)~\cite{Postgres}. We use different mechanisms to force join orders for those systems. Postgres has dedicated knobs to force join orders. For MonetDB, we ``brute-force'' join orders by executing each join as a separate query, generating multiple intermediate result tables. Skinner-C, described in Section~\ref{customizedSub}, uses a specialized execution engine. We set $w=\sqrt{2}$ in the UCT formula for Skinner-G and Skinner-H and $w=10^{-6}$ for Skinner-C. Unless noted otherwise, we use a timeout of $b=500$ loop iterations for Skinner-C (i.e., thousands or even tens of thousands of join order switches per second). For Skinner-G and -H, we must use much higher timeouts, starting from one second. All SkinnerDB-specific components are implemented in Java. Our current Skinner-C version only allows to parallelize the pre-processing step. Extending our approach to parallel join processing is part of our future work. To separate speedups due to join ordering from speedups due to parallelization, we compare a subset of baselines in single- as well as in  multi-threaded mode. The following experiments are executed on a Dell PowerEdge R640 server with 2 Intel Xeon 2.3~GHz CPUs and 256~GB of RAM. 

%For Skinner-G and -H, a much coarser timeout of (initially) one second works better (due to high switching overheads). 



\subsection{Performance on Join Order Benchmark}

\begin{table}[t]
\caption{Performance of query evaluation methods on the join order benchmark - single-threaded.\label{jobTable}}
\begin{tabular}{p{1.75cm}p{1.25cm}p{1.25cm}p{1.25cm}p{1.25cm}}
\toprule[1pt]
\textbf{Approach} & \textbf{Total Time} & \textbf{Total Card.\ } & \textbf{Max.\ Time} & \textbf{Max.\ Card.\ }\\
\midrule[1pt]
Skinner-C & 183 & 112M & 9 & 18M \\
\midrule
Postgres & 726 & 681M & 59 & 177M \\
S-G(PG) & 13,348 & N/A & 840 & N/A \\
S-H(PG) & 2,658 & N/A & 234 & N/A \\
\midrule
MonetDB & 986 & 2,971M & 409 & 1,186M \\
S-G(MDB) & 1,852 & N/A & 308 & N/A\\
S-H(MDB) & 762 & N/A & 114 & N/A\\
\bottomrule[1pt]
\end{tabular}
\end{table}



\begin{table}[t]
\caption{Performance of query evaluation methods on the join order benchmark - multi-threaded.\label{jobTableMT}}
\begin{tabular}{p{1.75cm}p{1.25cm}p{1.25cm}p{1.25cm}p{1.25cm}}
\toprule[1pt]
\textbf{Approach} & \textbf{Total Time} & \textbf{Total Card.\ } & \textbf{Max.\ Time} & \textbf{Max.\ Card.\ }\\
\midrule[1pt]
Skinner-C & 135 & 112M & 7 & 18M \\
%Skinner-R & 1,746,468 & N/A & 331736 & N/A \\
%\midrule
%Postgres & & & & \\
%S-G(PG) & N/A & & & \\
%S-H(PG) & & & & \\
\midrule
MonetDB & 105 & 2,971M & 26 & 1,186M \\
S-G(MDB) & 1,450 & N/A & 68 & N/A \\
S-H(MDB) &345 & N/A & 86 & N/A \\
\bottomrule[1pt]
\end{tabular}
\end{table}

We evaluate approaches on the join order benchmark~\cite{Gubichev2015}, a benchmark on real, correlated data. We follow the advice of the paper authors and explicitly prevent Postgres from choosing bad plans involving nested loops joins. Tables~\ref{jobTable} and \ref{jobTableMT} compare different baselines in single-threaded and for Skinner, and MonetDB, in multi-threaded mode (our server runs Postgres~9.5 which is not multi-threaded). We compare approaches by total and maximal (per query) execution time (in seconds). Also, we calculate the accumulated intermediate result cardinality of executed query plans. This metric is a measure of optimizer quality that is independent of the execution engine. Note that we cannot reliably measure cardinality for Skinner-G and Skinner-H since we cannot know which results were generated by the underlying execution engine before the timeout.

Clearly, Skinner-C performs best for single-threaded performance. Also, its speedups are correlated with significant reductions in intermediate result cardinality values. As verified in more detail later, this suggests join order quality as the reason. For multi-threaded execution on a server with 24 cores, MonetDB slightly beats SkinnerDB. Note that our system is implemented in Java and does not currently parallelize the join execution phase. 

When it comes to Skinner on top of existing databases, the results are mixed. For Postgres, we are unable to achieve speedups in this scenario (as shown in the appendix, there are cases involving user-defined predicates where speedups are however possible). Postgres exploits memory less aggressively than MonetDB, making it more likely to read data from disk (which makes join order switching expensive). For single-threaded MonetDB, however, the hybrid version  reduces total execution time by nearly 25\% and maximal time per query by factor four, compared to the original system. This is due to just a few queries where the original optimizer selects highly suboptimal plans. 



\begin{table}[t]
\caption{Performance of join orders in different execution engines for join order benchmark - single threaded.\label{joinOrdersTable}}
\begin{tabular}{p{1.5cm}p{1.5cm}p{1.75cm}p{1.75cm}}
\toprule[1pt]
\textbf{Engine} & \textbf{Order} & \textbf{Total Time} & \textbf{Max.\ Time} \\
\midrule[1pt]
Skinner & Skinner & 183 & 9 \\
& Optimal & 180 & 7 \\
\midrule
Postgres & Original & 726 & 59 \\
& Skinner & 567 & 14 \\
& Optimal & 555 & 14 \\
\midrule
MonetDB & Original & 986 & 409 \\
& Skinner & 138 & 7 \\
& Optimal & 134 & 6 \\
\bottomrule[1pt]
\end{tabular}
\end{table}


\begin{table}[t]
\caption{Performance of join orders in different execution engines for join order benchmark - multi-threaded.\label{joinOrdersTableMT}}
\begin{tabular}{p{1.5cm}p{1.5cm}p{1.75cm}p{1.75cm}}
\toprule[1pt]
\textbf{Engine} & \textbf{Order} & \textbf{Total Time} & \textbf{Max.\ Time} \\
\midrule[1pt]
Skinner & Skinner & 135 & 7 \\
& Optimal & 129 & 7 \\
%\midrule
%Postgres & Original & & \\
%& Skinner & & \\
%& Optimal & & \\
\midrule
MonetDB & Original & 105 & 26 \\
& Skinner & 53 & 2.7 \\
& Optimal & 51 & 2.3  \\
\bottomrule[1pt]
\end{tabular}
\end{table}

To verify whether Skinner-C wins because of better join orders, we executed final join orders selected by Skinner-C in the other systems. We also used optimal join orders, calculated according to the $C_{out}$ metric. Tables~\ref{joinOrdersTable} and \ref{joinOrdersTableMT} show that Skinner's join orders improve performance uniformly, compared to the original optimizer. Also, Skinner's execution time is very close to the optimal order, proving the theoretical guarantees from the last section pessimistic. 

\subsection{Further Analysis}

\begin{table}
\caption{Impact of replacing reinforcement learning by randomization.\label{randomizationTable}}
\begin{tabular}{llll}
\toprule[1pt]
\textbf{Engine} & \textbf{Optimizer} & \textbf{Time} & \textbf{Max.\ Time}\\
\midrule[1pt]
Skinner-C & Original & 182 & 9 \\
& Random & 2,268 & 332 \\
\midrule
Skinner-H(PG) & Original & 2,658 & 234 \\
& Random & 3,615 & 250 \\
\midrule
Skinner-H(MDB) & Original & 761 & 114 \\
& Random & $\geq$ 5,743 & $\geq$ 3,600 \\
\bottomrule[1pt]
\end{tabular}
\end{table}

\begin{table}[t]
\caption{Impact of SkinnerDB features.\label{featuresTable}}
\begin{tabular}{p{4.8cm}p{1.25cm}p{1.25cm}}
\toprule[1pt]
\textbf{Enabled Features} & \textbf{Total Time} & \textbf{Max.\ Time} \\
\midrule[1pt]
indexes, parallelization, learning & 135 & 7 \\
parallelization, learning & 162 & 9  \\
learning & 185 & 9 \\
none & 2,268 & 332 \\
\bottomrule[1pt]
\end{tabular}
\end{table}

We experiment with different variants of SkinnerDB. First of all, we compare learning-based selection against randomized selection. Table~\ref{randomizationTable} shows the performance penalty for randomized selection. Clearly, join order learning is crucial for performance. In Table~\ref{featuresTable}, we compare the impact of randomization to the impact of parallelizing pre-processing and adding hash indices on all join columns (which SkinnerDB exploits if the corresponding table is not used in pre-processing). Clearly, join order learning is by far the most performance-relevant feature of SkinnerDB.


\begin{figure}[t]
\subfigure[MonetDB spends most time executing a few expensive queries.]{
\begin{tikzpicture}
\begin{axis}[xlabel={Queries}, ylabel={Run Time (\%)}, width=4cm, ylabel near ticks, xlabel near ticks, legend entries={ Skinner, MonetDB}, legend pos=south east, legend style={font=\scriptsize}, ymajorgrids]
\addplot table[x index=0, y index=3, col sep=tab] {plots/runTimeSkinner.txt};
\addplot table[x index=0, y index=3, col sep=tab] {plots/runTimeSkew.txt};
\end{axis}
\end{tikzpicture}
}
\subfigure[SkinnerDB realizes high speedup for two expensive queries.]{
\begin{tikzpicture}
\begin{axis}[xlabel={MonetDB Time (ms)}, ylabel={Speedup}, width=4cm, ylabel near ticks, xlabel near ticks, xmode=log, ymode=log, ymajorgrids]
\addplot[scatter, only marks] table[x index=0, y index=2, col sep=tab] {plots/speedupSkew.txt};
\end{axis}
\end{tikzpicture}
}
\caption{Analyzing the source of SkinnerDB's speedups compared to MonetDB.\label{monetVsSkinnerFig}}
\end{figure}
% RAM: 16 GB
%              CPU: Intel® Core™ i5-7200U CPU @ 2.50GHz 2.71GHz
%              OS: Windows 10 Home 64-bit Operating System


We analyze in more detail where the speedups compared to MonetDB come from (all results refer to single-threaded mode). Figure~\ref{monetVsSkinnerFig} shows on the left hand side the percentage of execution time, spent on the top-k most expensive queries (x axis). MonetDB spends the majority of execution time executing two queries with highly sub-optimal join orders (we reached out to the MonetDB team to make sure that no straight-forward optimizations remove the problem). On the right side, we draw speedups realized by Skinner versus MonetDB's query execution time. MonetDB is actually faster for most queries while SkinnerDB has highest speedups for the two most expensive queries. Since those queries account for a large percentage of total execution time, Skinner-C outperforms MonetDB in single-threaded mode. 

\begin{figure}[t]
\subfigure[The growth of the search tree slows down over time.]{
\begin{tikzpicture}
\begin{axis}[xlabel={Time (scaled)}, ylabel={\#Nodes (scaled)}, width=4cm, ylabel near ticks, xlabel near ticks, ymajorgrids]
%\addplot table[x index=0, y index=2, col sep=tab] {plots/speedupSkew.txt};
\addplot coordinates {(0.25,0.65) (0.5, 0.85) (0.75,0.95) (1,1)};
\end{axis}
\end{tikzpicture}
}
\subfigure[SkinnerDB spends most time executing one or two join orders.]{
\begin{tikzpicture}
\begin{axis}[xlabel={Top-k Orders}, ylabel={Selections (\%)}, width=4cm, ylabel near ticks, xlabel near ticks, legend entries={T:500, T:10}, legend pos=south east, legend style={font=\scriptsize}, xtick=data, ymajorgrids]
\addplot coordinates {(1,0.45) (2,0.65) (3,0.72) (4,0.79) (5,0.81)};
\addplot coordinates {(1,0.65) (2,0.82) (3,0.88) (4,0.89) (5,0.90)};
%\addplot coordinates {(1,0.46) (2,0.57) (3,0.62) (4,0.65) (5,0.68)};
%\addplot coordinates {(1,0.63) (2,0.71) (3,0.74) (4,0.76) (5,0.77)};
\end{axis}
\end{tikzpicture}
}
\caption{Analysis of convergence of SkinnerDB.\label{convergenceFig}}
\end{figure}

Figure~\ref{convergenceFig} analyzes convergence of Skinner-C to optimal join orders. On the left side, we show that the growth of the search tree slows as execution progresses (a first indication of convergence). On the right side, we show that Skinner-C executes one (with a timeout of $b=10$ per time slice) or two (with a timeout of $b=500$, allowing less iterations for convergence) join orders for most of the time.

\begin{figure}[t]
\subfigure[Search tree size is correlated with query size.\label{uctMemFig}]{
\begin{tikzpicture}
\begin{axis}[xlabel={\# Joined Tables}, ylabel={\#Nodes}, width=4cm, ylabel near ticks, xlabel near ticks, ymajorgrids, xmode=linear, ymode=log]
\addplot[scatter, only marks] table[x index=0, y index=8, col sep=tab] {plots/treeGrowth.txt};
\end{axis}
\end{tikzpicture}
}
\subfigure[Size of join order progress tracker tree.\label{trackerMemFig}]{
\begin{tikzpicture}
\begin{axis}[xlabel={\# Joined Tables}, ylabel={\#Nodes}, width=4cm, ylabel near ticks, xlabel near ticks, ymajorgrids, xmode=linear, ymode=log]
\addplot[scatter, only marks] table[x index=0, y index=11, col sep=tab] {plots/treeGrowth.txt};
\end{axis}
\end{tikzpicture}
}
\subfigure[Size of final result tuple indices.\label{finalMemFig}]{
\begin{tikzpicture}
\begin{axis}[xlabel={\# Joined Tables}, ylabel={\#Size}, width=4cm, ylabel near ticks, xlabel near ticks, ymajorgrids, xmode=linear, ymode=log]
\addplot[scatter, only marks] table[x index=0, y index=12, col sep=tab] {plots/treeGrowth.txt};
\end{axis}
\end{tikzpicture}
}
\subfigure[Combined size of intermediate results, progress, and tree.\label{allMemFig}]{
\begin{tikzpicture}
\begin{axis}[xlabel={\# Joined Tables}, ylabel={All Data (GB)}, width=4cm, ylabel near ticks, xlabel near ticks, ymajorgrids, xmode=linear, ymode=log]
\addplot[scatter, only marks] table[x index=0, y index=9, col sep=tab] {plots/treeGrowth.txt};
\end{axis}
\end{tikzpicture}
}
\caption{Memory consumption of SkinnerDB.\label{memoryFigure}}
\end{figure}

Finally, we analyze memory consumption of Skinner-C. Compared to traditional systems, Skinner-C maintains several additional, auxiliary data structures. First, it keeps the UCT search tree. Second, it maintains a tree associating each join order to the last execution state (one tuple index for each base table). Third, it must keep the tuple vectors of all join result tuples in a hash table to eliminate duplicates from different join orders. On the other side, Skinner-C does not maintain any intermediate results as opposed to other systems (due to depth-first multiway join execution). Figure~\ref{memoryFigure} shows the maximal sizes of the aforementioned data structures during query executions as a function of query size. Storing result tuple index vectors (Figure~\ref{finalMemFig}) has dominant space complexity, followed by the progress tracker, and the UCT search tree. Overall, memory consumption is not excessive compared to traditional execution engines.


\begin{comment}
\begin{figure}
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 1, x descriptions at=edge bottom}, width=8.5cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Eddy,Reoptimizer,Postgres,S-G(Postgres),S-H(Postgres),Com-DB,S-G(Com-DB),S-H(Com-DB)}, legend columns=3, legend to name=b2millisLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks]
\nextgroupplot[bar width=3pt, title={UDF Equality Predicates, 250 tuples/table}, xtick=data]
\addChainPlotTime{plots/mb2s250millisAvg}{30000}
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},30000) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},30000);
\end{groupplot}
\end{tikzpicture}

\ref{b2millisLegend}
\caption{Trivial Optimization benchmark.\label{easyFig1}}
\end{figure}


Our primary goal is to achieve robust query evaluation for corner cases. Still, we also consider scenarios where sophisticated optimization only adds overheads. Figure~\ref{easyFig1} shows results for the Trivial Optimization benchmark in which all query plans avoiding Cartesian products are equivalent. We are mostly interested in relative execution times obtained for the same execution engine with different optimization strategies. Clearly, optimizers that avoid any exploration perform best in this scenario. For the four baselines sharing the Java-based execution engine (Optimizer, Re-Optimizer, and Eddy), this is the standard optimizer. For the baselines that are based on existing DBMS, the original optimizer works best in each case. The overhead of the adaptive, non-intrusive strategies is more pronounced for the commercial DBMS than for Postgres. We believe that this is due to the fact that our current implementation of the adaptive strategy for the commercial DBMS creates a new JDBC connection in each iteration for the adaptive strategies, this is not the case for Postgres. Still, execution time obtained by the hybrid execution strategies is in all cases within the constant bounds proven in Section~\ref{analysisSec} of the original. While robustness in corner cases clearly costs peak performance in trivial cases, the overheads are bounded.
\end{comment}

\begin{comment}
\begin{figure}
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=3 by 1, x descriptions at=edge bottom, y descriptions at=edge left, horizontal sep=5pt}, width=3.75cm, height=4cm, ybar=0pt, legend entries={Skinner-C,Eddy,Optimizer,Reoptimizer}, legend columns=4, legend to name=b2allGraphsLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks, xtick=data, ymax=10000]
\nextgroupplot[bar width=3pt, title={Chain Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmctsS}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINEddy}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINOpt}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINReopt}] {plots/mb2s1000allGraphsMillisAvg};
\nextgroupplot[bar width=3pt, title={Cycle Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEmctsS}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEEddy}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEOpt}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEReopt}] {plots/mb2s1000allGraphsMillisAvg};
\nextgroupplot[bar width=3pt, title={Star Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmctsS}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAREddy}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAROpt}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARReopt}] {plots/mb2s1000allGraphsMillisAvg};
\end{groupplot}
\end{tikzpicture}

\ref{b2allGraphsLegend}
\caption{Quantifying learning and sampling overheads for Easy Optimization benchmark.\label{easyFig2}}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=3 by 1, x descriptions at=edge bottom, y descriptions at=edge left, horizontal sep=5pt}, width=3.75cm, height=4cm, ybar=0pt, legend entries={Skinner-C,Eddy,Optimizer,Reoptimizer}, legend columns=4, legend to name=b2allGraphsLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={Chain Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmctsS}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINEddy}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINOpt}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINReopt}] {plots/mb2sizesMillisAvg};
\nextgroupplot[bar width=3pt, title={Cycle Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEmctsS}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEEddy}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEOpt}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEReopt}] {plots/mb2sizesMillisAvg};
\nextgroupplot[bar width=3pt, title={Star Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmctsS}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAREddy}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAROpt}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARReopt}] {plots/mb2sizesMillisAvg};
\end{groupplot}
\end{tikzpicture}

\ref{b2allGraphsLegend}
\caption{sizes}
\end{figure}
\end{comment}



\begin{comment}

\pgfplotsset{
   /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
        {draw=blue,fill=blue,mark=none},%
        {draw=blue!50,fill=blue!50,mark=none},%
        {draw=cyan,fill=cyan,mark=none},%
        {draw=blue!70!red,fill=blue!70!red,mark=none},%
        {fill=green,mark=none},%
        {fill=green!50,mark=none},%
        {fill=green!70!red,mark=none},%
        {fill=yellow,mark=none},%
        {fill=yellow!50,mark=none},%
        {fill=yellow!70!red,mark=none},
        {fill=black,mark=none}
     }
   },
}


% Identifier for join graph, T, nrTables, S, table size, m, m
\def\addPlot#1{
\nextgroupplot[bar width=1pt]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3skinner};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3eddy};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3opt};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3reopt};
}

% Identifier for join graph, T, nrTables, S, table size, m, m; title
\def\addTitledPlot#1#2{
\nextgroupplot[bar width=1pt, title={#2}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3skinner};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3eddy};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3opt};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3reopt};
}


\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=4 by 7, y descriptions at=edge left, x descriptions at=edge bottom, vertical sep=4pt, horizontal sep=5pt}, width=3.2cm, height=2.5cm, ylabel={T (ms)}, ylabel near ticks, xlabel={Test case}, xlabel near ticks, ybar=0pt, legend to name=mb3chainLegend, legend entries={Skinner, Eddy, Optimizer, Reoptimizer}, legend columns=4, ymode=log, ymax=15000, ymin=1, ylabel style={font=\scriptsize}, xlabel style={font=\scriptsize}, tick label style={font=\scriptsize}, ymajorgrids]
% 4 tables
\addTitledPlot{CHAINT4S1000m1}{{S; $m=1$}}
\addTitledPlot{CHAINT4S1000m2}{S; $m=n/2$}
\addTitledPlot{CHAINT4S1000000m1}{L; $m=1$}
\addTitledPlot{CHAINT4S1000000m2}{L; $m=n/2$}
% 5 tables
\addPlot{CHAINT5S1000m1}
\addPlot{CHAINT5S1000m2}
\addPlot{CHAINT5S1000000m1}
\addPlot{CHAINT5S1000000m2}
% 6 tables
\addPlot{CHAINT6S1000m1}
\addPlot{CHAINT6S1000m3}
\addPlot{CHAINT6S1000000m1}
\addPlot{CHAINT6S1000000m3}
% 7 tables
\addPlot{CHAINT7S1000m1}
\addPlot{CHAINT7S1000m3}
\addPlot{CHAINT7S1000000m1}
\addPlot{CHAINT7S1000000m3}
% 8 tables
\addPlot{CHAINT8S1000m1}
\addPlot{CHAINT8S1000m4}
\addPlot{CHAINT8S1000000m1}
\addPlot{CHAINT8S1000000m4}
% 9 tables
\addPlot{CHAINT9S1000m1}
\addPlot{CHAINT9S1000m4}
\addPlot{CHAINT9S1000000m1}
\addPlot{CHAINT9S1000000m4}
% 10 tables
\addPlot{CHAINT10S1000m1}
\addPlot{CHAINT10S1000m5}
\addPlot{CHAINT10S1000000m1}
\addPlot{CHAINT10S1000000m5}
\end{groupplot}
\end{tikzpicture}

\ref{mb3chainLegend}
\caption{Correlation Torture benchmark with four (upper row) up to ten tables (bottom row) and with 1,000 (S) or 1,000,000 tuples (L) per table.\label{mb3perTestcase}}
\end{figure}
\end{comment}

%(i.e., overhead of factor 10 and more) 
% (i.e., overhead of factor 100 and more)

%Beyond average run time, we care about robust performance for each test case. We ran another benchmark focused on optimizer robustness. SkinnerDB turns out to be the most robust optimizer by significant margins compared to Eddies, the Reoptimizer, and traditional optimizers. We report details in Appendix~\ref{experimentsApp}. 

%We ran another benchmark focused on optimizer robustness. The benchmark counts the number of ``optimizer failures'' (i.e., the optimizer produces a plan with cost ten times higher than necessary) and ``optimizer disasters'' (i.e., the optimizer produces a plan whose cost is two orders of magnitude higher than necessary). We focus on corner cases and compare SkinnerDB against Eddies, the Reoptimizer, and a traditional optimizer. SkinnerDB turns out to be the most robust optimizer by significant margins. % guarantees most robust optimization in corner cases. 



%It becomes apparent that the overall performance of the baselines is heavily influenced by outliers where evaluation takes significantly longer than necessary. Figure~\ref{disasterFig} makes this effect more visible and summarizes the results from Figure~\ref{mb3perTestcase}. 

% (otherwise, join ordering is trivial) - (where optimization is easy) 






==> sectionsTikz/experimentsApp.tex <==

%, and on a commercial database system ((``ComDB'') with an adaptive optimizer. and the commercial system have . We also re-implemented several research baselines (we were unsuccessful in obtaining the original code), notably Eddies~\cite{Tzoumas2008} and the Re-optimizer~\cite{Wu2016}. Some of our implementations are currently limited to simple queries and can therefore not be used for all benchmarks. Specifically for our micro-benchmarks on small data sets, we execute on a standard laptop with 16~GB of main memory and a 2.5~GHZ Intel i5-7200U CPU running Windows 10. 

We show results for additional benchmarks and baselines. As baseline (and underlying execution engine for SkinnerDB), we add a commercial database system ((``ComDB'') with an adaptive optimizer. We also re-implemented several research baselines (we were unsuccessful in obtaining the original code), notably Eddies~\cite{Tzoumas2008} and the Re-optimizer~\cite{Wu2016}. Some of our implementations are currently limited to simple queries and can therefore not be used for all benchmarks. The following experiments are executed on the hardware described before, except for our micro-benchmarks on small data sets which we execute on a standard laptop with 16~GB of main memory and a 2.5~GHZ Intel i5-7200U CPU.

We use an extended version of the \textit{Optimizer Torture Benchmark} proposed by Wu et al. The idea is to create corner cases where the difference between optimal and sub-optimal query plans is significant. \textit{UDF Torture} designates in the following a benchmark with queries where each join predicate is a user-defined function and therefore a black box from the optimizer perspective. We use one good predicate (i.e., join with that predicate produces an empty result) per query while the remaining predicates are bad (i.e., they are always satisfied for the input data). We experiment with different table sizes and join graph structures. \textit{Correlation Torture} is an extended variant of the original benchmark proposed by Wu et al~\cite{Wu2016}. This benchmark introduces maximal data skew by perfectly correlating values in different table columns. As in the original benchmark, we create chain queries with standard equality join and filter predicates. Correlations between predicates and data skew make it however difficult for standard optimizers to infer the best query plan. We vary the position of the good predicate via parameter $m$ between the beginning of the chain ($m=1$) and the middle ($m=nrTables/2$). %Due to space restrictions, we show a representative extract of our experimental results in the following.


\pgfplotsset{
   /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
        {fill=blue,mark=none},%
        {fill=blue!50,mark=none},%
        {fill=cyan,mark=none},%
        {fill=blue!70!red,mark=none},%
        {fill=green,mark=none},%
        {fill=green!50,mark=none},%
        {fill=green!70!red,mark=none},%
        {fill=yellow,mark=none},%
        {fill=yellow!50,mark=none},%
        {fill=yellow!70!red,mark=none},
        {fill=black,mark=none}
     }
   },
}


\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, width=8.5cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Eddy,Optimizer,Reoptimizer,Postgres,S-G(Postgres),S-H(Postgres),Com-DB,S-G(Com-DB),S-H(Com-DB),MonetDB}, legend columns=3, legend to name=b1millisLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={Chain Queries, 100 tuples/table}]
\addChainPlotTime{plots/mb1s100millisAvg}{30000}

\nextgroupplot[bar width=3pt, title={Star Queries, 100 tuples/table}]
\addStarPlotTime{plots/mb1s100millisAvg}{30000}

\end{groupplot}

\node at (3.25,-4.25) {\ref{b1millisLegend}};
\end{tikzpicture}

\caption{UDF Torture benchmark.\label{udfTortureFig}}
\end{figure}

UDF predicates may hide complex code, invocations of external services, or even calls to human crowd workers. They often have to be treated as black boxes from the optimizer perspective which makes optimization hard. Figure~\ref{udfTortureFig} (this and the following figures show arithmetic averages over ten test cases) compares all baselines according to the UDF Torture benchmark described before (the red line marks the timeout per test case). Skinner-C generally performs best in this scenario and beats existing DBMS by many orders of magnitude. We compare a Java-based implementation against highly optimized DBMS execution engines. However, a high-performance execution engine cannot compensate for the impact of badly chosen join orders. Among the other baselines using the same execution engine as we do, Eddy performs best while Optimizer and Re-optimizer incur huge overheads. Re-optimization is more useful in scenarios where a few selectivity estimates need to be corrected. Here, we essentially start without any information on predicate selectivity. For Postgres, our adaptive processing strategies reduce execution time by up to factor 30 for Postgres and large queries. For the commercial DBMS with adaptive optimizer, we achieve a speedup of up to factor 15 (which is in fact a lower bound due to the timeout). 



\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, width=8.5cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Eddy,Optimizer,Reoptimizer,Postgres,S-G(Postgres),S-H(Postgres),Com-DB,S-G(Com-DB),S-H(Com-DB),MonetDB}, legend columns=3, legend to name=b3largeMillisLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={$m=1$; 1,000,000 tuples/table}]
\addChainPlotTime{plots/mb3m1s1000000clearMillisAvg}{30000}
\nextgroupplot[bar width=3pt, title={$m=nrTables/2$; 1,000,000 tuples/table}]
\addChainPlotTime{plots/mb3m2s1000000clearMillisAvg}{30000}
%\nextgroupplot[bar width=3pt, title={Star Queries}]
%\addStarPlotTime{plots/mb3m1s1000000clearMillisAvg}{30000}
%\nextgroupplot[bar width=3pt, title={Star Queries, $m=nrTables/2$}]
%\addStarPlotTime{plots/mb3m2s1000000clearMillisAvg}{30000}
\end{groupplot}

\node at (3.25,-4.25) {\ref{b3largeMillisLegend}};
\end{tikzpicture}

\caption{Correlation Torture benchmark.\label{correlationLargeFig}}
\end{figure}

Even standard equality predicates can make optimization difficult due to predicate correlations. We evaluate all baselines on the Correlation Torture benchmark~\cite{Wu2016}, Figure~\ref{correlationLargeFig} shows first results. Many of the tendencies are similar to the ones in the UDF Torture benchmark. Skinner-C performs best, traditional query optimizers cope badly with strong predicate correlations. Compared to Figure~\ref{udfTortureFig}, the relative performance gap is slightly smaller. At least in this case, UDF predicates cause more problems than correlations between standard predicates. Again, our adaptive processing strategies improve performance of Postgres and the commercial DBMS significantly and for each configuration (query size and setting for $m$). 

\pgfplotsset{
   /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
        {fill=blue,mark=none},%
        {fill=blue!50,mark=none},%
        {fill=cyan,mark=none},%
        {fill=blue!70!red,mark=none},%
        {fill=green,mark=none},%
        {fill=green!50,mark=none},%
        {fill=green!70!red,mark=none},%
        {fill=yellow,mark=none},%
        {fill=yellow!50,mark=none},%
        {fill=yellow!70!red,mark=none},
        {fill=black,mark=none}
     }
   },
}

\begin{figure}[h!]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=2 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, xlabel={\# Tables}, ybar=0pt, legend entries={Skinner, Eddy, Optimizer, Reoptimizer}, width=4.5cm, height=3cm, ylabel near ticks, xlabel near ticks, legend columns=4, ymajorgrids]
\nextgroupplot[bar width=3pt, ylabel={\# Failures}, legend to name=failuresDisastersLegend, title={By Time}]
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3mctsFailures};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3eddyFailures};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3optFailures};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3reoptFailures};
\nextgroupplot[bar width=3pt, ylabel={\# Disasters}, legend to name=dummy, title={By Time}]
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3mctsDisasters};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3eddyDisasters};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3optDisasters};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3reoptDisasters};


\nextgroupplot[bar width=3pt, ylabel={\# Failures}, legend to name=dummy, title={By \#Evaluations}]
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3mctsFailuresPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3eddyFailuresPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3optFailuresPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3reoptFailuresPreds};
\nextgroupplot[bar width=3pt, ylabel={\# Disasters}, legend to name=dummy, title={By \#Evaluations}]
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3mctsDisastersPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3eddyDisastersPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3optDisastersPreds};
\addplot table[x index=1, y index=0, col sep=comma] {plots/mb3reoptDisastersPreds};
\end{groupplot}

\node at (3.25,-3.75) {\ref{failuresDisastersLegend}};
\end{tikzpicture}

%\ref{failuresDisastersLegend}
\caption{Number of ``optimizer failures'' and ``optimizer disasters''.\label{disasterFig}}
\end{figure}


A query evaluation method that achieves bounded overhead in each single case is typically preferred over a method that oscillates between great performance and significant overheads (even if the average performance is the same). Figure~\ref{disasterFig} summarizes results for a new run of the Correlation Torture benchmark, varying number of tables, table size, as well as parameter $m$. We study robustness of optimization and focus therefore on baselines that use the same execution engine. Note that we compare baselines not only with regards to time, but also with regards to the number of predicate evaluations (see lower row) which depends only on the optimizer. We classify for each baseline a test case as \textit{optimizer failure} if evaluation time exceeds the optimum among the other baselines for that test case by factor 10. We call a test case an \textit{optimizer disaster} for factor 100. The figure shows a tight race between Eddy and the traditional optimizer. Re-optimization clearly improves robustness. However, using our regret-bounded algorithms avoids any failures or disasters and is therefore the most robust optimization method. All implementations in Figure~\ref{disasterFig} share code to the extend possible. Still, some of the baselines need to add code that could in principle decrease performance (e.g., per-tuple routing policies for Eddy). To exclude such effects, we also count the number of atomic predicate evaluations for each baseline and re-calculate failures and disasters based on that (bottom row in Figure~\ref{disasterFig}). The tendencies remain the same.

\pgfplotsset{
    discard if not/.style 2 args={
        x filter/.code={
            \edef\tempa{\thisrowno{#1}}
            \edef\tempb{#2}
            \ifx\tempa\tempb
            \else
                \def\pgfmathresult{inf}
            \fi
        }
    }
}

% Parameters: File name, timeout
\def\addChainPlotTime#1#2{
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmctsS}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINEddy}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINOpt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINReopt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgres}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgresMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgresMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptive}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptiveMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptiveMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmonet}] {#1};
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},#2) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},#2);
}

% Parameters: File name, timeout
\def\addStarPlotTime#1#2{
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmctsS}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAREddy}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAROpt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARReopt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgres}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgresMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgresMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptive}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptiveMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptiveMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmonet}] {#1};
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},#2) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},#2);
}




\begin{figure}
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 1, x descriptions at=edge bottom}, width=8.5cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Eddy,Reoptimizer,Postgres,S-G(Postgres),S-H(Postgres),Com-DB,S-G(Com-DB),S-H(Com-DB)}, legend columns=3, legend to name=b2millisLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks]
\nextgroupplot[bar width=3pt, title={UDF Equality Predicates, 250 tuples/table}, xtick=data]
\addChainPlotTime{plots/mb2s250millisAvg}{30000}
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},30000) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},30000);
\end{groupplot}

\node at (3.25,-1.75) {\ref{b2millisLegend}};
\end{tikzpicture}

\caption{Trivial Optimization benchmark.\label{easyFig1}}
\end{figure}

Our primary goal is to achieve robust query evaluation for corner cases. Still, we also consider scenarios where sophisticated optimization only adds overheads. Figure~\ref{easyFig1} shows results for the Trivial Optimization benchmark in which all query plans avoiding Cartesian products are equivalent. We are mostly interested in relative execution times obtained for the same execution engine with different optimization strategies. Clearly, optimizers that avoid any exploration perform best in this scenario. For the four baselines sharing the Java-based execution engine (Optimizer, Re-Optimizer, and Eddy), this is the standard optimizer. For the baselines that are based on existing DBMS, the original optimizer works best in each case. While robustness in corner cases clearly costs peak performance in trivial cases, the overheads are bounded.






\pgfplotsset{
   /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
        {fill=blue,mark=none},%
        {fill=green,mark=none},%
        {fill=green!50,mark=none},%
        {fill=green!70!red,mark=none},%
        {fill=black,mark=none}
     }
   },
}


\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, width=8.25cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Postgres,S-G(Postgres),S-H(Postgres),MonetDB}, legend columns=3, legend to name=tpchLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={Query}, xticklabels={Q2,Q3,Q5,Q7,Q8,Q9,Q10,Q11,Q18,Q21}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={Standard TPC-H}]
\addplot table[x=Tick, y=Skinner] {plots/tpch.txt};
\addplot table[x=Tick, y=Postgres] {plots/tpch.txt};
\addplot table[x=Tick, y=SkinnerG] {plots/tpch.txt};
\addplot table[x=Tick, y=SkinnerH] {plots/tpch.txt};
\addplot table[x=Tick, y=Monet] {plots/tpch.txt};


\nextgroupplot[bar width=3pt, title={TPC-H with UDFs}]
\addplot table[x=Tick, y=Skinner] {plots/tpch.txt};
\addplot table[x=Tick, y=Postgres] {plots/tpchUDF.txt};
\addplot table[x=Tick, y=SkinnerG] {plots/tpchUDF.txt};
\addplot table[x=Tick, y=SkinnerH] {plots/tpchUDF.txt};
\addplot table[x=Tick, y=MonetDB] {plots/tpchUDF.txt};

\end{groupplot}

\node at (3.25,-4) {\ref{tpchLegend}};
\end{tikzpicture}

\caption{Performance on TPC-H queries.\label{tpchFig}}
\end{figure}


Finally, we benchmark several baselines on the more complex queries of the TPC-H benchmark~\cite{TPC2013}. We restrict evaluated approaches to the ones where our current implementation supports the full set of TPC-H queries. Figure~\ref{tpchFig} reports processing times of ten TPC-H queries that join at least three tables. For each query and each approach, we calculate the relative overhead (i.e., query execution time of approach divided by execution time of best approach for this query). The ``Max.\ Rel.\'' column contains for each approach the maximal value over all queries. We study original TPC-H queries as well as a variant that makes optimization hard. The latter variant replaces all unary query predicates by user-defined functions. Those user-defined functions are semantically equivalent to the original predicate. They typically increase per-tuple evaluation overheads. Most importantly, however, they prevent the optimizer from choosing good query plans. 



\begin{table}[b]
\caption{Result summary for TPC-H variants.\label{tpchTable}}
\begin{tabular}{llll}
\toprule[1pt]
\textbf{Scenario} & \textbf{Approach} & \textbf{Time (s)} & \textbf{Max.\ Rel.\ }\\
\midrule[1pt]
TPC-H & Skinner-C & 9 & 22 \\
\midrule
& Postgres & 15 & 37 \\
\midrule
& S-G(Postgres) & 182 & 594 \\
\midrule
& S-H(Postgres) & 38 & 97 \\
\midrule
& MonetDB & 2 & 3 \\
\midrule[1pt]
TPC-UDF & Skinner-C & 9& 3 \\
\midrule
& Postgres & 3,117 & 3,457 \\
\midrule
& S-G(Postgres) & 305 & 154 \\
\midrule
& S-H(Postgres) & 142 & 88 \\
\midrule
& MonetDB & 53 & 20 \\
\bottomrule[1pt]
\end{tabular}
\end{table}

The upper half of Figure~\ref{tpchFig} shows results on original TPC-H queries while the lower half reports on the UDF variant. Table~\ref{tpchTable} summarizes results, reporting total benchmark time as well as the maximal per-query time overhead (compared to the optimal execution time for that query over all baselines). MonetDB is the clear winner for standard queries (also note that MonetDB and SkinnerDB are column stores while Postgres is a row store). SkinnerDB achieves best performance on the UDF variant. Among the three Postgres-based approaches, the original DBMS performs best on standard cases. The hybrid approach performs reasonably on standard cases but reduces total execution time by an order of magnitude for the UDF scenario. We therefore succeed in trading peak performance in standard cases for robust performance in extreme cases.
\balance

 % On the UDF variant, the hybrid approach reduces total execution time by orders of magnitude.

==> sectionsTikz/experimentsOld.tex <==
\pgfplotsset{
    discard if not/.style 2 args={
        x filter/.code={
            \edef\tempa{\thisrowno{#1}}
            \edef\tempb{#2}
            \ifx\tempa\tempb
            \else
                \def\pgfmathresult{inf}
            \fi
        }
    }
}

% Parameters: File name, timeout
\def\addChainPlotTime#1#2{
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmctsS}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINEddy}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINOpt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINReopt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgres}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgresMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINpostgresMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptive}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptiveMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINadaptiveMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmonet}] {#1};
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},#2) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},#2);
}

% Parameters: File name, timeout
\def\addStarPlotTime#1#2{
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmctsS}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAREddy}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAROpt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARReopt}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgres}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgresMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARpostgresMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptive}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptiveMCTS-Multi-Pure}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARadaptiveMCTS-Multi-Hybrid}] {#1};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmonet}] {#1};
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},#2) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},#2);
}

We implemented the adaptive processing strategies described in Section~\ref{algorithmSec} in a novel DBMS called SkinnerDB. SkinnerDB is designed from the ground up for robust performance, in particular for queries that are hard to optimize for traditional DBMS (e.g., because of UDF predicates or strongly correlated predicates). The current prototype is implemented in Java. %, it supports SPJ queries. %It stores data column-wise and assumes that input data fits into main memory after applying unary predicates.
% (we are currently extending the prototype to handle a richer set of queries)

SkinnerDB can be used as a stand-alone system. In that case, a customized query execution engine is used that is tailored to the requirements of a learning-based query optimization strategy (see Section~\ref{customizedSub}). We call the stand-alone version \textit{Skinner-C} in the following. We use a budget (parameter $b$) of at most 1,000 considered tuples per executor invocation. Our customized execution engine operates on a columnar data layout and assumes that the working set (input data after applying unary predicates) fits into main memory. Alternatively, SkinnerDB can use an existing DBMS as execution engine. The existing DBMS is accessed via JDBC and must support an SQL interface. SkinnerDB can be configured to bypass the optimizer of the traditional DBMS completely, replacing it by a learning-based strategy. We call this version \textit{Skinner-G(X)} in the following, where X designates the DBMS whose execution engine we use. The current version uses optimizer hints to force the underlying DBMS to try out specific join orders. If the DBMS does not support optimizer hints, join orders could be enforced by decomposing joins into separate queries. The corresponding processing strategy is described in Section~\ref{genericSub}. Finally, SkinnerDB can be configured to use a hybrid configuration, dividing execution time between plans proposed by the optimizer of the underlying DBMS and the plans chosen according to the learning strategy. We call this version \textit{Skinner-H(X)} in the following (X designates again the underlying DBMS), details are given in Section~\ref{hybridSub}. 

We compare SkinnerDB against several existing DBMS. \textit{Postgres}~\cite{Postgres} is a popular open-source DBMS with a mature, cost-based query optimizer. \textit{MonetDB}~\cite{Boncz2008} is a column-store DBMS focused on high-performance analytical in-memory processing. We use SkinnerDB on top of Postgres via a pure learning-based approach (Skinner-G(Postgres)) and via the hybrid method (Skinner-H(Postgres)). We did not succeed in running Skinner on top of MonetDB: MonetDB seems not always to respect timeouts set by JDBC. We often had cases where MonetDB kept running until long after the timeout. Being able to impose reliable timeouts is a pre-requisite to use Skinner. We did however implement Skinner on top of a commercial database system, Com-DB in the following, which features an adaptive optimizer. %Our Skinner-adapter for Com-DB currently supports the simpler queries of our micro-benchmarks (but not full TPC-H). 

We compare SkinnerDB against a multitude of other baselines, representing fundamentally different optimization and execution strategies. To isolate the effects of the optimization strategy from the impact of the execution engine, we implemented several optimization strategies using the same customized execution engine as Skinner-C. \textit{Eddy} is an adaptive processing strategy, we use a variant that is based on reinforcement learning~\cite{Tzoumas2008}. We use the Q-learning rule as it was recommended by Tzoumas et al.\ for join ordering. \textit{Opt} designates in the following an idealized version of a traditional, dynamic programming based optimizer~\cite{Selinger1979}. We use a cost model that is tailored to our execution engine and pass it exact selectivity estimates for single (non-UDF) predicates. The latter assumption is optimistic as precise selectivity estimates for single predicates cannot always be obtained. Still, correlations between different predicates remain difficult. \textit{Reopt} designates a recently proposed method~\cite{Wu2016} to overcome the impact of erroneous cardinality estimates on the optimizer. It refines cardinality estimates for intermediate results via sampling, considering intermediate results appearing in the current query plan candidate, and iteratively re-optimizes based on refined estimates (until convergence).

The following experiments on small data sets are executed on a standard laptop with 16~GB of main memory and a 2.5~GHZ Intel i5-7200U CPU running Windows 10. The experiments on the TPC-H database are executed on a Dell PowerEdge R640 server with 2 Intel Xeon 2.3~GHz CPUs and 256~GB of RAM.

%We compare SkinnerDB against several existing DBMS. \textit{Postgres}~\cite{Postgres} is a popular open-source DBMS with a mature, traditional query optimizer. \textit{Com-DB} is a state-of-the-art commercial DBMS with an adaptive optimizer. \textit{MonetDB}~\cite{Boncz2008} is a column-store DBMS focused on analytical main-memory data processing. We use SkinnerDB on top of Postgres and Com-DB via a pure learning-based approach (Skinner-G(Postgres) and Skinner-G(Com-DB)) and via the hybrid method (Skinner-H(Postgres) and Skinner-H(Com-DB)). 

% a

% SIGMOD?% As pointed out in prior work~\cite{Wu2016}, evaluating query optimizers is difficult. Standard benchmarks such as TPC-H~\cite{TPC2013} have been designed to challenge the execution engine, rather than the optimizer. They exclude corner cases (e.g., UDF predicates or data skew and correlated predicates) that are known to cause problems in practice. Our main goal is to provide robust performance in corner cases, leading to optimizer failures (i.e., query plans that are much worse than the optimum) with traditional approaches. To achieve that, we are willing to trade peak performance on standard queries (due to learning overheads). We use several benchmarks to verify whether we achieve that goal. 

%Our first benchmark, \textit{Trivial Optimization}, is representative for standard benchmarks that are easy to optimize. We go to the extreme by creating scenarios in which all query plans are optimal. Our queries are chain queries with UDF equality join predicates, each table contains the same unique values in the join column. This allows us to study learning overheads. 

For our first benchmark, we use largely extended versions of the \textit{Optimizer Torture Benchmark} proposed by Wu et al. The idea is to create corner cases where the difference between optimal and sub-optimal query plans is significant. \textit{UDF Torture} designates in the following a benchmark with queries where each join predicate is a user-defined function and therefore a black box from the optimizer perspective. We use one good predicate (i.e., join with that predicate produces an empty result) per query while the remaining predicates are bad (i.e., they are always satisfied for the input data). We experiment with different table sizes and join graph structures. \textit{Correlation Torture} is an extended variant of the original benchmark proposed by Wu et al~\cite{Wu2016}. As in the original benchmark, we create chain queries with equi-joins and equality filter predicates. Correlations between predicates and data skew make it however difficult for standard optimizers to infer the best query plan. We vary the position of the good predicate via parameter $m$ between the beginning of the chain ($m=1$) and the middle ($m=nrTables/2$). %Due to space restrictions, we show a representative extract of our experimental results in the following.

\begin{table}[t]
\caption{Performance of different query evaluation approaches on the join order benchmark - single-threaded.\label{jobTable}}
\begin{tabular}{p{1.75cm}p{1.25cm}p{1.25cm}p{1.25cm}p{1.25cm}}
\toprule[1pt]
\textbf{Approach} & \textbf{Total Time} & \textbf{Total Card.\ } & \textbf{Max.\ Time} & \textbf{Max.\ Card.\ }\\
\midrule[1pt]
Skinner-C & 182,613 & 111,652,086  & 8,880 & 17,850,688 \\
Random & 2,268,190 & N/A & 332,403 &N/A \\
\midrule
Postgres & 725,804  & 680,633,677 & 59,457  & 177,276,053 \\
S-G(PG) & 13,347,957 & N/A & 839,669 & N/A \\
S-H(PG) & 2,658,166 & N/A & 234,013 & N/A \\
R-H(PG) & 3,614,559 & N/A & 250,711 &N/A \\
\midrule
MonetDB & 985,966 & 2,970,612,019 & 408,684 & 1,186,198,080 \\
S-G(MDB) & 1,852,464 & N/A & 308,058 & N/A\\
S-H(MDB) & 761,524 & N/A & 114,110 & N/A\\
R-H(MDB) & 5,743,782 & N/A & $\geq$ 3,600,000 & N/A \\
\bottomrule[1pt]
\end{tabular}
\end{table}

\begin{table}[t]
\caption{Performance of different query evaluation approaches on the join order benchmark - multi-threaded.\label{jobTable}}
\begin{tabular}{p{1.75cm}p{1.25cm}p{1.25cm}p{1.25cm}p{1.25cm}}
\toprule[1pt]
\textbf{Approach} & \textbf{Total Time} & \textbf{Total Card.\ } & \textbf{Max.\ Time} & \textbf{Max.\ Card.\ }\\
\midrule[1pt]
Skinner-C & 134,655  & 111,652,086 & 7,381 & 17,850,688 \\
Skinner-R & 1,746,468 & N/A & 331736 & N/A \\
%\midrule
%Postgres & & & & \\
%S-G(PG) & N/A & & & \\
%S-H(PG) & & & & \\
\midrule
MonetDB & 104,800 & 2,970,612,019 & 25,804 & 408,684 \\
S-G(MDB) & 1,449,919 & N/A & 68,380 & N/A \\
S-H(MDB) &344,621 & N/A & 85,623 & N/A \\
\bottomrule[1pt]
\end{tabular}
\end{table}

\begin{table}[t]
\caption{Performance of join orders in different execution engines for join order benchmark - single threaded.\label{joinOrdersTable}}
\begin{tabular}{p{1.5cm}p{1.5cm}p{1.75cm}p{1.75cm}}
\toprule[1pt]
\textbf{Engine} & \textbf{Order} & \textbf{Total Time} & \textbf{Max.\ Time} \\
\midrule[1pt]
Skinner & Skinner & 182,613 & 8,880 \\
& Optimal & 179,550 & 6,816 \\
\midrule
Postgres & Original & 725,804 & 59,457 \\
& Skinner & 567,356 & 14,199 \\
& Optimal & 554,641 & 13,628 \\
\midrule
MonetDB & Original & 985,966 & 408,684 \\
& Skinner & 137,565 & 6,569 \\
& Optimal & 133,734 & 5,814 \\
\bottomrule[1pt]
\end{tabular}
\end{table}


\begin{table}[t]
\caption{Performance of join orders in different execution engines for join order benchmark - multi-threaded.\label{joinOrdersTable}}
\begin{tabular}{p{1.5cm}p{1.5cm}p{1.75cm}p{1.75cm}}
\toprule[1pt]
\textbf{Engine} & \textbf{Order} & \textbf{Total Time} & \textbf{Max.\ Time} \\
\midrule[1pt]
Skinner & Skinner & 134,655 & 7,381 \\
& Optimal & 128996 & 6520 \\
%\midrule
%Postgres & Original & & \\
%& Skinner & & \\
%& Optimal & & \\
\midrule
MonetDB & Original & 104,800 & 25,804 \\
& Skinner & 53,432 & 2,657 \\
& Optimal & 51,423 & 2,322  \\
\bottomrule[1pt]
\end{tabular}
\end{table}

\begin{table}[t]
\caption{Performance of different skinner variants \label{joinOrdersTable}}
\begin{tabular}{p{5cm}p{1.25cm}p{1.25cm}}
\toprule[1pt]
\textbf{SkinnerC} & \textbf{Total Time} & \textbf{Max.\ Time} \\
\midrule[1pt]
Original & 134,655 & 7,381 \\
No indices & 162,049 & 8,799  \\
No indices and parallelization & 185,029 & 9,243 \\
No indices and parallelization, RL & 2,268,190 & 332,403 \\
\bottomrule[1pt]
\end{tabular}
\end{table}

\begin{comment}
\begin{figure}[t]
\begin{tikzpicture}
\begin{groupplot}[group style={group size=2 by 1}, width=4cm, ylabel near ticks, xlabel near ticks]
\nextgroupplot[title=Run Time Skew, xlabel={Queries}, ylabel={Run Time (\%)}]
\addplot table[x index=0, y index=3, col sep=tab] {plots/runTimeSkew.txt};
\nextgroupplot[title=Speedup Skew, xlabel={Query Time (s)}, ylabel={Speedup}]
\addplot table[x index=0, y index=3, col sep=tab] {plots/runTimeSkew.txt};
\end{groupplot}
\end{tikzpicture}
\caption{asdf}
\end{figure}
\end{comment}

\begin{figure}[t]
\subfigure[MonetDB spends most time executing a few expensive queries.]{
\begin{tikzpicture}
\begin{axis}[xlabel={Queries}, ylabel={Run Time (\%)}, width=4cm, ylabel near ticks, xlabel near ticks, legend entries={ Skinner, MonetDB}, legend pos=south east, legend style={font=\scriptsize}, ymajorgrids]
\addplot table[x index=0, y index=3, col sep=tab] {plots/runTimeSkinner.txt};
\addplot table[x index=0, y index=3, col sep=tab] {plots/runTimeSkew.txt};
\end{axis}
\end{tikzpicture}
}
\subfigure[SkinnerDB realizes high speedup for two expensive queries.]{
\begin{tikzpicture}
\begin{axis}[xlabel={MonetDB Time (ms)}, ylabel={Speedup}, width=4cm, ylabel near ticks, xlabel near ticks, xmode=log, ymode=log, ymajorgrids]
\addplot[scatter, only marks] table[x index=0, y index=2, col sep=tab] {plots/speedupSkew.txt};
\end{axis}
\end{tikzpicture}
}
\caption{Analyzing the source of SkinnerDB's speedups compared to MonetDB.}
\end{figure}
% RAM: 16 GB
%              CPU: Intel® Core™ i5-7200U CPU @ 2.50GHz 2.71GHz
%              OS: Windows 10 Home 64-bit Operating System


\begin{figure}[t]
\subfigure[The growth of the search tree slows down over time.]{
\begin{tikzpicture}
\begin{axis}[xlabel={Time (scaled)}, ylabel={\#Nodes (scaled)}, width=4cm, ylabel near ticks, xlabel near ticks, ymajorgrids]
%\addplot table[x index=0, y index=2, col sep=tab] {plots/speedupSkew.txt};
\addplot coordinates {(0.25,0.65) (0.5, 0.85) (0.75,0.95) (1,1)};
\end{axis}
\end{tikzpicture}
}
\subfigure[SkinnerDB spends most time executing one or two join orders.]{
\begin{tikzpicture}
\begin{axis}[xlabel={Top-k Orders}, ylabel={Selections (\%)}, width=4cm, ylabel near ticks, xlabel near ticks, legend entries={T:500, T:10}, legend pos=south east, legend style={font=\scriptsize}, xtick=data, ymajorgrids]
\addplot coordinates {(1,0.45) (2,0.65) (3,0.72) (4,0.79) (5,0.81)};
\addplot coordinates {(1,0.65) (2,0.82) (3,0.88) (4,0.89) (5,0.90)};
%\addplot coordinates {(1,0.46) (2,0.57) (3,0.62) (4,0.65) (5,0.68)};
%\addplot coordinates {(1,0.63) (2,0.71) (3,0.74) (4,0.76) (5,0.77)};
\end{axis}
\end{tikzpicture}
}
\caption{Analysis of convergence of SkinnerDB.}
\end{figure}

\begin{figure}[t]
\subfigure[Search tree size is correlated with query size.]{
\begin{tikzpicture}
\begin{axis}[xlabel={\# Joined Tables}, ylabel={\#Nodes}, width=4cm, ylabel near ticks, xlabel near ticks, ymajorgrids, xmode=linear, ymode=log]
\addplot[scatter, only marks] table[x index=0, y index=8, col sep=tab] {plots/treeGrowth.txt};
\end{axis}
\end{tikzpicture}
}
\subfigure[Progress tracker size]{
\begin{tikzpicture}
\begin{axis}[xlabel={\# Joined Tables}, ylabel={\#Nodes}, width=4cm, ylabel near ticks, xlabel near ticks, ymajorgrids, xmode=linear, ymode=log]
\addplot[scatter, only marks] table[x index=0, y index=11, col sep=tab] {plots/treeGrowth.txt};
\end{axis}
\end{tikzpicture}
}
\subfigure[Result size]{
\begin{tikzpicture}
\begin{axis}[xlabel={\# Joined Tables}, ylabel={\#Size}, width=4cm, ylabel near ticks, xlabel near ticks, ymajorgrids, xmode=linear, ymode=log]
\addplot[scatter, only marks] table[x index=0, y index=12, col sep=tab] {plots/treeGrowth.txt};
\end{axis}
\end{tikzpicture}
}
\subfigure[Combined size of intermediate results, progress, and tree.]{
\begin{tikzpicture}
\begin{axis}[xlabel={\# Joined Tables}, ylabel={All Data (GB)}, width=4cm, ylabel near ticks, xlabel near ticks, ymajorgrids, xmode=linear, ymode=log]
\addplot[scatter, only marks] table[x index=0, y index=9, col sep=tab] {plots/treeGrowth.txt};
\end{axis}
\end{tikzpicture}
}
\caption{Memory consumption of SkinnerDB.}
\end{figure}



\pgfplotsset{
   /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
        {fill=blue,mark=none},%
        {fill=blue!50,mark=none},%
        {fill=cyan,mark=none},%
        {fill=blue!70!red,mark=none},%
        {fill=green,mark=none},%
        {fill=green!50,mark=none},%
        {fill=green!70!red,mark=none},%
        {fill=yellow,mark=none},%
        {fill=yellow!50,mark=none},%
        {fill=yellow!70!red,mark=none},
        {fill=black,mark=none}
     }
   },
}


\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, width=8.5cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Eddy,Optimizer,Reoptimizer,Postgres,S-G(Postgres),S-H(Postgres),Com-DB,S-G(Com-DB),S-H(Com-DB),MonetDB}, legend columns=3, legend to name=b1millisLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={Chain Queries, 100 tuples/table}]
\addChainPlotTime{plots/mb1s100millisAvg}{30000}

\nextgroupplot[bar width=3pt, title={Star Queries, 100 tuples/table}]
\addStarPlotTime{plots/mb1s100millisAvg}{30000}

\end{groupplot}
\end{tikzpicture}

\ref{b1millisLegend}
\caption{UDF Torture benchmark.\label{udfTortureFig}}
\end{figure}

UDF predicates may hide complex code, invocations of external services, or even calls to human crowd workers. They often have to be treated as black boxes from the optimizer perspective which makes optimization hard. Figure~\ref{udfTortureFig} (this and the following figures show arithmetic averages over ten test cases) compares all baselines according to the UDF Torture benchmark described before (the red line marks the timeout per test case). Skinner-C generally performs best in this scenario and beats existing DBMS by many orders of magnitude. We compare a Java-based implementation against highly optimized DBMS execution engines. However, a high-performance execution engine cannot compensate for the impact of badly chosen join orders. Among the other baselines using the same execution engine as we do, Eddy performs best while Optimizer and Re-optimizer incur huge overheads. Re-optimization is more useful in scenarios where a few selectivity estimates need to be corrected. Here, we essentially start without any information on predicate selectivity. For Postgres, our adaptive processing strategies reduce execution time by up to factor 30 for Postgres and large queries. For the commercial DBMS with adaptive optimizer, we achieve a speedup of up to factor 15 (which is in fact a lower bound due to the timeout). 

\begin{comment}
\begin{figure}
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 1, x descriptions at=edge bottom}, width=8.5cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Eddy,Reoptimizer,Postgres,S-G(Postgres),S-H(Postgres),Com-DB,S-G(Com-DB),S-H(Com-DB)}, legend columns=3, legend to name=b2millisLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks]
\nextgroupplot[bar width=3pt, title={UDF Equality Predicates, 250 tuples/table}, xtick=data]
\addChainPlotTime{plots/mb2s250millisAvg}{30000}
\draw [red, ultra thick] (axis cs:\pgfkeysvalueof{/pgfplots/xmin},30000) -- (axis cs:\pgfkeysvalueof{/pgfplots/xmax},30000);
\end{groupplot}
\end{tikzpicture}

\ref{b2millisLegend}
\caption{Trivial Optimization benchmark.\label{easyFig1}}
\end{figure}


Our primary goal is to achieve robust query evaluation for corner cases. Still, we also consider scenarios where sophisticated optimization only adds overheads. Figure~\ref{easyFig1} shows results for the Trivial Optimization benchmark in which all query plans avoiding Cartesian products are equivalent. We are mostly interested in relative execution times obtained for the same execution engine with different optimization strategies. Clearly, optimizers that avoid any exploration perform best in this scenario. For the four baselines sharing the Java-based execution engine (Optimizer, Re-Optimizer, and Eddy), this is the standard optimizer. For the baselines that are based on existing DBMS, the original optimizer works best in each case. The overhead of the adaptive, non-intrusive strategies is more pronounced for the commercial DBMS than for Postgres. We believe that this is due to the fact that our current implementation of the adaptive strategy for the commercial DBMS creates a new JDBC connection in each iteration for the adaptive strategies, this is not the case for Postgres. Still, execution time obtained by the hybrid execution strategies is in all cases within the constant bounds proven in Section~\ref{analysisSec} of the original. While robustness in corner cases clearly costs peak performance in trivial cases, the overheads are bounded.
\end{comment}

\begin{comment}
\begin{figure}
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=3 by 1, x descriptions at=edge bottom, y descriptions at=edge left, horizontal sep=5pt}, width=3.75cm, height=4cm, ybar=0pt, legend entries={Skinner-C,Eddy,Optimizer,Reoptimizer}, legend columns=4, legend to name=b2allGraphsLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks, xtick=data, ymax=10000]
\nextgroupplot[bar width=3pt, title={Chain Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmctsS}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINEddy}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINOpt}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINReopt}] {plots/mb2s1000allGraphsMillisAvg};
\nextgroupplot[bar width=3pt, title={Cycle Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEmctsS}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEEddy}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEOpt}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEReopt}] {plots/mb2s1000allGraphsMillisAvg};
\nextgroupplot[bar width=3pt, title={Star Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmctsS}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAREddy}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAROpt}] {plots/mb2s1000allGraphsMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARReopt}] {plots/mb2s1000allGraphsMillisAvg};
\end{groupplot}
\end{tikzpicture}

\ref{b2allGraphsLegend}
\caption{Quantifying learning and sampling overheads for Easy Optimization benchmark.\label{easyFig2}}
\end{figure}
\end{comment}

\begin{comment}
\begin{figure}
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=3 by 1, x descriptions at=edge bottom, y descriptions at=edge left, horizontal sep=5pt}, width=3.75cm, height=4cm, ybar=0pt, legend entries={Skinner-C,Eddy,Optimizer,Reoptimizer}, legend columns=4, legend to name=b2allGraphsLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={Chain Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINmctsS}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINEddy}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINOpt}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CHAINReopt}] {plots/mb2sizesMillisAvg};
\nextgroupplot[bar width=3pt, title={Cycle Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEmctsS}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEEddy}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEOpt}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{CYCLEReopt}] {plots/mb2sizesMillisAvg};
\nextgroupplot[bar width=3pt, title={Star Graph}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARmctsS}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAREddy}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STAROpt}] {plots/mb2sizesMillisAvg};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{STARReopt}] {plots/mb2sizesMillisAvg};
\end{groupplot}
\end{tikzpicture}

\ref{b2allGraphsLegend}
\caption{sizes}
\end{figure}
\end{comment}



\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, width=8.5cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Eddy,Optimizer,Reoptimizer,Postgres,S-G(Postgres),S-H(Postgres),Com-DB,S-G(Com-DB),S-H(Com-DB),MonetDB}, legend columns=3, legend to name=b3largeMillisLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={\# Tables}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={$m=1$; 1,000,000 tuples/table}]
\addChainPlotTime{plots/mb3m1s1000000clearMillisAvg}{30000}
\nextgroupplot[bar width=3pt, title={$m=nrTables/2$; 1,000,000 tuples/table}]
\addChainPlotTime{plots/mb3m2s1000000clearMillisAvg}{30000}
%\nextgroupplot[bar width=3pt, title={Star Queries}]
%\addStarPlotTime{plots/mb3m1s1000000clearMillisAvg}{30000}
%\nextgroupplot[bar width=3pt, title={Star Queries, $m=nrTables/2$}]
%\addStarPlotTime{plots/mb3m2s1000000clearMillisAvg}{30000}
\end{groupplot}
\end{tikzpicture}

\ref{b3largeMillisLegend}
\caption{Correlation Torture benchmark.\label{correlationLargeFig}}
\end{figure}

Even standard equality predicates can make optimization difficult due to predicate correlations. We evaluate all baselines on the Correlation Torture benchmark~\cite{Wu2016}, Figure~\ref{correlationLargeFig} shows first results. Many of the tendencies are similar to the ones in the UDF Torture benchmark. Skinner-C performs best, traditional query optimizers cope badly with strong predicate correlations. Compared to Figure~\ref{udfTortureFig}, the relative performance gap is slightly smaller. At least in this case, UDF predicates cause more problems than correlations between standard predicates. Again, our adaptive processing strategies improve performance of Postgres and the commercial DBMS significantly and for each configuration (query size and setting for $m$). 

\begin{comment}

\pgfplotsset{
   /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
        {draw=blue,fill=blue,mark=none},%
        {draw=blue!50,fill=blue!50,mark=none},%
        {draw=cyan,fill=cyan,mark=none},%
        {draw=blue!70!red,fill=blue!70!red,mark=none},%
        {fill=green,mark=none},%
        {fill=green!50,mark=none},%
        {fill=green!70!red,mark=none},%
        {fill=yellow,mark=none},%
        {fill=yellow!50,mark=none},%
        {fill=yellow!70!red,mark=none},
        {fill=black,mark=none}
     }
   },
}


% Identifier for join graph, T, nrTables, S, table size, m, m
\def\addPlot#1{
\nextgroupplot[bar width=1pt]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3skinner};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3eddy};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3opt};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3reopt};
}

% Identifier for join graph, T, nrTables, S, table size, m, m; title
\def\addTitledPlot#1#2{
\nextgroupplot[bar width=1pt, title={#2}]
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3skinner};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3eddy};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3opt};
\addplot table[x index=1, y index=2, col sep=comma, discard if not={0}{#1}] {plots/mb3reopt};
}


\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=4 by 7, y descriptions at=edge left, x descriptions at=edge bottom, vertical sep=4pt, horizontal sep=5pt}, width=3.2cm, height=2.5cm, ylabel={T (ms)}, ylabel near ticks, xlabel={Test case}, xlabel near ticks, ybar=0pt, legend to name=mb3chainLegend, legend entries={Skinner, Eddy, Optimizer, Reoptimizer}, legend columns=4, ymode=log, ymax=15000, ymin=1, ylabel style={font=\scriptsize}, xlabel style={font=\scriptsize}, tick label style={font=\scriptsize}, ymajorgrids]
% 4 tables
\addTitledPlot{CHAINT4S1000m1}{{S; $m=1$}}
\addTitledPlot{CHAINT4S1000m2}{S; $m=n/2$}
\addTitledPlot{CHAINT4S1000000m1}{L; $m=1$}
\addTitledPlot{CHAINT4S1000000m2}{L; $m=n/2$}
% 5 tables
\addPlot{CHAINT5S1000m1}
\addPlot{CHAINT5S1000m2}
\addPlot{CHAINT5S1000000m1}
\addPlot{CHAINT5S1000000m2}
% 6 tables
\addPlot{CHAINT6S1000m1}
\addPlot{CHAINT6S1000m3}
\addPlot{CHAINT6S1000000m1}
\addPlot{CHAINT6S1000000m3}
% 7 tables
\addPlot{CHAINT7S1000m1}
\addPlot{CHAINT7S1000m3}
\addPlot{CHAINT7S1000000m1}
\addPlot{CHAINT7S1000000m3}
% 8 tables
\addPlot{CHAINT8S1000m1}
\addPlot{CHAINT8S1000m4}
\addPlot{CHAINT8S1000000m1}
\addPlot{CHAINT8S1000000m4}
% 9 tables
\addPlot{CHAINT9S1000m1}
\addPlot{CHAINT9S1000m4}
\addPlot{CHAINT9S1000000m1}
\addPlot{CHAINT9S1000000m4}
% 10 tables
\addPlot{CHAINT10S1000m1}
\addPlot{CHAINT10S1000m5}
\addPlot{CHAINT10S1000000m1}
\addPlot{CHAINT10S1000000m5}
\end{groupplot}
\end{tikzpicture}

\ref{mb3chainLegend}
\caption{Correlation Torture benchmark with four (upper row) up to ten tables (bottom row) and with 1,000 (S) or 1,000,000 tuples (L) per table.\label{mb3perTestcase}}
\end{figure}
\end{comment}

%(i.e., overhead of factor 10 and more) 
% (i.e., overhead of factor 100 and more)

Beyond average run time, we care about robust performance for each test case. We ran another benchmark focused on optimizer robustness. SkinnerDB turns out to be the most robust optimizer by significant margins compared to Eddies, the Reoptimizer, and traditional optimizers. We report details in Appendix~\ref{experimentsApp}. 

%We ran another benchmark focused on optimizer robustness. The benchmark counts the number of ``optimizer failures'' (i.e., the optimizer produces a plan with cost ten times higher than necessary) and ``optimizer disasters'' (i.e., the optimizer produces a plan whose cost is two orders of magnitude higher than necessary). We focus on corner cases and compare SkinnerDB against Eddies, the Reoptimizer, and a traditional optimizer. SkinnerDB turns out to be the most robust optimizer by significant margins. % guarantees most robust optimization in corner cases. 



%It becomes apparent that the overall performance of the baselines is heavily influenced by outliers where evaluation takes significantly longer than necessary. Figure~\ref{disasterFig} makes this effect more visible and summarizes the results from Figure~\ref{mb3perTestcase}. 


\pgfplotsset{
   /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
        {fill=blue,mark=none},%
        {fill=green,mark=none},%
        {fill=green!50,mark=none},%
        {fill=green!70!red,mark=none},%
        {fill=black,mark=none}
     }
   },
}


\begin{figure}[t]
\center
\begin{tikzpicture}
\begin{groupplot}[group style={group size=1 by 2, x descriptions at=edge bottom, vertical sep=0.85cm}, width=8.25cm, height=3cm, ybar=0pt, legend entries={Skinner-C,Postgres,S-G(Postgres),S-H(Postgres),MonetDB}, legend columns=3, legend to name=tpchLegend, ymode=log, ymajorgrids, ylabel={Time (ms)}, xlabel={Query}, xticklabels={Q2,Q3,Q5,Q7,Q8,Q9,Q10,Q11,Q18,Q21}, ylabel near ticks, xtick=data]
\nextgroupplot[bar width=3pt, title={Standard TPC-H}]
\addplot table[x=Tick, y=Skinner] {plots/tpch.txt};
\addplot table[x=Tick, y=Postgres] {plots/tpch.txt};
\addplot table[x=Tick, y=SkinnerG] {plots/tpch.txt};
\addplot table[x=Tick, y=SkinnerH] {plots/tpch.txt};
\addplot table[x=Tick, y=Monet] {plots/tpch.txt};


\nextgroupplot[bar width=3pt, title={TPC-H with UDFs}]
\addplot table[x=Tick, y=Skinner] {plots/tpch.txt};
\addplot table[x=Tick, y=Postgres] {plots/tpchUDF.txt};
\addplot table[x=Tick, y=SkinnerG] {plots/tpchUDF.txt};
\addplot table[x=Tick, y=SkinnerH] {plots/tpchUDF.txt};
\addplot table[x=Tick, y=MonetDB] {plots/tpchUDF.txt};

\end{groupplot}
\end{tikzpicture}

\ref{tpchLegend}
\caption{Performance on TPC-H queries.\label{tpchFig}}
\end{figure}

\begin{table}
\caption{Result summary for TPC-H variants.\label{tpchTable}}
\begin{tabular}{llll}
\toprule[1pt]
\textbf{Scenario} & \textbf{Approach} & \textbf{Time (s)} & \textbf{Max.\ Rel.\ }\\
\midrule[1pt]
TPC-H & Skinner-C & 9 & 22 \\
\midrule
& Postgres & 15 & 37 \\
\midrule
& S-G(Postgres) & 182 & 594 \\
\midrule
& S-H(Postgres) & 38 & 97 \\
\midrule
& MonetDB & 2 & 3 \\
\midrule[1pt]
TPC-UDF & Skinner-C & 9& 3 \\
\midrule
& Postgres & 3,117 & 3,457 \\
\midrule
& S-G(Postgres) & 305 & 154 \\
\midrule
& S-H(Postgres) & 142 & 88 \\
\midrule
& MonetDB & 53 & 20 \\
\bottomrule[1pt]
\end{tabular}
\end{table}


Finally, we benchmark several baselines on the more complex queries of the TPC-H benchmark~\cite{TPC2013}. We restrict evaluated approaches to the ones where our current implementation supports the full set of TPC-H queries. Figure~\ref{tpchFig} reports processing times of ten TPC-H queries that join at least three tables. We study original TPC-H queries as well as a variant that makes optimization hard. The latter variant replaces all unary query predicates by user-defined functions. Those user-defined functions are semantically equivalent to the original predicate. They typically increase per-tuple evaluation overheads. Most importantly, however, they prevent the optimizer from choosing good query plans. The upper half of Figure~\ref{tpchFig} shows results on original TPC-H queries while the lower half reports on the UDF variant. Table~\ref{tpchTable} summarizes results, reporting total benchmark time as well as the maximal per-query time overhead (compared to the optimal execution time for that query over all baselines). MonetDB is the clear winner for standard queries. SkinnerDB achieves best performance on the UDF variant. Among the three Postgres-based approaches, the original DBMS performs best on standard cases. The hybrid approach performs reasonably on standard cases but reduces total execution time by an order of magnitude for the UDF scenario. We therefore succeed in trading peak performance in standard cases for robust performance in extreme cases. % On the UDF variant, the hybrid approach reduces total execution time by orders of magnitude.

% (otherwise, join ordering is trivial) - (where optimization is easy) 






==> sectionsTikz/intro.tex <==

%\textit{``Let’s attack problems that really matter, those that account for optimizer disasters, and stop polishing the round ball!''} --- Guy Lohman\\

%So c’mon, folks, l
\begin{center}
\textit{``The consequences of an act affect the probability of its occurring again.''} --- B.F. Skinner.
\end{center}

Estimating execution cost of plan candidates is perhaps the primary challenge in query optimization~\cite{Lohman2014}. Query optimizers predict cost based on coarse-grained data statistics and under simplifying assumptions (e.g., independent predicates). If estimates are wrong, query optimizers may pick plans whose execution cost is sub-optimal by orders of magnitude. We present SkinnerDB, a novel database system designed from the ground up for reliable query optimization.

%that is 

SkinnerDB maintains no data statistics and uses no simplifying cost and cardinality models. Instead, SkinnerDB learns (near-)optimal left-deep query plans \textit{from scratch} and on the fly, i.e.\ \textit{during} the execution of a given query. This distinguishes SkinnerDB from several other recent projects that apply learning in the context of query optimization~\cite{Krishnan2018, Marcus2018}: instead of learning from past query executions to optimize the next query, we learn from the current query execution to optimize the remaining execution of the current query. Hence, SkinnerDB does not suffer from any kind of generalization error across queries (even seemingly small changes to a query can change the optimal join order significantly). %Everything we learn is immediately relevant to the query at hand.

SkinnerDB partitions the execution of a query into many, very small time slices (e.g., tens of thousands of slices per second). Execution proceeds according to different join orders in different time slices. Result tuples produced in different time slices are merged until a complete result is obtained. After each time slice, execution progress is measured which informs us on the quality of the current join order. At the beginning of each time slice, we choose the join order that currently seems most interesting. In that choice, we balance the need for exploitation (i.e., trying join orders that worked well in the past) and exploration (i.e., trying join orders about which little is known). We use the UCT algorithm~\cite{Kocsis2006} in order to optimally balance between those two goals.


\begin{figure}[t]
\begin{tikzpicture}
\draw[ultra thick, ->] (0,0) -- (0,3);
\draw[ultra thick, ->] (0,0) -- (4.5,0);
\node[align=center] at (-1.25,2.5) {Optimal};
\node[align=center] at (-1.25,1.5) {Near-Optimal};
\node[align=center] at (-1.25,0.5) {Expected\\Near-Optimal};
\node at (1,-0.5) {Complete};
\node at (2.5,-0.5) {Partial};
\node at (4,-0.5) {None};
\node[align=center, blue] at (1,2.5) {Traditional\\Optimization};
\node[align=center, blue] at (2.5,1.5) {Robust\\Optimization};
\node[align=center, blue] at (4,0.5) {Regret-Bounded\\Evaluation};
\node[font=\itshape] at (0,3.2) {Plan Quality};
\node[font=\itshape] at (2.5,-1) {A-priori Information};
\foreach \i in {1,2.5,4}{%
\draw[black] (\i,-0.1) -- (\i,0.1);
}
\foreach \i in {0.5,1.5,2.5}{%
\draw[black] (-0.1,\i) -- (0.1,\i);
}
\end{tikzpicture}
\caption{Tradeoffs between a-priori information and guarantees on plan quality in query evaluation.\label{guaranteesVsAssumptionsFig}}
\end{figure}

Along with SkinnerDB, we introduce a new quality criterion for query evaluation methods. We measure the distance (additive difference or ratio) between expected execution time and execution time for an optimal join order. This criterion is motivated by formal regret bounds provided by many reinforcement learning methods. In the face of uncertainty, based on minimal assumptions, they still bound the difference between expected and optimal average decision quality. Traditional query optimization guarantee optimal plans, provided that complete information (e.g., on predicate selectivity and predicate correlations) is a-priori available. We assume that no a-priori information is available at the beginning of query execution (see Figure~\ref{guaranteesVsAssumptionsFig}, comparing different models in terms of assumptions and guarantees). Our scenario matches therefore the one considered in reinforcement learning. This motivates us to apply a similar quality criterion. The adaptive processing strategies used in SkinnerDB are optimized for that criterion.




SkinnerDB comes in multiple variants. Skinner-G sits on top of a generic SQL processing engine. Using optimizer hints (or equivalent mechanisms), we force the underlying engine to execute specific join orders on data batches. We use timeouts to limit the impact of bad join orders (which can be significant, as intermediate results can be large even for small base table batches). Of course, the optimal timeout per batch is initially unknown. Hence, we iterate over different timeouts, carefully balancing execution time dedicated to different timeouts while learning optimal join orders. Skinner-H is similar to Skinner-G in that it uses an existing database management system as execution engine. However, instead of learning new plans from scratch, it partitions execution time between learned plans and plans proposed by the original optimizer. 

Both, Skinner-G and Skinner-H, rely on a generic execution engine. However, existing systems are not optimized for switching between different join orders during execution with a very high frequency. Skinner-C exploits a customized execution engine that is tailored to the requirements of regret-bounded query evaluation. It features a multi-way join strategy that keeps intermediate results minimal, thereby allowing quick suspend and resume for a given join order. Further, it allows to share execution progress between different join orders and to measure progress per time slice at a very fine granularity (which is important to quickly obtain quality estimates for join orders). 

In our formal analysis, we compare expected execution time against execution time of an optimal join order for all Skinner variants. For sufficiently large amounts of input data to process and under moderately simplifying assumptions, we are able to derive upper bounds on the difference between the two metrics. In particular for Skinner-C, the ratio of expected to optimal execution time is for all queries upper-bounded by a low-order polynomial in the query size. Given misleading statistics or assumptions, traditional query optimizers may select plans whose execution time is higher than optimal by a factor that is exponential in the number of tables joined. The same applies to adaptive processing strategies~\cite{Tzoumas2008} which, even if they converge to optimal join orders over time, do not bound the overhead caused by single tuples processed along bad join paths.

SkinnerDB pays for reliable join ordering with overheads for learning and join order switching. In our experiments with various baselines and benchmarks, we study under which circumstances the benefits outweigh the drawbacks. When considering accumulated execution time on difficult benchmarks (e.g., the join order benchmark~\cite{Gubichev2015}), it turns out that SkinnerDB can beat even highly performance-optimized systems for analytical processing with a traditional optimizer. While per-tuple processing overheads are significantly lower for the latter, SkinnerDB minimizes the total number of tuples processed via better join orders.

We summarize our original scientific contributions:

\begin{itemize}
\item We introduce a new quality criterion for query evaluation strategies that compares expected and optimal execution cost.
\item We propose several adaptive execution strategies based on reinforcement learning. 
\item We formally prove correctness and regret bounds for those execution strategies.
\item We experimentally compare those strategies, implemented in SkinnerDB, against various baselines.
\end{itemize}

The remainder of this paper is organized as follows. We discuss related work in Section~\ref{relatedSec}. We describe the primary components of SkinnerDB in Section~\ref{overviewSec}. In Section~\ref{algorithmSec}, we describe our query evaluation strategies based on reinforcement learning. In Section~\ref{analysisSec}, we analyze those strategies formally, we prove correctness and performance properties. Finally, in Section~\ref{experimentsSec}, we describe the implementation in SkinnerDB and compare our approaches experimentally against a diverse set of baselines. The appendix contains additional experimental results.

%The remainder of this paper is organized as follows. We discuss related work in Section~\ref{relatedSec}. In Section

%executing diverse queries on 

%We evaluate SkinnerDB experimentally against various adaptive and non-adaptive baselines, using a multitude of benchmarks (e.g., the join order benchmark, TPC-H, and variants of the optimizer torture benchmark). We 


\begin{comment}
The goal of query optimization is to translate a declarative query, describing data to generate, into an optimal query plan. Execution cost of good and bad plans for a given query often differs by many orders of magnitude~\cite{Gubichev2015}, making reliable query optimization a prerequisite for high-performance data processing. Perhaps surprisingly, the primary challenge in query optimization is often not the enumeration of an overly large search space. Instead, the primary challenge is to reliably identify the plan with minimal execution cost.

Execution cost estimates are based on cardinality estimates for intermediate results, generated during the execution of a query plan. Accurately estimating the size of intermediate results is however inherently difficult before a plan is executed~\cite{Gubichev2015}. For instance, correlations between query predicates make it hard to estimate the selectivity of predicate groups. Complex user-defined predicates (UDFs) have to be treated as black boxes from the optimizer perspective, at least when being encountered for the first time, and make optimization even harder. Traditional optimizers base their estimates on coarse-grained statistics about value distributions and many simplifying assumptions (e.g., independence between different query predicates) that are all too often violated. In that case, disastrous query plans may result whose execution time is higher than the optimum by many orders of magnitude. 

We can gain information on the cardinality of intermediate results by executing plans (or plan fragments) on data samples. Such information is valuable as it might lead to better decisions with regards to query plan properties such as join order. On the other side, collecting information is computationally expensive. We cannot obtain reliable size estimates for all intermediate result candidates (as their number grows quickly as a function of query size). We need an appropriate strategy to balance the value of collected information against the cost of collecting it. The area of reinforcement learning~\cite{Kaelbling1996} has produced a rich body of work providing strategies with formal guarantees for such scenarios. In this paper, we propose, analyze, and evaluate several query processing strategies that use reinforcement learning to evaluate queries in a near-optimal fashion.

The idea to use adaptive query processing~\cite{Avnur2000}, even based on reinforcement learning~\cite{Tzoumas2008}, is not new and has been explored a decade ago. Ultimately, adaptive processing strategies have not seen widespread adoption in practice and the dominant approach to query evaluation separates optimization from query execution. We believe however that the time is right to re-evaluate adaptive processing strategies and that adaptivity combined with learning could hold the key to more robust query evaluation performance. First, new reinforcement learning algorithms~\cite{Browne2012} have become available that were used with significant success on large-scale planning problems (such as query optimization). Second, growing main memory sizes have enabled data processing in RAM in many scenarios~\cite{Kemper2011}. In such scenarios, fine-grained random data access becomes efficient. It thereby facilitates data processing strategies that use random sampling or switch quickly between different join orders (such as the strategies proposed in this paper). Third, many emerging scenarios lead to queries becoming more diverse, e.g.\ mixing SQL with machine learning primitives~\cite{Kumar2015} or UDFs hiding complex code~\cite{Karanasos2014a}, or even the invocation of human crowd workers~\cite{Franklin2011}. All those tendencies make it more difficult to apply traditional query optimization, based on analytical cost models. Finally, previously proposed adaptive processing strategies such as Eddies typically require a redesign of the execution engine, thereby hindering adoption. In this paper, we show that (while a specialized execution engine remains helpful) learning based strategies can be used on top of existing database management systems (DBMS) in a \textit{completely non-intrusive manner} (i.e, without changing a single line of DBMS code). 
\end{comment}

\begin{comment}

%Our ambition in SkinnerDB is to translate such regret bounds from the domain of reinforcement learning to the domain of query evaluation. 


Query optimization is hard due to unreliable cardinality and cost models. We present SkinnerDB, a system that is designed from the ground up for reliable optimization. SkinnerDB divides query execution into many small time slices. It tries different join orders in different slices, measures evaluation progress, and gradually converges to optimal left-deep join orders for the current query. Query results are combined from partial results produced in different episodes. 

We use reinforcement learning to converge to optimal join orders. Reinforcement learning provides us with a principled mechanism to balance exploitation (trying join orders that worked well in past episodes) and exploitation (trying join orders about which little is known). We use the UCT algorithm which formally guarantees that regret (i.e., expected difference between actual and possible reward) is bounded. We design SkinnerDB to translate those guarantees, given simplifying assumptions, to the query evaluation domain. This means that we guarantee near-optimal expected execution time with regards to join ordering once query execution is long enough.


Our focus differs from prior work on learning optimizers~\cite{Stillger2001} or learning DBMS~\cite{Pavlo2017}. Those approaches generally learn from the execution of past queries in order to improve optimization of the following queries. This is however only possible if future queries are similar enough to past queries,if this similarity can be recognized by the optimizer, and if the underlying data remains stable. Even slight changes to a query can change execution time of plan candidates significantly. Instead of learning from past executions, our goal is to learn \textit{during the execution of a query}. This ensures that all gained knowledge is directly applicable to the query at hand.

%To enable learning during the execution of a single query, we divide query evaluation into many small time periods. We may try out a different join order in each period. Our selection of the next join order is generally based on our experiences gained from trying join orders in the preceding time periods. Here, we face a dilemma. In order to finish execution as quickly as possible, we are motivated to \textit{exploit} previously gained knowledge and to use a join order that has worked well in the preceding periods (i.e., small execution time for a small data batch or, equivalently, fast progress for a fixed time budget). On the other side, we are motivated to try out join orders about which little is known so far as we have not tried them (often) yet. Such \textit{exploration} could give us valuable information allowing us to speed up query evaluation via better choices in the future. All our processing strategies use the so called UCT algorithm~\cite{Kocsis2006} to strike an optimal balance between exploration (i.e., learning about new join orders) and exploitation (i.e., using join orders that have shown to work well for the current query). 

SkinnerDB supports three processing strategies. The first processing strategy sits on top of an existing DBMS that is used as execution engine. In our experiments (see Section~\ref{experimentsSec}), we use for instance Postgres, MonetDB, and a commercial DBMS as underlying execution engines. We initially partition input data into small batches and use optimizer hints combined with timeouts to force the DBMS to explore different join orders. A crucial question in this context is the choice of an appropriate timeout. Choosing the timeout per batch too low prevents us from making progress. Choosing it too high allows bad join orders to increase execution time far beyond the time required by an optimal join order. Of course, we cannot know initially what timeout is optimal. We use an iterative scheme that selects timeouts from a geometric progression, carefully balancing execution time between different timeouts and slowly increasing the set of considered timeouts as execution time increases. The UCT algorithm, based on an appropriate search space and reward function, governs the choice of join orders for specific timeouts. The algorithm is iterative and ends once all data batches have been processed, thereby generating a complete result for the input query.

This strategy completely bypasses the original query optimizer. This is appropriate in corner cases for difficult-to-optimize queries with UDF predicates for instance. However, it adds unnecessary learning overheads for standard queries that are easy to optimize by the original system. To combine good performance for difficult queries with reasonable performance for standard queries, we propose a hybrid evaluation strategy. This strategy divides execution time between time dedicated to plans proposed by the original optimizer and execution time dedicated to the learning based approach. We show later, from the theoretical and empirical perspective, that this strategy achieves robust performance in a variety of scenarios.

The previous two strategies can in principle work on top of any SQL engine that supports timeouts and a means of fixing join orders. We treat the DBMS as a black box and make no assumptions on the internal processes by which queries are evaluated. For this flexibility, we pay a performance overhead. Our last and most efficient evaluation strategy is based on a specialized execution engine, that is tailored towards the requirements of a learning based query evaluation strategy. Most importantly, the execution engine must enable us to switch quickly between different join orders, to repeatedly interrupt processing of a join order with little penalty, and to share evaluation progress as much as possible between different join orders. Among the key ideas to achieve those features, is a multi-way join strategy and a specialized tuple representation. Both aim at keeping intermediate results produced during execution as small as possible to speed up restoring and backing up evaluation progress when switching join orders.

Reinforcement learning methods typically come with formal guarantees bounding the expected regret (which is obtained by making optimal or near-optimal choices during learning). Our goal is to translate those regret bounds into bounds on execution cost regret in query evaluation. More precisely, we define as \textit{regret} the time difference between actual query evaluation time for a given query and evaluation time required by an optimal join order. We show (in Section~\ref{analysisSec}) that our processing strategies offer bounds on expected regret of the form $(1-1/Poly(m))\cdot n+O(\log(n)))$ where $n$ is evaluation time and $m$ is the number of joined tables in the current query ($Poly()$ designates a polynomial). We put those results into context. For traditional optimizers, the difference between execution time of an optimal and sub-optimal query plan can grow exponentially in the number of query tables. Hence, for worst-case queries where simplifying assumptions in cardinality estimation lead to sub-optimal plan choices, the regret of a traditional optimizer could grow as $(1-1/Exp(m))\cdot n$ (where $Exp(m)$ designates an exponential function in the number of joined tables). Hence, our evaluation strategies are provably more robust than traditional query optimization. To the best of our knowledge, our evaluation strategies are the first ones for which such bounds have been proven. 

Furthermore, we show in our experiments that we obtain significantly better performance in corner cases than three high-performance DBMS. We show that our methods are more robust than re-optimization or prior adaptive strategies (Eddy with reinforcement learning~\cite{Tzoumas2008}). In summary, the original scientific contributions of this paper are the following.

%Also, we show that, in particular via the hybrid processing strategies, existing DBMS can be made more robust for difficult queries in a completely non-intrusive manner. I

\begin{itemize}
\item We describe several novel query evaluation strategies based on reinforcement learning. Some of those strategies can be used on top of any existing DBMS in a completely non-intrusive manner. Our primary contribution is a specialized query execution engine that is tailored towards the requirements of reinforcement learning.
\item We analyze our methods formally. In particular, we prove that the expected regret (i.e., difference between actual execution time and time for the optimal join order) is upper-bounded.
\item We evaluate our methods experimentally against various adaptive and non-adaptive processing strategies and DBMS on the join order benchmark~\cite{Gubichev2015}, TPC-H variants, and on synthetic test cases. 
\end{itemize}

%Especially in corner cases, our methods improve performance by many orders of magnitude. Even for existing DBMS, we achieve more robust performance by partially bypassing the original optimizer via optimizer hints alone.

%, against Postgres, MonetDB, and a commercial DBMS with an adaptive optimizer. 

The remainder of this paper is organized as follows. We discuss related work in Section~\ref{relatedSec}. In Section~\ref{algorithmSec}, we describe our query evaluation strategies based on reinforcement learning. In Section~\ref{analysisSec}, we analyze those strategies formally, we prove correctness and performance properties. Finally, in Section~\ref{experimentsSec}, we describe the implementation in SkinnerDB and compare our approaches experimentally against a diverse set of baselines. The appendix contains additional experimental results.
\end{comment}

==> sectionsTikz/overview.tex <==
\section{Overview}
\label{overviewSec}

\tikzstyle{SkinnerComponent}=[anchor=center, draw=black, fill=blue!15, minimum width=1.6cm, align=center, font=\small]

\tikzstyle{SkinnerComponent2}=[anchor=center, draw=black, rounded corners=0.15cm, fill=red!15, minimum width=1.75cm, align=center, font=\small]

\tikzstyle{SkinnerIO}=[anchor=center, font=\small]

\tikzstyle{SkinnerFlow}=[ultra thick, draw]


\begin{figure}
\begin{tikzpicture}
\node[SkinnerIO] (query) at (-2,0) {Query};
\node[SkinnerIO] (result) at (-2,-1) {Result};
\node[SkinnerComponent] (preprocessor) at (-0.25,0) {Pre-\\Processor};
\node[SkinnerComponent] (postprocessor) at (-0.25,-1) {Post-\\Processor};
\node[SkinnerComponent, minimum width=4.25cm, minimum height=2.7cm] (joinProcessor) at (3.125,-0.15) {};
\node at (3.125,1) {Join Processor};
%\draw[fill=blue!15, draw] (1.75,-1.5) rectangle (6,2);
\node[SkinnerComponent2] (optimizer) at (2,0.25) {Learning\\Optimizer};
\node[SkinnerComponent2] (executor) at (4.25,0.25) {Join\\Executor};
\node[SkinnerComponent2] (tracker) at (4.25,-1) {Progress\\Tracker};
\node[SkinnerComponent2] (calculator) at (2,-1) {Reward\\Calculator};
\draw[SkinnerFlow, ->] (query) -- (preprocessor);
\draw[SkinnerFlow, ->] (postprocessor) -- (result);
\draw[SkinnerFlow, ->] (optimizer) -- (executor);
\draw[SkinnerFlow, <->] (executor) -- (tracker);
\draw[SkinnerFlow, ->] (tracker) -- (calculator);
\draw[SkinnerFlow, ->] (calculator) -- (optimizer);
\draw[SkinnerFlow, ->] (preprocessor.east) -- ++ (0.4,0);
\draw[SkinnerFlow, ->] (postprocessor.east) ++ (0.4,0) -- ++ (-0.4,0);
\end{tikzpicture}
\caption{Primary components of SkinnerDB.\label{architectureFig}}
\end{figure}

Figure~\ref{architectureFig} shows the primary components of SkinnerDB. This high-level outline applies to all of the SkinnerDB variants. 

The pre-processor is invoked first for each query. Here, we filter base tables via unary predicates. Also, depending on the SkinnerDB variant, we partition the remaining tuples into batches or hash them (to support joins with equality predicates). 

Join execution proceeds in small time slices. The join processor consists of several sub-components. The learning optimizer selects a join order to try next at the beginning of each time slice. It uses statistics on the quality of join orders that were collected during the current query execution. Selected join orders are forwarded to the join executor. This component executes the join order until a small timeout is reached. We add result tuples into a result set, checking for duplicate results generated by different join orders. The join executor can be either a generic SQL processor or, for maximal performance, a specialized execution engine. The same join order may get selected repeatedly. The progress tracker keeps track of which input data has been processed already. For Skinner-C, it even tracks execution state for each join order tried so far, and merges progress across join orders. At the start of each time slice, we consult the progress tracker to restore the latest state stored for the current join order. At the end of it, we backup progress achieved during the current time slice. The reward calculator calculates a reward value, based on progress achieved during the current time slice. This reward is a measure for how quickly execution proceeds using the chosen join order. It is used as input by the optimizer to determine the most interesting join order to try in the next time slice.

Finally, we invoke the post-processor, using the join result tuples as input. Post-processing involves grouping, aggregation, and sorting. In the next section, we describe the algorithms executed within SkinnerDB.

%Before starting execution, the executor restores 

%For maximal performance, a specialized execution engine supporting fast join order switching should be used. 

%Before execution starts, we consult the progress tracker component to restore execution state 

==> sectionsTikz/postgresApp.tex <==
We describe the non-intrusive version of SkinnerDB in more detail. Our system uses an adapter component that needs to be specialized to each database system. For instance, the component issues DBMS-specific commands to bypass the original optimizer. To make the following explanations more concrete, we describe optimization on top of the Postgres database system. The following approach can however be ported easily to different DBMS engines as long as certain conditions are satisfied (e.g., the engine must implement JDBC-based timeouts efficiently).

We perform the following steps for an input query with a single join block (no nested queries). We use the original Postgres optimizer and engine to process queries joining less than three tables. If the query joins at least three tables then join ordering becomes important. In a first step, we evaluate unary predicates on all base tables. This is important as we would otherwise filter the same tuples multiple times, creating unnecessary overheads. We insert filtered tables into views associated with the base tables.

Next, we initialize the UCT algorithm for the current query. We set the appropriate optimizer parameters (e.g, the Postgres parameter {\textsf join\_collapse\_limit}) to ensure that the input join order is not changed. Each iteration of the UCT algorithm selects a join order to evaluate. We evaluate join orders on a small data batches. Given a join order such as $L\Join O\Join C$, we select a small batch from the leftmost table ($L$) and join it with remaining (i.e., not yet processed) tuples from all other tables. 

Hence, we need a mechanism to retrieve small batches from a relation. Perhaps the easiest method uses a combination of LIMIT and OFFSET clauses to retrieve batches. For instance, assume that the first 500 tuples have been processed for tables $O$ and $C$ and the first 12000 tuples have been processed for table $L$ (this information is captured in the table offsets). We generally form batches whose size is a fixed percentage of the relation cardinality. Assume we consider batches of size 0.1\% and table $L$ has six million entries. Hence, we want to retrieve the next 6,000 tuples from table $L$. For the other tables, we want to consider all tuples after the offset. 

This translates into an SQL query of the following form: {\textsf Select ... From (Select ... From L LIMIT 6000 OFFSET 12000) AS L, (SELECT ... FROM O OFFSET 500) AS O, (SELECT ... FROM C OFFSET 500) AS C WHERE ...}. We can execute that query with a timeout and insert its result into a temporary table. If the timeout is reached before processing finishes then no tuples are inserted and a reward of zero is counted. If processing finishes, a reward of one is assigned to the join order $L\Join O\Join C$, tuples are inserted, and the offset of table $L$ is increased by 6,000 tuples. Processing finishes once the offset for a table reaches its cardinality (i.e., we run out of tuples). 

In that case, a complete join result has been generated. Group-by clauses, aggregates, and having clauses are now applied in a post-processing step. If the current join query is nested within a larger query, processing continues for that query, using the previously generated intermediate result.

Note that the aforementioned method for accessing tuple batches comes with inefficiencies. More precisely: we read the first tuples of each table many times, leading to bounded but non-negligible overheads. Also, the retrieval method is based on the assumption that tuple order remains fixed during processing. Another possibility is to partition tables a-priori into batches. This creates partitioning overheads but no tuples need to be skipped. Both approaches lead to overheads on standard queries. They pay however off once finding good join orders becomes difficult.

==> sectionsTikz/regretApp.tex <==

We analyze regret for two previously proposed approaches in a worst case: traditional optimizers~\cite{Selinger1979}, separating planning from execution, and Eddies~\cite{Tzoumas2008}.

Assume a query joining $m$ tables ($m$ is a constant) of cardinality $s$ ($s$ is variable). Tables are connected in a chain via join predicates and one unary predicate is placed on each table. All predicates evaluate to true on each tuple with the exception of the unary predicate on table $t^*$, located on one end of the chain. The latter predicate evaluates to false on each tuple. We consider left-deep join orders that avoid Cartesaian products and measure execution cost by the number of tuples read. Clearly, an optimal plan reads tuples from $t^*$ first and terminates in $O(s)$. If we choose to start from the table at the opposite end of the chain, $t^{-}$, compared to $t^*$, execution cost are in $O(s^{m-1})$. 

If a traditional optimizer~\cite{Selinger1979} cannot reliably estimate the selectivity of predicates (e.g., because they are user-defined functions or because of data skew), we can consider the choice of the first join order table as random. Assuming for instance a uniform distribution, the expected regret is in $O(s^{m-2})$ (based on a $1/m$ chance of selecting $t^-$). Eddies~\cite{Tzoumas2008} fare slightly better in this extreme case. They operate on small data batches (e.g., tuples) and adapt their join order based on feedback. However, Eddies never discard partial results and join them with all remaining tables. If at least one tuple is selected from table $t^-$, there is no other way of completing it into result tuples than consecutive joins with all remaining tables. However, as the associated join predicates are non-selective, execution time will be in $O(s^{m-2})$. Assuming optimistically that Eddies will learn an optimal order after the very first tuple is selected, and assuming a uniform distribution over tables for the initial tuple choice, we have expected regret in $O(s^{m-3})$ for Eddies. 

==> sectionsTikz/related.tex <==
\section{Related Work}
\label{relatedSec}

%Various algorithms have been proposed that exhaustively or heuristically explore the space of alternative plans for a given query~\cite{Bennett1991, graefe1993volcano, ioannidis1990randomized, Selinger1979, Steinbrunn1997}. They are typically based on analytical models that allow them to estimate execution cost for a given plan. Doing so requires first to estimate the cardinality and size of intermediate results generated during the execution of a plan candidate. The standard approach to estimate cardinality is based on data statistics in the form of histograms~\cite{Ioannidis1995, Muralikrishna1988, Piatetsky-Shapiro1984}. Creating and maintaining histograms leads however to overheads, in particular for large and frequently updated data sets~\cite{Karanasos2014a}. Histogram-based cardinality estimates are inherently unreliable as histograms cannot take into account all possible data correlations and their granularity is limited. Statistics-based cardinality estimation becomes impossible for emergent scenarios where query parts must be treated as black boxes from the optimizer perspective~\cite{Garcia-molina2014}. 

%The insight that cardinality and therefore cost estimates are notoriously unreliable has triggered research on query optimization methods that rely less on such estimates. Robust query optimization algorithms~\cite{Babcock2005, D.2008} assume that cardinality estimates are approximately known within certain bounds. They find plans that perform reasonably well across all possible scenarios. Such approaches need however reasonably close estimates to work well (which is often not the case~\cite{El-Helw2009}) and are typically subject to additional restrictions (e.g., uncertainty refers only to the cardinality of base tables after filtering~\cite{D.2008}). An even more extreme reaction to uncertain cost and cardinality estimates are query optimization methods which assume no information about the selectivity of a few predicates~\cite{Dutt2014a, Dutt2014}. In contrast to this work, those prior approaches use however analytical cost and cardinality models that are based on simplifying assumptions (e.g., independent predicates). 

%A complementary line of research has explored methods to improve estimates by information gathered at run time or in a pre-processing step. Several systems~\cite{Brown2003, Ilyas2004, Tzoumas} perform a pre-processing step to find out about data correlations to improve cardinality estimates. This creates however overheads and certain query properties (e.g., their predicates) must be known in advance. Approaches for interleaved query execution and optimization~\cite{Aboulnaga2004a, Avnur2000, Babu2005} repair initial plans at run time if cardinality estimates turn out to be wrong. They require reasonable cardinality estimates to start from and suboptimal plans are not always associated with erroneous cardinality estimates (instead, the model might only overestimate cost or cardinality for the truly optimal plan while estimates for sub-optimal plans are accurate). Other approaches evaluate predicates on data samples to estimate cardinality~\cite{Bruno2002, Chaudhuri2001, Haas1992, Haas2011, Karanasos2014a, Lipton1990a, Markl2013, Wu2016}. Most of them generate an initial plan via standard methods from which the intermediate results are selected for cardinality estimation via sampling. All of them rely in some form on standard cost and cardinality models to generate query plans. They are therefore implicitly based on simplifying assumptions and cannot give end-to-end guarantees on expected query evaluation cost.

%The practicality of such approaches was questioned due to high sampling overheads~\cite{Ioannidis1995}. The shift towards main-memory databases might however change those

%A large body of work addresses the question of how to make query optimizers more robust. 
Our approach connects to prior work collecting information on predicate selectivity by evaluating them on data samples~\cite{Bruno2002, Chaudhuri2001, Haas1992, Haas2011, Karanasos2014a, Lipton1990a, Markl2013, Wu2016}. We compare in our experiments against a recently proposed representative~\cite{Wu2016}. Most prior approaches rely on a traditional optimizer to select interesting intermediate results to sample. They suffer if the original optimizer generates bad plans. The same applies to approaches for interleaved query execution and optimization~\cite{Aboulnaga2004a, Avnur2000, Babu2005} that repair initial plans at run time if cardinality estimates turn out to be wrong. Robust query optimization~\cite{Alyoubi2015, Alyoubi2016, Babcock2005, D.2008} assumes that predicate selectivity is known within narrow intervals which is often not the case~\cite{El-Helw2009}. Prior work~\cite{Dutt2014a, Dutt2014} on query optimization without selectivity estimation is based on simplifying assumptions (e.g., independent predicates) that are often violated.

%in the context of databases 

Machine learning has been used to estimate cost for query plans whose cardinality values are known~\cite{Akdere2011, Li2012}, to predict query~\cite{Ganapathi} or workflow~\cite{Popescu2013} execution times, result cardinality~\cite{Malik2006, Malik2007}, or interference between query executions~\cite{Duggan2011}. LEO~\cite{Aboulnaga2004a, Stillger2001}, IBM's learning optimizer, leverages past query executions to improve cardinality estimates for similar queries. Ewen et al.~\cite{Ewen2005} use a similar approach for federated database systems. Several recent approaches~\cite{Krishnan2018, Marcus2018} use learning for join ordering. All of the aforementioned approaches learn from past queries for the optimization of future queries. To be effective, new queries must be similar to prior queries and this similarity must be recognizable. Instead, we learn \textit{during} the execution of a query. %given query to converge to optimal join orders. This requires specialized execution strategies and is necessary to derive formal bounds on expected regret. 

%This works only if past queries are similar and if this similarity can be recognized (slight changes in the query can lead to huge differences in execution time for a given join order). Instead, we focus on learning during the execution of a given query. 

%Ewen et al.~\cite{Ewen2005} use a similar approach for federated database systems. Recent efforts leverage machine learning for database tuning and physical design optimization~\cite{Aken, Basu2015a, Pavlo2017}. Another recent work learns from past query executions to improve answers to future approximate queries~\cite{YongjooParkAhmadShahabTajikMichaelCafarella2017}. Our work focuses on join ordering and we learn during the execution of a query. 

%Our work differs in several aspects from those prior approaches. First, it targets the classical query optimization problem (instead of tuning or physical design optimization) where choosing a wrong join order can easily have devastating effects. Second, instead of learning from past executions to benefit future executions, the goal is to learn and improve \textit{during} the execution of a query. %Most importantly, the goal is to provide formal end-to-end guarantees on expected execution time which distinguishes Skinner from all prior work.

%We propose adaptive query processing strategies. 
Adaptive processing strategies have been explored in prior work~\cite{Avnur2000, Deshpande2004, Deshpande2006a, Quanzhong2007a, Raman2003, Tzoumas2008, Viglas2003}. Our work uses reinforcement learning and is therefore most related to prior work using reinforcement learning in the context of Eddies~\cite{Tzoumas2008}. We compare against this approach in our experiments. Eddies do not provide formal guarantees on the relationship between expected execution time and the optimum. They never discard intermediate results, even if joining them with the remaining tables creates disproportional overheads. Eddies support bushy query plans in contrast to our approach. Bushy plans can in principle decrease execution cost compared to the best left-deep plan. However, optimal left-deep plans typically achieve reasonable performance~\cite{Gubichev2015}. Also, as we show in our experiments, reliably identifying near-optimal left-deep plans can be better than selecting bushy query plans via non-robust optimization.

%Among the differences are for instance the following. First, we use a more recent reinforcement learning algorithm~\cite{Gelly2012} as base. Second, we cleanly separate learning-related data structures from the execution engine, allowing us to perform join order learning on top of existing DBMSs in a non-intrusive manner (Eddies associate single tuples or tuple batches with meta-data). Third, Eddies do not deliberately discard intermediate result tuples but complete them instead. We take great care not to spend a disproportional amount of time on bad join orders and may discard intermediate results if they seem to be part of bad join orders. We could not achieve our formal regret bounds without that feature. 

Our work relates to prior work on filter ordering with regret bounds~\cite{Condon2009a}. Join ordering introduces however new challenges, compared to filter ordering. In particular, applying more filters can only decrease the size of intermediate results. The relative overhead of a bad filter order, compared to the optimum, grows therefore linearly in the number of filters. The overhead of bad join orders, compared to the optimum, can grow exponentially in the query size. This motivates mechanisms that bound join overheads for single data batches, as well as mechanisms to save progress for partially processed data batches. 

Worst-case optimal join algorithms~\cite{Ngo2012, Veldhuizen2012} bound cost as a function of worst-case query result size. We bound expected execution cost as a function of cost for processing an optimal join order. Further, prior work on worst-case optimal joins focuses on conjunctive queries while we support a broader class of queries, including queries with user-defined function predicates. Our approach applies to SQL with standard semantics while systems for worst-case optimal evaluation typically assume set semantics~\cite{Veldhuizen2012}. 

%In contrast to worst-case optimal join algorithms~\cite{Ngo2012}, our guarantees are probabilistic and refer to optimal execution time (not worst-case result sizes). Also, they are valid for arbitrary predicates (no restriction to equality predicates).

% They did not see widespread adoption in practice but the tradeoffs have changed since that time. First, main-memory resident data sets are more common, reducing the overhead of randomized access (which is typical for adaptive processing strategies). Second, user-defined predicates and complex functions are more common in queries which reduces the efficiency of traditional query evaluation strategies. Finally, a plethora of new reinforcement learning methods have become available in the meantime (e.g., the UCT algorithm~\cite{Browne2012}) that have not been used for query evaluation so far. Our approach differs from prior work in adaptive processing in terms of scope (i.e., focus on main memory data processing), methods (i.e., powerful reinforcement methods will be used that were not available or not yet popularized when adaptive processing was explored for the last time), and focus (the goal is to translate formal guarantees, provided by reinforcement learning methods, into guarantees on near-optimal evaluation costs). 

%Further, note that prior adaptive processing strategies typically rely heavily on initial query plans, produced by a traditional optimizer. If the initial plan is far from the optimum, most prior strategies do not even formally guarantee to converge to an optimal plan over time (not to mention doing so with regret bounds). For instance, measuring the conditional selectivity of predicates in a given join order~\cite{Quanzhong2007} and performing adaptive optimization based on that is insufficient: useful correlations between predicates may remain undiscovered if they do not manifest in the initial join order. Our work goes far beyond those prior approaches. It represents a radical departure from traditional methods as it abandons traditional optimization altogether. Instead of relying on initial plans that are produced based on simplifying assumptions, the entire space of plans is systematically explored. This exploration is controlled by sophisticated search strategies that result in formal regret bounds.
